HypeR: Hypothetical Reasoning With What-If and How-To Queries Using a Probabilistic Causal Approach

What-if (provisioning for an update to a database) and how-to (how to modify the database to achieve a goal) analyses provide insights to users who wish to examine hypothetical scenarios without making actual changes to a database and thereby help plan strategies in their fields. Typically, such analyses are done by testing the effect of an update in the existing database on a specific view created by a query of interest. In real-world scenarios, however, an update to a particular part of the database may affect tuples and attributes in a completely different part due to implicit semantic dependencies. To allow for hypothetical reasoning while accommodating such dependencies, we develop HypeR, a framework that supports what-if and how-to queries accounting for probabilistic dependencies among attributes captured by a probabilistic causal model. We extend the SQL syntax to include the necessary operators for expressing these hypothetical queries, define their semantics, devise efficient algorithms and optimizations to compute their results using concepts from causality and probabilistic databases, and evaluate the effectiveness of our approach experimentally.

==> algorithms_what_if.tex <==
\section{algorithms and optimizations}\label{sec:algorithms}


% \subsection{Causal Hypothetical Updates}
% \amir{Why do we need this section?}
% \babak{We are going to related causal inference with the proposed probablistic model. We need a short intro to causal inference here.}

% \sr{*****COPY PASTE FROM OLD SECTION 2 BELOW******}

% \paragraph{Causal model}
% We assume that the database $D$ is associated with a Probabilistic Causal Model (PCM) $P$ \cite{?}. 
% % that defines the probability distribution over $PWD(D)$ after a hypothetical update.
% The PCM defines a probability distribution based on the database, the update, and the causal dependency DAG. 
% We next give an intuitive description of a causal DAG. We refer the reader to the causal inference literature for the formal definitions of PCMs, causal DAGs, and the structural equations that define the probability distribution in a rigorous manner \cite{?}, as these are beyond the scope of this paper.

% In a causal DAG $G = (\mb{V},\mb{E})$, each node $A_i \in \mb{V}$ represents an attribute name and each edge $(A_i, A_j) \in \mb{E}$ says that the attribute $A_i$ affects the attribute $A_j$. 
% % \amir{verify:} Only attributes in ${\mb A_{mu}}$ can have incoming edges, as they are the only ones that can be changed. 
% Given a database instance $D$, a {\em grounded causal DAG} is a DAG based a causal DAG $G$, where each node represents a cell of $D$ with attribute $A_i$ and the edges represent the dependency relationships between the attributes, as expressed in $G$. 
% Formally, if $G = (\mb{V},\mb{E})$, the grounded DAG, $G_g$, includes the nodes $\{A[t_i] \in D ~|~ A \in \mb{V}\}$ and $(A_i[t_k], A_j[t_k])$ is in $G_g$ if $(A_i, A_j) \in \mb{E}$. Additionally, $(A_i[t_a], A_j[t_b])$ may be included in $G_g$ if there is a cross-tuple dependency between the attribute $A_i[t_a]$ and the attribute $A_j[t_b]$. 

% Throughout the paper, we assume that we have {\em structural homogeneity}, introduced in \cite{SalimiPKGRS20}. 
% % which is necessary for estimating the conditional probability distributions from a given database. 
% \amir{verify:} Specifically, we assume that for every grounded attribute $A \in {\mb A_{mu}}$, its values in the database share the same conditional probability distribution, given their parents in the causal DAG. 
% % For instance, in Figure~\ref{ex:grounded-graph}, we assume that all groundings of type $\mathit{Price}$ share the same conditional probability distribution.
% For instance, in Figure~\ref{ex:grounded-graph}, we assume that $\pr_{D,P,u}(\mathit{Price}[p_1] \mid \mathit{Quality}[p_1])$ share the same probability distribution as $\pr_{D,P,u}(\mathit{Price}[p_2] \mid \mathit{Quality}[p_2])$.
% This will allow us to compute what-if and how-to query results using causal inference in the following sections. 


% \begin{table}[h]
% \begin{small}
% \centering
% \caption{Notations \amir{move to the model section}}\label{tbl:notations}
% \begin{tabular}{| c | c | c |}
% \hline $D$ & Database instance\\
% $PWD(D)$ & Possible worlds of $D$\\
% $u$ & Hypothetical updates\\
% $G$ & Causal DAG\\
% $P$ & PCM based on $D$ and $G$\\
% $\pr_{D,P,U}$ & Probability dist. over $PWD(D)$ defined by $D,P,U$\\
% \hline
% \end{tabular}
% \end{small}
% \end{table}

\subsection{Computation of What-If Queries}
A naive computation of what-if queries would consider all possible paths in the grounded causal graph, and thus result in exponential complexity in the size of the database. 
% Therefore, we consider a partition of the database into blocks of tuples, where each block is independent from all other blocks. 

% However, if the database $D$ can be partitioned into blocks of tuples $B_1, \ldots, B_l$ such that $B_i \subseteq D$, $\cup_{i=1}^l B_i = D$, $B_i \cap B_j = \emptyset$, the computation can be made more effitient


% We use the following {\em structural homogeneity assumption} introduced in \cite{SalimiPKGRS20}, which is necessary for estimating the conditional probability distributions from a given observed dataset, and thereby conduct causal inference. \amir{More context?}
% % Recall that  $\fAtt^{\skl} \subseteq \FAtt^{\skl}$ denotes the set of all groundings of an attribute $\fAtt \in \FAtt$ in $\FAtt^{\skl}$: 

% \begin{itemize}
%     \item \textbf{Structural homogeneity:}  All grounded attributes ${\mb A_{mu}}$ of the same  attribute $A \in \mb A_{mu}$ share the same structural equation and, hence, the same conditional probability distribution in equation \ref{eq:bayesian}.
% \end{itemize}

% %that all the grounded atoms $\fAtt[\mb x] \in \fAtt^{\skl}$ of an attribute function $\fAtt \in \fAtt$ have the same generative process. 
% For instance, in Figure~\ref{ex:grounded-graph}, we assume that all groundings of type $\mathit{Price}$ share the same conditional probability distribution. 

To simplify computation in the context of probabilistic databases, the literature proposes block-independent databases \cite{ReS07,DalviRS09}.

\begin{definition}[Block-independent database]
Given a database $D$ associated with a PCM $P$ with a grounded causal DAG $G_g$, $D$ is a block-independent database if $D$ can be partitioned into blocks of tuples $B_1, \ldots, B_l$ such that $B_i \subseteq D$, $\cup_{i=1}^l B_i = D$, $B_i \cap B_j = \emptyset$, and for each $t \in B_i$ and $t' \in B_j$, there are no edges in $G_g$ between the cells of $t$ and $t'$, i.e., $t$ and $t'$ are independent in the PCM. 
\end{definition}

\begin{example}\label{ex:blocks}
In the database presented in Figure \ref{fig:database}, blocks can be defined according to the category, i.e., the first three tuples in Figure \ref{tbl:amazondatabase} form a block that is independent from the rest of the tuples since they all have Category Laptop. 
\end{example}


In our model, given a database $D$ with independent blocks $B_1, \ldots, B_l$, we can decompose the probability of an instance $I$ by using the formula
$\pr_{D,U}(I) = \prod_{i=1}^l \pr_{D,U}({B_i})$. 
In particular, when the blocks are of size $1$, i.e., all tuples in $D$ are independent, we can say that $\pr_{D,U}(I) = \prod_{i=1}^n \pr_{D,U}({t_i})$. 

We can also marginalize the distribution $\pr_{D,U}$ over the possible worlds of the database $D$ given a what-if query $Q$, denoted by $PWD(Q,D)$ (Definition \ref{def:rel-poss-worlds}) to get a distribution and a set of possible worlds for any subset of tuples $B_i\subseteq D$, $PWD(Q',B_i)$, where $PWD(Q,B_i)$ are all instances where all tuples $t' \notin B_i$ remain unchanged and all attributes of $t\in B_i$ can get all possible values from their respective domains.
% For this analysis, we consider a block decomposition of $D$, denoted by $\mathcal{B}_D=\{B_1,\cdots,B_k\}$ where $B_i\cap B_j = \phi, \forall i\neq j$ and $\cup B_i = D$ where tuples in different blocks are independent. 

% We now present a proposition that allows us to compute the output of a what-if query over the entire database by computing a slightly different what-if query over each block and summing the results. 
We now present a definition of decomposable functions that allows us to compute the output of a what-if query over the entire database by computing a slightly different what-if query over each block and summing the results. 

\begin{definition}[Decomposable aggregate function]\label{def:decomposable}
Given a database $D$ that can be divided into blocks $\mathcal{B} = \{B_1, \ldots, B_l\}$, a what-if query $Q$, and a PCM $P$ that defines the possible worlds of $Q(D)$, an aggregate function $f: D \to \mathbb{R}$ is decomposable if there exist functions $f': \mathcal{B} \to \mathbb{R}$ and $g: \{x_1, \ldots, x_l\} \to \mathbb{R}$, $x_i \in \mathbb{R}$, such that: 
\begin{itemize}
    \item $f(Q,D,I) = g(\{f'(Q,D,B) \mid \forall B\in \mathcal{B}_I\})$
    \item $\alpha g(\{x_1,\ldots,x_l\}) = g(\{\alpha x_1,\ldots,\alpha x_l\})$, $\forall \alpha \geq 0$
    \item $ g(\{x_1,\ldots,x_l\}) + g(\{y_1,\ldots,y_l\}) = g(\{x_1+y_1,\ldots, x_l+y_l\})$
\end{itemize}\label{assume:homogenous}
\end{definition}

Every supported aggregate function in this paper  
($\sumsql$, $\avg$, $\ct$, $\minsql$) is decomposable. We next demonstrate this for $\avg$. 
% e.g., $\sumsql$ can be broken down into the sum of each block as $f'$ and the sum of the sums of all blocks as $g$. 
\begin{example}\label{ex:decomposable}
Reconsider the what-if query in Figure \ref{fig:whatif-query}. Suppose the database can be partitioned into blocks by Category as demonstrated in Example \ref{ex:blocks}. 
In this case $f(Q,D,I) = \avg(\{t'.Price \mid t'\in I, t.Category = Laptop, t'.ID=t.ID\})$. 
We use the formula for decomposing average $\avg(D) = \sum_{i=1}^l \frac{|B_i|}{|D|} \avg(B_i)$. 
For each block, 
$f'(Q,B'',B') = \frac{|B''|}{|D|} \avg(\{t'.Price \mid t'\in I, t.Category = Laptop, t'.PID=t.PID\})$ and $g = \sumsql$. Indeed, $\sumsql$ satisfies the properties in Definition \ref{def:decomposable}.
\end{example}

% represented as $f$ in the query in Figure \ref{fig:generic-query}, there exists a function that operates on blocks $f'$ such that $f(Q,D,I) = \sum_{B\in \mathcal{B}_I} f'(Q,D,B)$ for some $f'$. 
% All supported aggregates satisfy this assumption Note that $f(Q,D,B)=f'(Q,D,B)$ if $Agg$ denotes $\ct$ or $\sumsql$. Whenever $Agg=\avg$ or $Agg=\minsql$, $f'(Q,D,B)=c f(Q,D,B)$, where $c$ is a constant that can be estimated from the query $Q$. \sg{Add more discussion on f'}

% \begin{proposition}\label{prop:blocks}
% Consider the what-if query $Q$:
% \begin{align*}
% &Q\equiv\when\  g(A_l)\  Then\\
% &\update\ A_c= c\\
% &\select\ Agg(\post(B))\\
% &\where\  \pre(A_j)=a_j~\and\ \post(A_i) = a_i %~\and\\
% %&\groupby&\  \pre(A_k), \post(A_p)
% \end{align*}
% and $f(Q,D,I)$ as in Definition \ref{def:agg_func}. If $f(Q,D,I) = \sum_{B\in \mathcal{B}_I} f'(Q,D,B)$, then $Q(D) = \sum_{B''\in \mathcal{B}_D}\expectation_{B' \in \overline{PWD}(Q,B'')}[f'(Q, D, B')] $.
% \end{proposition}

\begin{proposition}\label{prop:blocks}
Given a database $D$ that can be divided into blocks $\mathcal{B} = \{B_1, \ldots, B_l\}$, the what-if query $Q$:
\begin{align*}
&\use\\ 
& (\select\ T1.ID, T1.A_j, T1.A_i, Agg1(T2.B)\\
& \where\ T1.ID = T2.ID\\ 
& \groupby\ T1.ID) \as\ RelevantView\\
&\when\  g(A_l)\  Then\\
&\update(A_c)= c\\
&\outputw\ Agg2(\post(B))\\
&\forw\ \pre(A_j)=a_j~\and\
\post(A_i) = a_i 
%~\and\\
%&\groupby&\  \pre(A_k), \post(A_p)
\end{align*}
and $f(Q,D,I)=Agg(\{t'.B \mid t'\in I, t\in Pre(Q,I), t'.ID=t.ID, t' \in Post(Q,I)\})$. 
If $Agg$ is a decomposable function, i.e., there exist  functions $g$ and $f'$ according to Definition~\ref{def:decomposable}, 
% then the expected output of the query $Q(D) = g\left(\left\{\expectation_{B' \in \overline{PWD}_{B''}}[f'(Q, D, B')] \forall B''\in \mathcal{B}_D\right\}\right)$.
then $Q(D) = g(\{Q'(B'') \mid \forall B''\in \mathcal{B}\})$, 
where $Q'$ is the same query as $Q$ with $f'$ replacing $f$ and $Q'(B'') = \expectation_{B' \in \overline{PWD}_{B''}}[f'(Q, D, B')]$.
\label{lem:general}
\end{proposition}

We leverage the following properties in the proof of the above proposition, when given a database $D$ with a block partition $\mathcal{B}=\{B_1,\cdots,B_l\}$, and a what-if query, $Q$, with a set of updates $U$:
\begin{enumerate}
    \item $\sum_{I\in PWD(Q,D)} \Pr_{D,U}(I) = 1$ and $\sum_{I'\in PWD(Q,B_i)} \Pr_{D,U}(I') = 1$, i.e., the sum of probabilities for all possible worlds of a database or a block is 1.
    \item $PWD(Q,D) = \times_{i=1}^l \overline{PWD}(Q,B_i)$, where $\overline{PWD}(Q,B_i) = \{I\cap B_i,~\forall I\in PWD(Q,B_i)\}$  and $I\cap B_i = \{t \mid t\in I, t.ID=t'.ID \text{ for some }t'\in B\}$. I.e., $PWD(Q,D)$ is equal to the Cartesian product of $\overline{PWD}(Q,B_i), \forall B_i\in \mathcal{B}_D$, where $\overline{PWD}(Q,B_i)$ contains all instances from $PWD(Q,B_i)$ restricted to tuples in $B_i$.
    % \item Consider a partitioning of $D$ into blocks $\mathcal{B}_D=\{B_1,\cdots,B_l\}$. 
    % $PWD$ is equal to the Cartesian product of $\overline{PWD}_{B_i}, \forall B_i\in \mathcal{B}_D$, where $\overline{PWD}_{B_i}$ contains all instances from $PWD_{B_i}$ restricted to tuples in $B_i$. Mathematically, $\overline{PWD}_B = \{I\cap B,~\forall I\in PWD_B\}$  where $I\cap B = \{t: t\in I, t.ID=t'.ID \text{ for some }t'\in B\}$.
    \item If the tuples in different blocks of the database are independent, then $\Pr_{D,U}(I) = \prod\limits_{I'\in PWD(Q,B_i), \forall B_i\in \mathcal{B}} \Pr_{D,U}(I') $
\end{enumerate} 



\begin{example}\label{ex:prop-blocks}
Continuing Example \ref{ex:decomposable}, for the what-if query $Q$ in Figure \ref{fig:query}. Suppose the database can be partitioned into blocks by Category as demonstrated in Example \ref{ex:blocks}. 
$Q(D)$ is then defined as the sum of the results of queries $Q'$ over each block $B$, where the aggregate function in $Q'$ for block $B$ is defined as $\frac{|B_i|}{|D|} \avg(\{t'.Price \mid t'\in I, t.Category = Laptop, t'.ID=t.ID\})$. 
\end{example}



The next proposition defines the link between a what-if query answer and causal inference. 

% \begin{proposition}
% Given a what-if query $Q$ with a $\select$ clause on $\maxi/\mini Agg(\post(A_T))$, and a database $D$ partitioned into blocks $\mathcal{B} = \{B_1, \ldots, B_l\}$. 
% Assume that $Agg(\post(D.A_T))$ can be decomposed into $\sum_{B_i \in \mathcal{B}}Agg'(B_i)$, then $Q(D) = $ \amir{continue}.
% \end{proposition}

\begin{proposition}\label{prop:causal-results}
Given a database $D$, a PCM $P$, and the what-if query $Q$ \amir{change $Agg(*)$ to $Agg(\post(B))$?}:
\begin{align*}
&\when\ g(A_l)\  Then\\
&\update A_c\ BY\ f(A_c)\\
&\select\ Agg(*)\\
&\where\  \pre(A_j)=a_j~ \and\
\post(A_i) = a_i 
\end{align*}
the following holds:
\begin{itemize}
    \item If $Agg = \ct$, $Q(D) =  |D| \pr(A_i=a_i|A_c = f(A_c), A_j=a_j, g(A_j)) + \sum_{t\in D}\mathbbm{1}\{t.A_j=a_j, t\notin g(D.A_j), t.A_i=a_i\}$
    \item If $Agg = \sumsql$, \amir{continue}
    % $Q(D) =  \expectation(A_i=a_i|A_c = f(A_c), A_j=a_j, g(A_j)) + \expectation_{t\in D}\mathbbm{1}\{t.A_j=a_j, t\notin g(D.A_j), t.A_i=a_i\}$
    \item If $Agg = \avg$, \amir{continue}
    \item If $Agg = \minsql$, \amir{continue}
\end{itemize}
\end{proposition}


For simplicity, Propositions \ref{prop:blocks} and \ref{prop:causal-results} do not consider a $\groupby$ clause and an intervention over multiple disconnected attributes, but it can easily be extended to include these. 

After establishing the connection between what-if query results to causal inference, any causal inference approach can be employed (e.g., regression \cite{?} and matching \cite{?}) to get the probability estimations, and thus the query results. 

% We now describe the algorithm for computing the result of a what-if query. \amir{describe the algorithm and connect to causal inference.}

% \begin{algorithm}[]
% 	\SetKwFunction{Evaluate What-if Query}{Evaluate What-if Query}
% 	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% 	\LinesNumbered
% 	\Input{What-if query $Q$, database $D$ with block partition $B_1, \ldots, B_l$}
%     \Output{$Q(D)$}
% 	\BlankLine
% 	Find $f'$ such that $f(Q,D,I) = g(f'(Q,D,B_1), \ldots, f'(Q,D,B_l))$\;
% 	$res \gets 0$\;
% 	\For{$B_i \in \mathcal{B}$}
% 	{
% 	   % $\expectation_{B' \in \overline{PWD}(Q,B_i)}[f(Q, D, B')] \gets$ \amir{connect to causal inference}\;
% 	   $sum_{u \in \dom(Backdoor(A_{c1}, A_{c2}))} \pr(B_{A_{c1}, A_{c2} \gets f_1(A_{c1}), f_2(A_{c2})}(u)) \pr(u \mid \post \amir{ conditions})$\;
% 	    $res \gets res + \expectation_{B' \in \overline{PWD}(Q,B_i)}[f(Q, D, B')]$\;
% 	}
% 	\Return $res$\;\label{l:return}
% 	\caption{Evaluate What-if Query} 
% 	\label{algo:what-if}
% \end{algorithm}



==> amazon_example.tex <==

\begin{figure}[h]
    % \vspace{-2mm}
    \centering
	\begin{footnotesize}
% 		\begin{subfigure}{1\linewidth}
% 		\centering
%         \begin{tabular}{ |c|c|c|c|c|c|c|c| } 
%          \hline
%          \rowcolor{lightgray}
%          PID  & Category & Price &  Sales Rank & Brand & Color \\ 
%          \hline
%          1 &  Laptop & 999 &  4443 & Vaio & Silver\\ 
%          2 &  Laptop & 529 &  1122 & Asus & \\ 
%          3 &  Laptop & 599 &  62 & HP & Silver\\ 
%          4 &  DSLR Camera & 549  & 1 & Canon & Black\\ 
%          5 & Sci Fi eBooks & Fantasy & 15.99  & 137 & \\ 
%          \hline
%         \end{tabular}
%         \caption{Product}\label{tbl:amazondatabase}
% 		\end{subfigure}
%         \begin{subfigure}{1\linewidth}
%         \centering
% 		\begin{tabular}{ |c|c|c|c|c| } 
%          \hline
%          \rowcolor{lightgray}
%          PID & ReviewID & Sentiment & Rating & Helpfulness\\ 
%          \hline
%           1 & 1 & -0.95 & 2 & 0.67\\ 
%          2 & 2 & 0.7 & 4 & 0.5\\ 
%          2 &  3 & -0.2 & 1 & 0 \\
%          3 &  3 & 0.23 & 3 & 0 \\
%          3 &  5 & 0.95 & 5 & 0.95\\
%          4 &  5 & 0.7 & 4 & 0.34\\
%          5 &  5 & 0.6 & 4 & 0.2\\
%          5 &  5 & 0.7 & 5 & 0.4\\
%          \hline
%         \end{tabular}
%         \caption{Review}\label{tbl:amazonreview}
% 		\end{subfigure}
    \begin{subfigure}{1\linewidth}
		\centering
        \begin{tabular}{c|c|c|c|c|c|c|c| } 
         \cline{2-7} 
        %  \rowcolor{lightgray}
         & \cellcolor[HTML]{C0C0C0} PID  & \cellcolor[HTML]{C0C0C0} Category & \cellcolor[HTML]{C0C0C0} Price &  \cellcolor[HTML]{C0C0C0} Brand & \cellcolor[HTML]{C0C0C0} Color & \cellcolor[HTML]{C0C0C0} Quality\\ 
         \hline
         $p_1$ & 1 &  Laptop & 999 & Vaio & Silver & 0.7\\ 
         $p_2$ & 2 &  Laptop & 529 & Asus &  & 0.65 \\ 
         $p_3$ & 3 &  Laptop & 599 & HP & Silver & 0.5 \\ 
         $p_4$ & 4 &  DSLR Camera  & 549 & Canon & Black & 0.75\\ 
         $p_5$ & 5 & Sci Fi eBooks & 15.99  & & & 0.4 \\ 
         \hline
        \end{tabular}
        \caption{Product}\label{tbl:amazondatabase}
		\end{subfigure}
    \begin{subfigure}{1\linewidth}
        \centering
		\begin{tabular}{ c|c|c|c|c| } 
        %  \hline
        %  \rowcolor{lightgray}
        \cline{2-5}
         & \cellcolor[HTML]{C0C0C0} PID & \cellcolor[HTML]{C0C0C0} ReviewID & \cellcolor[HTML]{C0C0C0} Sentiment & \cellcolor[HTML]{C0C0C0} Rating\\ 
         \hline
         $r_1$ & 1 & 1 & -0.95 & 2\\ 
         $r_2$ & 2 & 2 & 0.7 & 4\\ 
         $r_3$ & 2 &  3 & -0.2 & 1 \\
         $r_4$ & 3 &  3 & 0.23 & 3 \\
         $r_5$ & 3 &  5 & 0.95 & 5 \\
         $r_6$ & 4 &  5 & 0.7 & 4 \\
        %  $r_7$ & 5 &  5 & 0.6 & 4 \\
        %  $r_8$ & 5 &  5 & 0.7 & 5 \\
         \hline
        \end{tabular}
        \caption{Review}\label{tbl:amazonreview}
		\end{subfigure}
	\end{footnotesize}
	\caption{Amazon product database}\label{fig:database}
	\vspace{-2mm}
\end{figure}

% \begin{table*}[]
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c|c| } 
%  \hline
%  PID  & Category & Price &  Sales Rank & Brand & Color \\ 
%  \hline
%  1 &  Electronics$\rightarrow$ Laptop & 999 &  4443 & Vaio & Silver\\ 
%  2 &  Electronics$\rightarrow$ Laptop & 529 &  1122 & Asus & \\ 
%  3 &  Electronics$\rightarrow$ Laptop & 599 &  62 & HP & Silver\\ 
%  4 &  Electronics$\rightarrow$ DSLR Camera & 549  & 1 & Canon & Black\\ 
%  5 &  Kindle eBooks$\rightarrow$ Science Fiction \& Fantasy & 15.99  & 137 &  & \\ 
%  \hline
% \end{tabular}
% \end{center}
% \caption{Product database}\label{tbl:amazondatabase}
% \end{table*}

% \begin{table}[]
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c| } 
%  \hline
%  PID & ReviewID & Sentiment & Rating & Helpfulness\\ 
%  \hline
%   1 & 1 & -0.95 & 2 & 0.67\\ 
%  2 & 2 & 0.7 & 4 & 0.5\\ 
%  2 &  3 & -0.2 & 1 & 0 \\
%  3 &  3 & 0.23 & 3 & 0 \\
%  3 &  5 & 0.95 & 5 & 0.95\\
%  4 &  5 & 0.7 & 4 & 0.34\\
%  5 &  5 & 0.6 & 4 & 0.2\\
%  5 &  5 & 0.7 & 5 & 0.4\\
%  \hline
% \end{tabular}
% \end{center}
% \caption{Amazon Review database}\label{tbl:amazonreview}
% \end{table}

\begin{figure}[t]
    \centering
\begin{tikzpicture}[scale=0.7]
\begin{scope}[every node/.style={shape=rectangle, rounded corners,thick,draw,, top color=white, bottom color=blue!25}, 
other/.style={shape=rectangle, rounded corners,thick,draw,, top color=white, bottom color=red!25}]
    \node (Q) at (2.7,5.5) {\small Quality};
    \node (A) at (-.3,4) {\small Category};
    \node (B) at (0,5.5) {\small Brand};
    \node (K) at (4,4) {\small Color};
    \node (C) at (6.2,4) {\small Price};
    \node (F) at (3,3) {\small Rating};
    \node (G) at (1,2) {\small Sentiment};
    \node[other] (P) at (6,2.5) {\small Price};
    % \node (H) at (3,1) {\small Helpfulness};
    % \node (M) at (-3.5,3) {9};
\end{scope}

\begin{scope}[>={Stealth[black]},
            %   every node/.style={fill=white,circle},
              every edge/.style={draw=black, thick}]
    \path [->] (A) edge node {} (F);
    \path [->] (B) edge node {} (F);
    \path [->] (K) edge node {} (F);
    \path [->] (C) edge node {} (F);
    \path [->] (A) edge node {} (G);
    \path [->] (F) edge node {} (G);
    \path [->] (B) edge node {} (K);
    \path [->] (B) edge node {} (C);
    % \path [->] (G) edge node {} (H);
    \path [->] (B) edge node {} (A);
    
    \path [->] (Q) edge node {} (C);
    \path [->] (Q) edge node {} (F);
    \path [->] (B) edge node {} (Q);
    \path [->,bend right] (Q) edge node {} (G);
    
    \path [->,dashed] (P) edge node {} (F);
\end{scope}
\end{tikzpicture}
    \caption{A graph showing the dependencies between the attributes in the database in Figure \ref{fig:database}. Blue nodes are attributes of the same tuple and the red node is an attribute of a different tuple. A dashed edge denotes a dependency between attributes of different tuples}\label{fig:causal-graph}
\end{figure}




\begin{figure}
    \small
\begin{subfigure}{1\linewidth}
	\centering
    \begin{align*}
    &\when\ Brand = Asus\\
    &\intervene(Price)= 1.1 \times Price\\
    &\select\ \avg(Rating)~ \from\ Product~ 
    % \as\ T1~ 
    \sqland\ Review\\
    % ~ \as\ T2\\
    &\where\  \pre(Category) = Laptop 
    % ~\sqland\
    % T1.PID=T2.PID
    % \post(Brand) = Asus
    \end{align*}
    \caption{What-if query asking ``would increasing price of Asus laptops by 10\% affect their rating?''}\label{fig:query}
\end{subfigure}
\begin{subfigure}{1\linewidth}
    \centering
    \begin{align*}
    &\howto\ \intervene\ Sentiment\\
    &\suchthat\ -1 \leq Sentiment \leq 1, Cost(Sentiment) < 1\\
    &\toh\ \maxi\ \avg(\post(Price))\\
    &\when\ Category = Laptop\\
    &\where\  \pre(Category) = Laptop 
    % \sqland\
    % Product.PID=Review.PID
    \end{align*}
    \caption{How-to query asking ``how to maximize the average price of laptops by only changing the sentiment of the reviews of laptops so that they will be between -1 and 1 and closest to their original values?''}\label{fig:howto-query}
    \end{subfigure}
\caption{Causal what-if and how-to queries on the database in Figure \ref{fig:database}}\label{fig:queries}
\end{figure}

\begin{example}
Consider a simplified version of the Amazon product database \cite{HeM16} shown in Figure \ref{fig:database} describing product details and product reviews. Each tuple has a unique tuple identifier next to it for clarity. 
Also consider the query in Figure \ref{fig:query} stating intuitively ``what would be the effect of increasing the price of Asus laptops by 10\% on their ratings?''. 
Previous work \cite{DeutchIMT13,Nguyen0WZYTS18,DeutchMT15} would mechanically change the price values in Table \ref{tbl:amazondatabase} and re-evaluate the query, or perform view maintenance to update the results. 
However, in realistic scenarios, we know that changing the Price of a laptop product may affect other attributes of that product and may also affect other products. 
To account for such complex interactions, we can use the causal model whose intuitive representation is shown as a DAG in Figure \ref{fig:causal-graph}. 
For example, changing the Price of a laptop may affect its Rating since it is now a better deal (denoted as the edge from the blue Price node to the blue Rating node in Figure \ref{fig:causal-graph}). 
Furthermore, increasing the Price of Asus laptops may affect the Rating of Vaio laptops and vice versa (denoted as the edge from the red Price node to the blue Rating node  in Figure \ref{fig:causal-graph}). 
In general, a directed edge stands for an affect of the outbound node on the inbound node, e.g., Price affects Rating. 
% The node Quality has a dashed boundary since it is a hidden confounder that is not explicitly present in the database (we will address its inclusion in the graph in the sequel). 
\babak{I assume the example will be revised after the introduction is wrriten. It is not compeling as it is. I would suggest the following structure for the exmpale: (1) describe the data, (2) argue that the such dara provides us with a chance to answer several what-if and how-to questions that are importanty for bussiness, (3) compe up with a couple of intersting what-if and how-to queries and explain why they are important for optimising bussiness operations, (4)  describe how these queries can be cpatured using our system ..., (5) dicuss the novelty of our apporach which is accounting for the underling probablistic causal depedancies and compare with the existing work. Item (5) should be dicussed within the context of the exmaple.}
\end{example}

==> experimentsold.tex <==
\section{experiments}\label{sec:experiments}
We evaluate the effectiveness of \sys\ on various real-world and synthetic datasets and answer the following questions: 
\begin{compactenum}
    \item Do the results provided by \sys\ make sense in real-world scenarios?
    \item How does \sys\ compare to other baselines for hypothetical reasoning when the ground truth is available? 
    % Is the output provided by \sys\ accurate whenever ground truth is available?
    \item How does the runtime of \sys\ depend on query complexity and dataset properties like number of tuples, the causal graph structure, \common{discretization of continuous attributes, and the number of attributes in different operators of the query}?
    \item \common{How does combining a sampling approach with \sys\ influences runtime performance and the quality of the results?}
\end{compactenum}
% \textbf{Q1:} How flexible is \sys's syntax to capture different types of hypothetical updates? How do \sys's insights relate to the intuitions from existing literature?  \textbf{Q2:} How does \sys\ compare to prior techniques for reasoning about hypothetical updates? Is \sys's output accurate whenever ground truth is available? \textbf{Q3:} How does the efficiency of \sys\ depend on query complexity and dataset properties like number of records, causal graph structure and update complexity?
Our experimental study includes 5 datasets and 3 baselines that are either inspired by previous approaches or simulate the absence of a causal model. 
We provide a qualitative and quantitative evaluation of \sys, showing that it gives logical results in real-world scenarios and achieves interactive performance in most cases. 

\paratitle{\revb{Implementation} and setup} We implemented the algorithms in Python. \sys\ was run on a MacOS laptop with 16GB RAM and 2.3 GHz Dual-Core Intel Core i5 processor. We used random forest regressor~\cite{randomforest} to estimate conditional probabilities.

\subsection{Datasets and Baselines}
We give a short description of the datasets and baselines used in this section. 

\paratitle{Datasets} The following datasets and causal models were used.
% We consider the following datasets.
%along a a causal model we build for each one %\amir{verify. In the bullets, specify for each one how was the causal model obtained and describe it shortly}. 
\begin{itemize}
    \item The {\bf Adult} income dataset \cite{Adult} comprises demographic information of individuals along with their education, occupation, hours of work, annual income, etc. It is composed of a single table. We used the causal graph from prior studies~\cite{chiappa2019path}. 
    % In the DAG, the demographic attributes like gender, race and country are root nodes that affect all other attributes. 
    \item {\bf German} dataset \cite{Dua2019} contains details of bank account holders including demographic and financial information along with their credit risk. It composed of a single table and the causal graph was used from~\cite{chiappa2019path}.
    \item {\bf Amazon} dataset \cite{HeM16} is a relational database consisting of two types of tables, as described in Figure~\ref{fig:database}, and the causal graph is presented in Figure \ref{fig:causal-graph}. We identified product brand from their description, used Spacy~\cite{spacy} for sentiment analysis of reviews and estimated quality score from expert blogs~\cite{pcmag}. %The causal graph in Figure \ref{fig:causal-graph} was used for this dataset. 
    \item {\bf German-Syn} is a synthetically generated dataset using the same causal graph as \texttt{German} dataset~\cite{Dua2019}. It consists of a single table. \reva{We consider two different versions for our analysis, one with {20K records} and the other with {1 million} records.}
    \item {\bf Student-Syn} dataset contains two different tables (a) Student information consisting of their age, gender, country of origin and their attendance. (b) Student participation attributes like discussion points, assignment scores, announcements read and overall grade. Each student was considered to enroll in $5$ different courses and their overall grade is an average over respective courses. This data was generated keeping in mind the effect of attendance on class discussions, announcements and grade. The causal model has student age, gender and country of origin as the root nodes, which affect their attendance and other performance related attributes. 
    %\item Datasets:Adult, Amazon, Spotify?, (Academic, patent), MAS academic, synthetic data
    %\item Scraping quality: from reviews - easier, from external websites - harder
    %\item Implementation: 
    %what-if done by Thursday (for blocks), how-to done by next week
    %\item Baselines: Caravan (what-if), Tiresias (how-to), Stochastic package builder (how-to), our approach when there is all attributes and tuples are independent
    %\item Queries: 4-5 queries for each dataset
    %\item Runtime v.s. baselines
    % \item Size of grounded causal graph
    %\item Compare solutions with baselines (synthetic database where Tiresias messes up)
\end{itemize}
%\include{student_causal_graph}
\paratitle{Variations and baselines}
In the experiments, \sys\ is run assuming that background knowledge about the causal graph is known a priori. 
We consider one variation where the causal model is not available (denoted by \sys-NB), \common{and another where we perform sampling for training the regressor (denoted \sys{}-sampled),} and  two different baselines of \sys\ to evaluate hypothetical queries: 
\begin{itemize}
    \item {\bf \sys-NB:} when no causal model is available, all attributes are assumed to affect the updated attribute and the output.
    \item \reva{{\bf \sys{}-sampled:} is an optimized version of \sys{}  that considers a randomly chosen subset of $100$k records for the calculation of conditional probabilities of Proposition~\ref{prop:causal-results}. The choice of sample size is discussed in Section~\ref{sec:sol_quality}}
    \item {\bf Indep:} baseline inspired by previous work on provenance updates \cite{DeutchIMT13}: this approach ignores the causal graph and assumes that there is no dependency between different attributes and tuples.
    \item {\bf Opt-HowTo:} baseline for how-to analysis where we compute the optimal solution by enumerating all possible updates, evaluating what-if query output for each update and choosing the one that returns the optimal result.
   
\end{itemize}

% \subsection{Setup and Baselines} We implemented the algorithms in Python and used causal graph for Adult and German datasets from~\cite{}. All codes were run on a MacOS laptop with 16GB RAM and 2.3 GHz Dual-Core Intel Core i5 processor.   The causal graph for Amazon is same as the one discussed in Figure~\ref{fig:database}. We used random forest regressor~\cite{} to estimate conditional probabilities.

% \noindent \textbf{Baselines.} We consider two different variations of \sys to evaluate query output. i) \sys\ is run assuming that background knowledge about the causal graph is known aprior and ii) \sys-NB assumes that there is no background knowledge. In this case, all attributes are assumed to be common confounders of the updated attribute and the output variable. We consider a baseline Indep, which ignores the causal graph and assumes that there is no dependence between different attributes. \sg{inspired by previous models that do probabilistic updates without capturing dependance}

% For how-to analysis, we consider an optimal baseline that enumerates all possible updates, evaluates what-if query output for each update and chooses the one that returns the optimal result.

\subsection{What-If Real World Use Cases}

\begin{figure}[t]
    \centering \small
\begin{subfigure}{\linewidth}
	\centering
    % \begin{align*}
    % %&\when\ Brand = Asus\\
    % &\update(X)= x\\
    % &\select\ \ct(Credit=Good)\\
    % &\from\ D\\
    % &\where\  \pre(X_2) = x_2\\
    % \end{align*}
\begin{align*}
    %&\when\ Brand = Asus\\
        \use\ D~~
        \update(B)= b~~
        \outputw\ \ct(Credit=Good)~~
        \forw\ \pre(A) = a
    \end{align*}
 \cut{
    \begin{align*}
    %&\when\ Brand = Asus\\
        & \use\ D\\
        &\update(B)= b\\
        &\outputw\ \ct(Credit=Good)\\
        &\forw\ \pre(X_2) = x_2
    \end{align*}
    }
    \vspace{-4mm}
    \caption{What-if query (German dataset): What fraction of individuals will have good credit if $B$ is updated to $b$?}\label{fig:whatif:endtoend}
\end{subfigure}
\begin{subfigure}{\linewidth}
	\centering \small
	\vspace{-2mm}
    % \begin{align*}
    % %&\when\ Brand = Asus\\
    % &\update(X)= x\\
    % &\select\ \ct(Credit=Good)\\
    % &\from\ D\\
    % &\where\  \pre(X_2) = x_2\\
    % \end{align*}
    \begin{align*}
    %&\when\ Brand = Asus\\
       \use\ D \quad \quad
        \update(B)= b \quad \quad
        \outputw\ \ct(*) \\
        \forw\   \post(Income)>50k~  \sqland\ \pre(A) = a
    \cut{
        & \use\ D\\
        &\update(B)= b\\
        &\outputw\ \ct(*)\\
        &\forw\ \post(Income)>50k~ \sqland\ \pre(a)A= a
        }
    \end{align*}
    \vspace{-5mm}
    \caption{What-if query (Adult dataset): How many individuals with attribute $A=a$ will have income $\geq 50K$ if $B$ is updated to $b$?}\label{fig:whatif:adult}
\end{subfigure}
\caption{What-if queries for real world use cases}\label{fig:real-world-queries}
%\vspace{-5mm}
\end{figure}
{
\begin{table}[t] \centering \small
\vspace{-2mm}
\caption{\textmd{Average Runtime in seconds for $\ct$ query to evaluate the effect of a hypothetical update on target for what-if queries. \reva{The time in (..) in the last row is by \sys(-NB)-sampled, which takes the same time as \sys(-NB)\ on all other datasets with $<100k$ tuples.}%{\color{red} (1) for what-if? (2) can you add a column for \sys-sampled?}
}
%\vspace{-3mm}
}
	\label{tbl:data}
	{\footnotesize
		\begin{tabular}{@{}lrrrrrrrrr@{}}\toprule
			{Dataset} & {Att. [$\#$]} & {Rows[$\#$]} &  \sys & \sys-NB &  Indep   \\ \midrule
			\textbf{Adult}~\cite{Adult} & 15 & 32k & 45s  &105s & 3s&  \\ 
			\textbf{German}~\cite{Dua2019}& 21  & 1k & 1.2s & 12.5s&0.4s & \\ 
		    {\textbf{Amazon}}~\cite{HeM16}& {5,3} &{3k, 55k}  & 1.7s & 10.5s&0.8s & \\ 
		   \textbf{Student-syn}& 3,6  & 10k,50k & 4.5s  &12.3s & 1.2s & \\
		   
		   \reva{\textbf{German-Syn} (20k)}& 6  & 20k & 7.2s & 22.45s & 1.4s & \\ 
			
		\reva{\textbf{German-Syn} (1M)}& \reva{6}  & \reva{1M} & \reva{390s (44.5s)} & \reva{1173s (132s)} & \reva{73s} & 
		\end{tabular}
		}
		\vspace{-4mm}
	
\end{table}
}



\begin{figure}
    \centering
    \subcaptionbox{\texttt{German} \label{fig:exp:germanreal}}{
    \includegraphics[width=0.47\columnwidth]{plots/german_real.pdf}}
     \subcaptionbox{\texttt{Adult} \label{fig:exp:adultreal}}{
    \includegraphics[width=0.47\columnwidth]{plots/adult_real.pdf}}
    \caption{What-if query output for \texttt{German} and \texttt{Adult} datasets on updating each attribute to their min and max values; a larger gap %in the two values 
    denotes higher attribute importance. %for the outcome. 
    }
    \label{fig:real}
    \vspace{-5mm}
\end{figure}
In this experiment, we evaluate the output of \sys\  on a diverse of hypothetical queries on various real-world datasets. Due to the absence of ground-truth, we discuss the coherence of our observations with intuitions from existing literature.

\paratitle{German} We considered a hypothetical update of fixing attributes `Status', `Credit history', and `housing' to their respective minimum and maximum values to evaluate the effect of these attributes on individual credit. Figure~\ref{fig:whatif:endtoend} demonstrates the query template where $X,x, X_2,x_2$ are varied to evaluate the effect of different updates. Whenever status or credit history are updated to the maximum value, more than $81\%$ of the individuals have good credit. Similarly, updating these attributes to the minimum value reduces the credit rating of more than $30\%$ individuals. 
On the other hand, updating other attributes like `housing' and `investment' affects the credit score of less than $20\%$ individuals. Figure~\ref{fig:exp:germanreal} presents the effect of updating these attributes to their minimum and maximum value. Larger gap in the query output for Status and credit history shows that these attributes have a higher impact on credit score.
We also tested the effect of updating pairs of attributes and observed that {\bf updating `credit history' and `status' at the same time can affect the credit score of more than $70\%$ individuals.}
These observations are consistent with our intuitions that credit history and account status have the maximum impact of individual credit. 

\paratitle{Adult} This dataset has been widely studied in the fairness literature to understand the impact of individual's gender on their income. It has a peculiar inconsistency where married individuals report total household income demonstrating a strong causal impact of marital status on their income \cite{DBLP:conf/sigmod/SalimiGS18,TAGH+17,10.1109/ICDM.2011.72}. We ran a hypothetical what-if query to analyze the fraction of high-income individuals when everyone is married (Figure~\ref{fig:whatif:adult}). We observed that $38\%$ of the individuals have more than $50$K salary. Similarly, {\bf if all individuals were unmarried or divorced, less than $9\%$ individuals have salary more than $50$K}. This wide gap in the fraction of high-income individuals for two different updates of marital status demonstrate its importance to predict household income. Figure~\ref{fig:exp:adultreal} shows the effect of updating the attributes with the minimum or the maximum value in their domain.
Additionally, updating class of all individuals has a smaller impact on the fraction with higher income. These observations match the observations of existing literature~\cite{GalhotraPS21}, where marital status, occupation and education have the highest influence on income.



\paratitle{Amazon} We evaluated the effect of changing price of products of different brands on their rating.  When all products have price more than the $80^{th}$ percentile, around $32\%$ of the products have average rating of more than $4$. {\bf On further reducing the laptop prices to $60^{th}$ and $40^{th}$ percentiles, more than $60\%$ of the products get an average rating of more than $4$}. This shows that reducing laptop price increases average product ratings. Among different brands, we observed that Apple laptops have the maximum increase in rating on reducing laptop prices, followed by Dell, Toshiba, Acer and Asus. These observations are consistent with previous studies on laptop brands~\cite{amazonstudy}, which mention Apple as the top-quality brand in terms of quality, customer support, design, and innovation.%The chances of getting a perfect rating do not improve when the price of Asus laptops is reduced more than $20\%$. These 

\vspace{-2mm}
\subsection{Solution Quality Comparison}\label{sec:sol_quality}
In this experiment, we analyzed the quality of the solution generated by \sys\ with respect to the ground truth and baselines over synthetic datasets. The ground truth values are calculated using the structural equations of the 
causal DAG for the synthetic data. %\amir{I suggest seperating by what-of and how-to and not by dataset}

% \paragraph{What-If}

% \paratitle{German-Syn} 
\paratitle{What-if}
For the \reva{German-Syn (1M)} dataset, Figure~\ref{fig:exp:germansyn} presents the output of a query that updates different attributes related to individual income and evaluates the probability of achieving good credit. For all attributes, \reva{\sys, \sys-sampled, and \sys-NB estimate the query output accurately with an error margin of less than $5\%$.}  In contrast, Indep baseline ignores the causal structure and relies on correlation between attributes to evaluate the output. Since, the individuals with high status are highly correlated with good credit, Indep incorrectly outputs that updating Status would automatically improve credit for most of the individuals.


% \paratitle{Student-Syn}
For the Student-Syn dataset, Figure~\ref{fig:exp:studentsyn} presents the average grade of individuals on updating different attributes that are an indicator of their academic performance. In all cases, \sys\ and \sys-NB output is accurate while Indep is confused by correlation between attributes and outputs noisy results.
In addition to these hypothetical updates, we considered complex what-if queries that analyzed the effect of assignment and discussion attributes on individuals that read announcements and have high attendance. In these individuals, we observed that improving assignment score has the maximum effect on overall grade of individuals.

\begin{figure}
    \centering
    \subcaptionbox{Solution quality % vs. number of samples 
    \label{fig:exp:variance}}{
    \includegraphics[width=0.5\columnwidth]{plots/samplesize_variance.pdf}}
     \subcaptionbox{Running time 
     %vs. number of samples 
     \label{fig:exp:sampletime}}{
    \includegraphics[width=0.41\columnwidth]{plots/samplesizetime.pdf}}
    \caption{\reva{Effect of varying sample size on \sys{}-sampled output and running time for \texttt{German-Syn} (1M) dataset}}
    \label{fig:samplesize}
    \vspace{-5mm}
\end{figure}



\paratitle{\reva{Effect of Sample size}} \reva{Figure~\ref{fig:samplesize} compares the effect of changing the sample size on the quality of output generated (Figure~\ref{fig:exp:variance}) and running time (Figure~
\ref{fig:exp:sampletime}) by \sys{}-sampled. Figure~\ref{fig:exp:variance} shows that the standard deviation in query output of \sys-sampled reduces with an increase in sample size and is within $1\%$ of the mean whenever more than $100k$ samples are considered. In terms of running time, we observe a linear increase in time taken to calculate query output. Due to low variance of \sys{}-sampled for $100k$ samples and reasonable running time, we consider 100k as the sample-size for subsequent analysis. }
% \paragraph{How-to}

% \paratitle{German-Syn} 
\paratitle{How-to}
For the \reva{German-Syn (20k)} dataset, we considered a how-to query that aims to maximize the fraction of individuals receiving good credit. We provided Status, Savings, Housing and Credit amount as the set of attributes in the \howto\ operator. \revb{\sys\ returned that updating two attributes i)  account status, and ii) housing attributes is sufficient to achieve good credit. This showed that updating a single attribute would not maximize the fraction of individuals with good credit. We evaluated the ground truth (Opt-HowTo) by enumerating all possible update queries  and  used the structural equations of the causal graph to evaluate the post-update value of the objective function for each update. We identified that \sys's output matches the ground truth update. }

% \paratitle{Student-Syn} 
For the Student-Syn dataset, we evaluated a how-to query to maximize average grades of individuals with a budget of updating atmost one attribute. \sys\ returned that improving individual attendance provide the maximum benefit in average grades.
This output is consistent with ground truth calculated by evaluating the effect of all possible updates (Opt-HowTo). %\sys takes less than $7$ seconds to identify the solution while Opt-HowTo requires 
%$2.42$min. 
% $2$min $25$sec.





\paratitle{\revc{Effect of discretization}}
\revc{\sys{} bucketizes all continuous attributes before solving the integer program. In this experiment, we evaluate the effect of number of buckets on the solution quality and running time on a modified version of \texttt{German-Syn} (20k) dataset that contains continuous attributes.  We partitioned the dataset into equi-width buckets and compared the solution returned by 
\sys{} and the optimal solution calculated after discretization (Opt-discrete) with the ground truth solution (OptHowTo). Figure~\ref{fig:exp:bucketquality} compares the quality of \sys{} and Opt-discrete as a ratio of the optimal value. We observe that the solution quality improves with the increase in the number of buckets and the returned solution is within $10\%$ of the optimal value whenever we consider more than $4$ buckets. The solution returned by Opt-discrete is similar to that of \sys{}. The time taken by Opt-discrete increases exponentially with the number of buckets. In contrast, time taken by \sys{} does not increase considerably as the number of variables in the integer program depends linearly on the number of buckets. This shows that running \sys{} over a bucketized version of the dataset leads to competitive quality in reasonable amount of time.
}
\begin{figure}
    \centering
    \subcaptionbox{Solution quality % vs. number of buckets 
    \label{fig:exp:bucketquality}}{
    \includegraphics[width=0.45\columnwidth]{plots/howto_bucket.pdf}}
     \subcaptionbox{Running time% vs. number of buckets 
     \label{fig:exp:buckettime}}{
    \includegraphics[width=0.45\columnwidth]{plots/howto_buckettime.pdf}}
    \vspace{-0.5mm}
    \caption{\revc{How-to Query output for \texttt{German-Syn (20k)} with varying number of buckets.}}
    \label{fig:buckettradeof}
    \vspace{-5mm}
\end{figure}

\begin{figure}
    \centering
    \subcaptionbox{\reva{\texttt{German-Syn (1M)}} \label{fig:exp:germansyn}}{
    \includegraphics[width=0.45\columnwidth]{plots/correctness_german.pdf}}
     \subcaptionbox{\texttt{Students-Syn} \label{fig:exp:studentsyn}}{
    \includegraphics[width=0.45\columnwidth]{plots/correctness_student.pdf}}
    \caption{\reva{What-If Query output.% for \texttt{German-Syn} (1M) and \texttt{Student-Syn} datasets
    }}
    \label{fig:corr}
    \vspace{-5.5mm}
\end{figure}

\subsection{Runtime Analysis and Comparison}\label{subsec:runtime}
In this section, we evaluate the effect of different facets of the input on the runtime of \sys. \reva{Note that our approach comprises two steps: (a) creating the aggregate view on which the query should be computed (done using a join-aggregate query), and (b) training regression functions to calculate conditional probability in the calculation of query output (the mathematical expression is in Proposition~\ref{prop:causal-results}). This training is performed over a subset of the attributes of the view computed in the previous step. 
Training a regression function is more time-consuming than computing the aggregate view in step (1). Therefore, \sys{} is as scalable as prior techniques for regression (we use a random forest regressor from the sklearn package).  Hence the parameters we consider } include (1) database size, (2) backdoor set size (see Section \ref{sec:whatif-algo}), and (3) query complexity.
Since the effect of (1), (2) on the runtime of what-if query evaluation is directly translated to an effect on the runtime of how-to query evaluation, for how-to queries, we focus on the effect of the number of attributes in the $\howto$ operator which will change the optimization function $\phi$ (see Section \ref{sec:howto-algo}). We use the synthetic datasets \texttt{German-Syn} and \texttt{Student-Syn}. 

\paratitle{What-if: database size} Table~\ref{tbl:data} presents the average running time to evaluate the response to a what-if query in seconds. \reva{To further evaluate the effect of database size on running time, we considered \texttt{German-Syn} dataset and varied the number of tuples from $10K$ to $1M$. In this experiment we consider a new variation of \sys{}, denoted by \sys-sampled, which considers a randomly chosen subset of $100K$ records for the calculation of conditional probabilities of Proposition~\ref{prop:causal-results}. Figure~\ref{fig:scalability} compares the average time taken by \sys{}, \sys{}-sampled with Indep for five different What-If queries and Opt-HowTo for How-to queries.
We observed a linear increase in running time with respect to the dataset size for all techniques except \sys{}-sampled.  The increase in running time is due to the time taken to train a regressor which is used to estimate conditional probabilities for query output calculation
% \footnote{\reva{To answer a what-if or how-to query,  aggregate view calculation requires less than $1\%$ of the total time. The majority of the time is spent on calculating the query output using the result in Proposition~\ref{prop:causal-results}} }. 
To answer a what-if (or how-to) queries,  aggregate view calculation requires less than $1\%$ of the total time. The majority of the time is spent on calculating the query output using the result in Proposition~\ref{prop:causal-results}.
Therefore, the time taken by \sys-sampled does not increase considerably when the dataset size is increased beyond 100K. 

}

\paratitle{What-if: backdoor set size} This experiment changed the background knowledge to increase the backdoor set from $2$ attributes to $6$ attributes. The running time to calculate expected fraction of high credit individuals on updating account status increased from $7.2$ seconds when backdoor set contains age and sex to $22.45$ seconds when the backdoor set contains all attributes. %We observe similar trends for How-to analysis.

\paratitle{What-if: query complexity} 
In this experiment, we synthetically add multiple attributes in the \texttt{Student-syn} dataset and the different operators of the query to estimate their on running time.

On adding multiple attributes in the \use\ operator, the time taken to compute the \augmentedtable\ increases minutely. For \texttt{Student-Syn}, \use\ operator was evaluated in less than $0.5$ seconds when $5$ different attributes are added from other datasets. The increase in these attributes do not affect the running time of subsequent steps unless the attributes in \forw\ operator increase.


We now compare the effect of adding multiple attributes in the \forw\  operator of a \ct{} query.  Adding conditions involving \pre\ value of randomly chosen attributes increases the number of attributes used to train the regressor, which increases the running time (Figure~\ref{fig:exp:timewhatif}).  Running time increased from $4.2$ seconds when \forw\  operator is empty to $12.1$ seconds and $17.7$ seconds when it contains $5$ and $10$ attributes, respectively. In contrast, Indep is more efficient as it does not use additional attributes to compute query output.
However, if the added attribute is in the backdoor set, then the output is evaluated faster. To understand the effect of adding such attributes, we considered a query where the backdoor set contained $10$ binary attributes. To evaluate the output, probability calculation iterated over the domain of backdoor attributes and required $49.7$ seconds. The running time reduced to $7.4$ seconds when $5$ conditions on these attributes are added to the \forw\ operator.

%Changing the aggregate in \outputw\ shows varied running time for \ct\ and \sumsql. For \ct, the query ran in less than $5$ seconds while for \sumsql, the query took around $40$ seconds. The increased running time for \sumsql\ is due to the evaluation of probability values for all values in the domain of $Y$ (output attribute).

\paratitle{How-to: query complexity} Figure~\ref{fig:exp:timehowto} presents the effect of the number of attributes in \howto\ operator on the time taken to process the query. Increasing attributes leads to a linear increase in the number of variables in the integer program.  Therefore, the time taken by \sys\ increases from $7$ seconds for $5$ attributes in \howto\ operator to $20$ seconds for $10$ attributes. In contrast, Opt-HowTo considers all possible combinations of attribute values in the domain of attributes in the \howto operator. It takes around $4$minutes for $5$ attributes and more than $90$ minutes for $10$ attributes. This shows that the Integer Program based optimization provides orders of magnitude improvement in running time.


\begin{figure}
    \centering
    \subcaptionbox{What-if (\forw\ operator)  \label{fig:exp:timewhatif}}{
    \includegraphics[width=0.45\columnwidth]{plots/whatiffor.pdf}}
     \subcaptionbox{How-to (\howto) \label{fig:exp:timehowto}}{
    \includegraphics[width=0.45\columnwidth]{plots/howtotime.pdf}}
    \caption{Running Time comparison on varying number of attributes in different operators for \texttt{Student-Syn} dataset.}
    \label{fig:corr:time}
    %\vspace{-2mm}
\end{figure}


\begin{figure}
    \centering
    \subcaptionbox{ What-if query  \label{fig:exp:scalabilitywhatif}}{
    \includegraphics[width=0.43\columnwidth]{plots/scalabilitywhatif.pdf}}
     \subcaptionbox{ How-to query \label{fig:exp:scalabilityhowto}}{
    \includegraphics[width=0.45\columnwidth]{plots/scalabilityhowto.pdf}}
    \caption{\reva{Running Time comparison on varying dataset size for \texttt{German-Syn} dataset averaged over five different queries.}}
    \label{fig:runtime-sample}
    \vspace{-5mm}%{\color{red} (1) the Y-axis title is cropped, (2) is this an average over what-if and how-to? how are they combined?}}
    \label{fig:scalability}
    %\vspace{-7mm}
\end{figure}
%\begin{enumerate}
%    \item Amazon-- real world
%    \item Hyper-All in fig 5
%    \item show different types of queries
%    \item How-to: ground truth should be a baseline
%    \item Effect of dataset size, backdoor set on performance
%    \item Effect of query complexity: cost of each clause
%    \item Effect of optimizations
%    \item non-linear causal equations
%\end{enumerate}
%pre-processing cost

%implementation and optimizations: Separate discussion


==> model.tex <==
\section{Model for Hypothetical Updates}\label{sec:model}
% We next review our model for probabilistic causal queries. 
Our model draws on ideas from probabilistic databases and causal inference. We first review basic database concepts and then define hypothetical updates, possible worlds, and causal models. 

\begin{table}[h]
\begin{small}
\centering
\caption{Notations}\label{tbl:notations}
\begin{tabular}{| c | c | c |}
\hline $D$ & Database instance\\
$PWD(D)$ & Possible worlds of $D$\\
$u$ & Hypothetical updates\\
$G$ & Causal DAG\\
$P$ & PCM based on $D$ and $G$\\
$\pr_{D,P,U}$ & Probability dist. over $PWD(D)$ defined by $D,P,U$\\
\hline
\end{tabular}
\end{small}
\end{table}


\begin{figure}[h]
    \centering
\begin{tikzpicture}[scale=0.7]
\begin{scope}[every node/.style={shape=rectangle, rounded corners,thick,draw, top color=white, bottom color=purple!25}]
    \node (A) at (-3,4) {Product};
    \node (B) at (2,4) {Review};
\end{scope}

\begin{scope}[>={Stealth[black]},
            %   every node/.style={fill=white,circle},
              every edge/.style={draw=black, thick}]
    \path [->] (A) edge node[above] {PID} (B);
\end{scope}
\end{tikzpicture}
    \caption{Schema graph}\label{fig:schema-graph}
\end{figure}


\paragraph{Schemas, databases, and aggregate queries.}
We focus in this paper on star schemas \cite{snowflake} where there is a central fact table connected by Foreign Key (FK) joins to the other tables called `dimensional tables'. 
The schema is associated with a directed graph, called a {\em schema graph}, whose nodes are the table names and there is a directed labeled edge between two table names if they have an FK join between them \cite{KalashnikovLS18}. We further assume that the label of each edge makes clear the FK attribute to join on. 
The restriction of star schemas will allow us to combine our model with causal inference on relational databases, while the schema graph allows our query syntax (which will be defined in Section \ref{sec:syntax}) to be simpler. 
% \babak{The restriction on star schema comes out the blue. Should we justify it?}


Let ${\mb A}=\{ID,A_1,\ldots,A_m\}$ denote the set of attributes and $\mathcal{R} (ID, A_2, \dots,$ $A_m)$
denote a relation schema over them. 
% \amir{do we still need ids if we have tuple identifiers?}. 
Then the set ${\DDom}^m=\Dom(ID)\times \Dom(A_1)\times \cdots\times \Dom(A_m)$ specifies the domain of all
possible tuples. A dataset $D\subseteq {\DDom}^m$ is a specific instance of the
schema $\mathcal{R}$. 
% We use $t \in\DDom^m$ to denote a tuple in the schema $\mathcal{R}$. 
We assume that $ID$ is an attribute denoting the unique ID of each one of the tuples in $D$. 
We use $A_i[t] \in \Dom(A_i)$ to denote the value of the attribute $A_i$ of the tuple $t$, and $A_j[D]$ to denote the entire column $\langle A_j[t_1], A_j[t_2], \dots, A_j[t_n]\rangle$, where $|D| = n$. We further associate each tuple with a unique identifier as demonstrated by the identifiers $p_i, r_j$ in Figure \ref{fig:database}.
% and use $D.A_j$ to denote the column $\langle t_1.A_j, t_1.A_j, \dots, t_n.A_j\rangle$ 
% where $|D| = n$ and $t_i$ denotes the tuples in $D$.

\babak{The above paragraphs should be moved to preliminaries.}

In the sequel, we define updates on certain attributes. To model the concept of attributes that can be updated and attributes that are constant, we split the attribute set into two subsets. 
Let ${\mb A}= {\mb A_{im}} \mathbin{\dot{\cup}} {\mb A_{mu}}$ where ${\mb A_{im}}$ denotes the immutable attributes and ${\mb A_{mu}}$ denotes the mutable attributes, ${\mb A_{im}} \cap {\mb A_{mu}} = \emptyset$. In particular, $ID \in {\mb A_{im}}$, i.e., the ID attribute of the tuples is considered immutable. 
% \babak{same comment as above applied to what comes next} \amir{I'm not sure if we should justify the model here since the readers do not yet have a full understanding of causality (this limitation stems from the need to summarize the attributes without changing the distribution)}

\babak{Do we need to talk about queries in this section? I think the purpuse of this section is to define hypothetical updates and their probablistic influence on the other attributes.}We also allow aggregate queries on top of our hypothetical queries. We use a standard form of aggregate query \cite{?}, namely:
\textsc{SELECT Agg($A_i$), $A_j$ FROM $D$ WHERE Cond GROUPBY $A_j$}, where \textsc{Agg}$ \in \{\ct,\sumsql,\avg,\minsql\}$ and \textsc{Cond} is a selection condition on the attributes of $D$. 

\begin{example}
The schema of the product table is depicted in Figure \ref{tbl:amazondatabase} is (PID, Category, Price, Brand, Color, Quality). 
Each tuple in Figure \ref{tbl:amazondatabase} has a unique id number (the first attribute) and each attribute has a domain. For example, $\Dom(Price) = [0,500K]$. 
The first tuple has $Category[p_1] = Laptop$ and $Price[p_1] = 999$ etc. 
The schema graph describing the link between that tables in Figure \ref{fig:database} is depicted in Figure~\ref{fig:schema-graph}. 
The mutable attributes are Price, Quality, Category, Color, Rating, and Sentiment. 
An example for an aggregate query on this database is:
\begin{align*}
% &\select\ \avg(Price)& \\
% &\where\  Category = Laptop ~\sqland\
% Price > 500
&\select\ \avg(Rating)~ \from\ Product~ 
\sqland\ Review\\
&\where\  \pre(Category) = Laptop
\end{align*}
\end{example}

\paragraph{Possible worlds and hypothetical updates}
% Our what-if and how-to queries will create a probabilistic database. 
Our what-if and how-to queries will create a probability space over all possible database instances that stem from the initial instance. 
Thus, we adapt the notion of possible worlds from the literature of probabilistic databases \cite{?} and define the set of possible worlds as the set of all instances with the same number of tuples that may contain different values in their attributes from the appropriate domains. 
% We next define the set of possible worlds for a database instance $D$
\begin{definition}\label{def:possible-worlds}
Given a database instance $D \subseteq {\DDom}^m$ with $n$ tuples, the set of possible worlds of $D$ is $PWD(D) = {\DDom}^m = \{(v_1,\cdots,v_m) ~|~ v_i\in A_i\}^n$.
We omit the subscript $D$ whenever it is clear from the context.
\end{definition}

Later in this section, we will associate a probability with each possible world. 

\begin{figure}[h]
\begin{center}
\begin{footnotesize}
\begin{tabular}{c|c|c|c|c|c|c|c| } 
 \cline{2-7}
%  \rowcolor{lightgray}
 & \cellcolor[HTML]{C0C0C0} PID  & \cellcolor[HTML]{C0C0C0} Category & \cellcolor[HTML]{C0C0C0} Price & \cellcolor[HTML]{C0C0C0} Brand & \cellcolor[HTML]{C0C0C0} Color & \cellcolor[HTML]{C0C0C0} Quality \\ 
 \hline
 $p_1$ & 1 &  Laptop & 999 & Vaio & Silver & 0.7\\ 
 $p_2$ & 2 &  Laptop & \cellcolor{blue!25}582 & Asus &  & 0.65\\ 
 $p_3$ & 3 &  Laptop & 599 & HP & Silver  & 0.5\\ 
 $p_4$ & 4 &  DSLR Camera & 549 & Canon & Black & 0.75\\ 
 $p_5$ & 5 &  Sci Fi eBooks & 15.99 & &  & 0.4\\ 
 \hline
\end{tabular}
\end{footnotesize}
\end{center}
\caption{Possible world of the table in Figure \ref{tbl:amazondatabase} which, along with the table in Figure \ref{tbl:amazonreview} is a possible world $I$ of the database shown in Figure \ref{fig:database}. The only change is in the price of $p_2$ (the blue cell) which is increased by 10\%}\label{tbl:possible-world}
\end{figure}

\begin{example}\label{ex:possible-world}
Reconsider the database table in Figure \ref{tbl:amazondatabase}. One possible world, $I$, of this database is the table shown in Figure \ref{tbl:possible-world} where the value of the $Price[p_2]$ was increased by 10\%, along with the table in Figure \ref{tbl:amazonreview}. This is a possible world since the tables share the same schema and the same number of tuples while there are differences in the values of the cells. 
% A possible world of $p_1$ (considering only Figure \ref{tbl:amazondatabase}) is the first tuple in Figure \ref{tbl:possible-world} and the second to fifth tuples shown in Figure \ref{tbl:amazondatabase}. 
\end{example}


Another component in our model is the hypothetical update to the database. 
Intuitively, a what-if query asks what would be the answer to some question if the database was hypothetically updated in a specific manner. We next model this update.

\begin{definition}\label{def:update}
Given a database $D$, a subset of tuples $S\subseteq D$, an attribute $A_{c} \in {\mb A_{mu}}$, and a function $f: \DDom(A_c) \to \DDom(A_c)$, a hypothetical update is a function $u: D \to \DDom(A_c)$ such that $\forall t_i \in S.~u(t_i) = f(A_c[t_i])$ and $\forall t_j \in D \setminus S.~u(t_j) = A_c[t_j]$. 
\end{definition}

\begin{example}\label{ex:update}
Consider the tuple $p_2$ in the database shown in Figure \ref{fig:database}. 
If we define $S = \{p_2\}$, $A_c = Price$, and $f(x) = 1.1\cdot x$, the hypothetical update to the database will be $u(p_2) = 582$, and $u(p_i) = Price[p_i]$, for all $i \neq 2$. 
If there is no dependency between attributes and tuples in the database, after the update, we will get the database $I$ that is composed of the table shown in Figure \ref{tbl:possible-world} (with only $Price[p_2]$ being changed) and the table in Figure \ref{tbl:amazonreview}. 
However, in many realistic scenarios, there is such a dependency and we next show a way to capture it using causality. 
\end{example}

% The probability of an instance $I \in PWD$ is defined by the PCM $P$ and denoted by $\Pr(I_{S.A_c \gets f(S.A_c)})$. 
% Note that if $I \in PWD$ contains $t_i \in I$ whose counterpart, $t_i'$ is in $S$ such that $t_i.A_c \neq f(t_i.A_c)$, then $\Pr(I_{A_c \gets f(A_c)}) = 0$. 
% Interventions can also be performed on multiple attributes 
% % (as shown in Figure \ref{fig:generic-query}) 
% when there are no edges connecting the attributes in the $\intervene$ clause (this is a stricter restriction than a path between the attributes) \amir{verify}.
% \babak{The intervene oprator and the possible world paragraphs should be integrared.}




\paragraph{Causal model}
We assume that the database $D$ is associated with a Probabilistic Causal Model (PCM) $P$ \cite{?}. 
% that defines the probability distribution over $PWD(D)$ after a hypothetical update.
The PCM defines a probability distribution based on the database, the update, and the causal dependency DAG. 
We next give an intuitive description of a causal DAG. We refer the reader to the causal inference literature for the formal definitions of PCMs, causal DAGs, and the structural equations that define the probability distribution in a rigorous manner \cite{?}, as these are beyond the scope of this paper.

In a causal DAG $G = (\mb{V},\mb{E})$, each node $A_i \in \mb{V}$ represents an attribute name and each edge $(A_i, A_j) \in \mb{E}$ says that the attribute $A_i$ affects the attribute $A_j$. \amir{verify:} Only attributes in ${\mb A_{mu}}$ can have incoming edges, as they are the only ones that can be changed. 
Given a database instance $D$, a {\em grounded causal DAG} is a DAG based a causal DAG $G$, where each node represents a cell of $D$ with attribute $A_i$ and the edges represent the dependency relationships between the attributes, as expressed in $G$. 
Formally, if $G = (\mb{V},\mb{E})$, the grounded DAG, $G_g$, includes the nodes $\{A[t_i] \in D ~|~ A \in \mb{V}\}$ and $(A_i[t_k], A_j[t_k])$ is in $G_g$ if $(A_i, A_j) \in \mb{E}$. Additionally, $(A_i[t_a], A_j[t_b])$ may be included in $G_g$ if there is a cross-tuple dependency between the attribute $A_i[t_a]$ and the attribute $A_j[t_b]$. 

% We refer the reader to the causal inference literature for the formal definitions of PCMs and causal DAGs \cite{?}, as these are beyond the scope of this paper.

\begin{figure*}[t]
    \centering
\begin{tikzpicture}[scale=0.7]
\begin{scope}[every node/.style={shape=rectangle, rounded corners,thick,draw, top color=white, bottom color=blue!25}]
    \node (Q) at (-9.7,6.5) {\small Quality[$p_1$]};
    \node (A) at (-13.8,4) {\small Category[$p_1$]};
    \node (B) at (-13,5.5) {\small Brand[$p_1$]};
    \node (K) at (-6.4,4) {\small Color[$p_1$]};
    \node (C) at (-7,5.5) {\small Price[$p_1$]};
    \node (F) at (-8,3) {\small Rating[$r_1$]};
    \node (G) at (-11.9,2) {\small Sentiment[$r_1$]};
\end{scope}

\begin{scope}[>={Stealth[black]},
              every edge/.style={draw=black, thick}]
    \path [->] (A) edge node {} (F);
    \path [->] (B) edge node {} (F);
    \path [->] (K) edge node {} (F);
    \path [->,bend right] (C) edge node {} (F);
    \path [->] (A) edge node {} (G);
    \path [->] (F) edge node {} (G);
    \path [->] (B) edge node {} (A);
    
    \path [->] (Q) edge node {} (C);
    \path [->] (Q) edge node {} (F);
    \path [->] (B) edge node {} (Q);
    \path [->] (Q) edge node {} (G);
    \path [->] (B) edge node {} (C);
    \path [->] (B) edge node {} (K);
\end{scope}
% \end{tikzpicture}
% \begin{tikzpicture}[scale=0.7]
\begin{scope}[every node/.style={shape=rectangle, rounded corners,thick,draw, top color=white, bottom color=red!25}]
    \node (Q) at (2.7,6.5) {\small Quality[$p_2$]};
    \node (A) at (-2.5,5) {\small Category[$p_2$]};
    \node (B) at (0,6) {\small Brand[$p_2$]};
    \node (K) at (6.4,4) {\small Color[$p_2$]};
    \node (P) at (5,5.5) {\small Price[$p_2$]};
    \node (R) at (-1,2) {\small Rating[$r_2$]};
    \node (G) at (-4.7,2) {\small Sentiment[$r_2$]};
    \node (R3) at (6.3,2) {\small Rating[$r_3$]};
    \node (S3) at (2.6,2) {\small Sentiment[$r_3$]};
\end{scope}

\begin{scope}[>={Stealth[black]},
            every edge/.style={draw=black, thick}]
    \path [->] (A) edge node {} (R);
    \path [->] (B) edge node {} (R);
    \path [->] (K) edge node {} (R);
    \path [->] (P) edge node {} (R);
    \path [->] (A) edge node {} (G);
    \path [->] (B) edge node {} (A);
    
    \path [->] (Q) edge node {} (P);
    \path [->] (Q) edge node {} (R);
    \path [->] (B) edge node {} (Q);
    \path [->] (Q) edge node {} (G);

    \path [->] (Q) edge node {} (R3);
    \path [->] (Q) edge node {} (S3);
    
    \path [->] (A) edge node {} (R3);
    \path [->] (B) edge node {} (R3);
    \path [->] (K) edge node {} (R3);
    \path [->,bend right] (P) edge node {} (R3);
    
    \path [->,dashed] (C) edge node {} (R);
    \path [->,dashed] (C) edge node {} (R3);
    \path [->,dashed] (P) edge node {} (F);
    
    \path [->] (R) edge node {} (G);
    \path [->] (R3) edge node {} (S3);
    
    \path [->] (B) edge node {} (P);
    \path [->] (B) edge node {} (K);
    
\end{scope}
\end{tikzpicture}
    \caption{Part of the grounded causal graph for the tuples in Figure \ref{fig:database}. 
    $A[p_i]$ ($A[r_j]$) represents the attribute $A$ of tuple $p_i$ ($r_j$). Blue nodes are related to $p_1$, red nodes are related to $p_2$, and dashed edges represent cross-tuple dependencies}
    \label{fig:grounded-causal-graph}
\end{figure*}


\begin{example}\label{ex:grounded-graph}
Figure \ref{fig:grounded-causal-graph} shows a part of the grounded causal graph depicted in Figure \ref{fig:causal-graph}. Nodes of the form $A[t_i]$ represent the attribute $A$ of tuple $t_i$. The part of the graph shown in the figure focuses on $p_1, p_2, r_1, r_2, r_3$ in Figure \ref{fig:database} and shows the cross-attribute affect on the tuple, e.g., the Brand Vaio affects the average Rating of the laptop. There are also cross-tuple dependencies, e.g., the Price of the Vaio laptop ($p_1$) affects the Rating of the Asus laptop ($r_2$). 
\end{example}


We can now define the the probability distribution implied by the PCM over the set of possible worlds after a hypothetical update. 

\begin{definition}\label{def:probability-dist}
Let $D$ be a database, let $P$ be a PCM, and let $U$ be a set of hypothetical updates. If $PWD$ is the set of possible worlds associated with $D$, then the probability distribution function $\pr_{D,P,U}: PWD \to [0,1]$ maps each element $I \in PWD$ to a real value in $[0,1]$ such that $\sum_{I\in PWD} \pr_{D,P,U}(I) = 1$. 
\end{definition}

% We can also marginalize the distribution function over $PWD$, given a hypothetical update, to get a distribution and a set of possible worlds per set of tuples $B$, $PWD(B)$, where $PWD(B)$ are all instances where all tuples $t' \in D \setminus S$ remain unchanged and all attributes of tuples $t \in B$ can get all possible values from their respective domains. In particular, $\sum_{I\in PWD(D)} \pr_{D,P,u}(I) = 1$ and $\sum_{I\in PWD(B)} \pr_{D,P,u}(I) = 1$, i.e., the sum of probabilities for all possible worlds of a database or a tuple is 1. 
% Given a partition of $D$ into sets $\mathcal{B} = \{B_1, 'ldtos, B_l\}$, 
% the connection between the two notions is expressed by the equation $PWD(D) = \times_{i=1}^l PWD(B_i)$, i.e., the set of possible worlds of a database is the Cartesian product of the possible worlds of the partitions in the database. 
% We can also marginalize the distribution function over $PWD$, given a hypothetical update, to get a distribution and a set of possible worlds per tuple $t$, $PWD_t$, where $PWD_t$ are all instances where all tuples $t' \neq t \in D$ remain unchanged and all attributes of $t$ can get all possible values from their respective domains. In particular, $\sum_{I\in PWD} \pr_{D,P,u}(I) = 1$ and $\sum_{I\in PWD_t} \pr_{D,P,u}(I) = 1$, i.e., the sum of probabilities for all possible worlds of a database or a tuple is 1. The connection between the two notions is expressed by the equation $PWD = \times PWD_t$, i.e., the set of possible worlds of a database is the Cartesian product of the possible worlds of each tuples in the database. 
% Moreover, if the tuples in the database are independent, it holds that $\Pr(I) = \prod_{I'\in PWD_t, \forall t\in D} \Pr(I')$. \babak{Why do we need to bring the indepdance assumtion and probabality of a tuple here?}


\begin{example}\label{ex:probability-dist}
Continuing Example \ref{ex:update}, the possible world, $I$, in Figure \ref{tbl:possible-world} is assigned a probability based on the PCM, $P$, defined by the database in Figure \ref{fig:database}, the grounded causal DAG shown in part in Figure \ref{fig:grounded-causal-graph}, and the update that increases the Price value of $p_2$ by 10\%. 

If we were to use a different PCM, $P'$, that would have specified that all attributes and tuples are independent (i.e., the graph in Figure \ref{fig:grounded-causal-graph} was composed of disjoint nodes), then $\pr_{D,P',u}(I) = 1$. 
\end{example}


Throughout the paper, we assume that we have {\em structural homogeneity}, introduced in \cite{SalimiPKGRS20}. 
% which is necessary for estimating the conditional probability distributions from a given database. 
\amir{verify:} Specifically, we assume that for every grounded attribute $A \in {\mb A_{mu}}$, its values in the database share the same conditional probability distribution, given their parents in the causal DAG. 
% For instance, in Figure~\ref{ex:grounded-graph}, we assume that all groundings of type $\mathit{Price}$ share the same conditional probability distribution.
For instance, in Figure~\ref{ex:grounded-graph}, we assume that $\pr_{D,P,u}(\mathit{Price}[p_1] \mid \mathit{Quality}[p_1])$ share the same probability distribution as $\pr_{D,P,u}(\mathit{Price}[p_2] \mid \mathit{Quality}[p_2])$.
This will allow us to compute what-if and how-to query results using causal inference in the following sections. 



\amir{Definitions that can be added to this section but are left in later sections: block-independent database and possible worlds per block, decomposable function}

==> oldnotes.tex <==

\section{Preliminaries}
\label{sec:back}
The notation we use in this paper is summarized in Table~\ref{tab:notations}. We denote variables by uppercase letters,
$X, Y, Z, $ $V$; their values with lowercase letters, $x,y,z, v$; and sets of variables or values using boldface ($\mb X$ or
$\mb x$).  The domain of a variable $X$ is $Dom(X)$, and the domain of
a set of variables is $Dom(\mb X) = \prod_{X\in \mb X} Dom(X)$. All domains are discrete and finite; continuous domains are assumed to be binned. We use the abbreviation $\pr(\mb x)$ to represent a joint probability distribution $\pr(\mb X=\mb x)$. The basic semantic framework of our proposal rests on probabilistic causal models \cite{pearl2009causality}, which we review next.

\begin{table}
%\begin{table}[b!] 
	\centering
	\begin{tabular}{|l|l|} \hline
		\textbf{    Symbol} & \textbf{Meaning} \\ \hline
		$X, Y, Z$ & attributes (variables)\\
		$\mb{X}, \mb{Y}, \mb{Z}$ & sets of attributes \\
		$Dom(X), Dom(\mb{X})$ & their domains \\
		$x \in Dom(X)$ & an attribute value \\ 
		$\mb{x} \in Dom(\mb{X})$& a tuple of attribute values \\
		$\mb{k} \in Dom(\mb{K})$& a tuple of context attribute values \\
		$\cg$ & causal diagram \\
		 $\pcm$ & probabilistic causal model\\
		 		 $O_{\mb X \leftarrow\mb x}$ & potential outcome\\
		 $\pr(\mb V= \mb v), \pr(\mb v)$ &  joint probability distribution\\
		 $\pr(o_{\mb X \leftarrow\mb x})$ & abbreviates $\pr(O_{\mb X \leftarrow\mb x}=o)$\\
	\hline
	\end{tabular}
	\caption{ {\bf Notation used in this paper.}}
	\label{tab:notations}
\end{table}

%\subsection{Probabilistic Causal Models}
%\label{sec:back}

%is an operation that sets the values of $\mb X$ to $\mb x$. Denote by $\cm_{\mb x}=\langle \mb U, \mb V, \mb F_{\mb x}\rangle$ a {\em modified causal model} induced by the intervention $\Do(\mb X=\mb x)$, where $\mb F_{\mb x}$ is obtained from $\mb F$ by replacing the structural equations associated with $\mb X$ by constants $\mb x$. The effect of an {\em intervention} $\Do(\mb X=\mb x)$ is given by the submodel $\cm_{\mb x}$.

\par {\bf Probabilistic causal models.}  A {\em probabilistic causal model} (PCM) is a tuple $\pcm$, where $\cm = \langle \mb U, \mb V, \mb F\rangle$ is a {\em causal model} consisting of a set of \emph{observable or endogenous} variables $\mb V$ and a set of
\emph{background or exogenous} variables $\mb U$ that are outside of the model, and $\mb F = (F_X)_{X \in \mb V}$
is a set of \emph{structural equations} of the form
$F_X : Dom(\Pa_{\mb V}(X)) \times Dom(\Pa_{\mb U}(X)) \rightarrow Dom(X)$, where
$\Pa_{\mb U}(X) \subseteq \mb{U}$ and $\Pa_{\mb V}(X) \subseteq \mb V-\set{X}$
are called \textit{exogenous parents} and \textit{endogenous parents} of $X$, 
respectively. The values of $\mb U$ are drawn from the distribution $\pr(\mb u)$. A PCM $\pcm$ can be represented as a directed graph
$\cg=\langle \mb V, \mb E \rangle$, called a {\em causal diagram}, where each node represents a variable, and there are directed edges from the
elements of $\Pa_{\mb U}(X) \cup \Pa_{\mb V}(X)$ to $X$. We say a variable $Z$ is a {\em descendant} of another variable $X$ if $Z$ is {\em caused} (either {\em directly} or {\em indirectly}) by $X$, i.e., if there is a directed edge or path from $X$ to $Z$ in $G$; otherwise, we say that $Z$ is a {\em non-descendant} of $X$. 
\par 
{\bf Interventions and potential outcomes.}
An {\em intervention} or an {\em action} on a set of variables
$\mb X \subseteq \mb V$, denoted 
$\mb X \leftarrow \mb x$, is an operation that {\em modifies} the underlying causal model by replacing the structural equations associated with $\mb X$ with a constant $\mb x \in Dom(\mb X)$. The {\em potential outcome} of a variable $Y$ after the intervention $\mb X \leftarrow \mb x$ in a context $\mb u \in Dom(\mb U)$, denoted $Y_{\mb X \leftarrow\mb x}(\mb u)$, is the {\em solution} to $Y$ in the modified set of structural equations.  Potential outcomes satisfy the following {\em consistency rule} used in derivations presented in Section~\ref{sec:identif}.
%
%
\begin{align}
\mb X(\mb u)= \mb x \implies Y_{\mb X \leftarrow\mb x}(\mb u)= y \label{eq:consistency}
\end{align}
%
%
%
This rule states that in contexts where $\mb X=\mb x$, the outcome is invariant to the intervention $\mb X \leftarrow\mb x$. For example, changing the income-level of applicants to high does not change the loan decisions for those who already had high-incomes before the intervention.

The distribution  $\pr(\mb u)$ induces a probability distribution over endogenous variables and potential outcomes. Using PCMs, one can express {\em counterfactual queries} of the form $\pr(Y_{\mb X \leftarrow\mb x}=y \mid \mb k)$, or simply $\pr(y_{\mb X \leftarrow\mb x} \mid \mb k)$; this reads as ``For contexts  with attributes $\mb k$, what is the probability that we would observe $Y=y$ had $\mb X$ been $\mb x$?" and is given by the following expression: 
%
%
\vspace{-0.1cm}
\begin{align} 
  \pr(y_{\mb X \leftarrow \mb x} \mid \mb k)
  &= \sum_{\mb u } \ \pr(y_{\mb X \leftarrow \mb x}(\mb u)) \ \pr(\mb u \mid  \mb k) \label{eq:abduction}
\end{align}
%
%
%Equation (\ref{eq:abduction}) readily suggests Pearl's three-step procedure for answering counterfactual queries ~\cite{pearl2009causality}: (1) update $\pr(\mb u)$ to obtain $\pr(\mb u|  \mb e)$ ({\em abduction}). (2) obtain the modified causal model $M_{\mb x}$ to compute $Y_{X \leftarrow x}(\mb u)$ ({\em action}). (3) evaluate the RHS of (\ref{eq:abduction}) using the index function $\pr(Y_{X \leftarrow x}(\mb u)=y)$ {(\em prediction)}.
%

\noindent Equation~\eqref{eq:abduction} readily suggests Pearl's three-step procedure for answering counterfactual queries~ \cite{pearl2009causality}[Chapter~7]: (1) update $\pr(\mb u)$ to obtain $\pr(\mb u \mid  \mb k)$ ({\em abduction}), (2) modify the causal model to reflect the intervention ${\mb X \leftarrow \mb x}$ ({\em action}), and (3) evaluate the RHS of (\ref{eq:abduction}) using the index function $\pr(Y_{\mb X \leftarrow \mb x}(\mb u)=y)$ {(\em prediction)}. However, performing this procedure requires the underlying PCM to be fully observed, i.e, the distribution $\pr(\mb u)$ and the underlying structural equations must be known, which is an impractical requirement. In this paper, we assume that only background knowledge of the underlying causal diagram is available, but exogenous variables and structural equations are unknown. 



\par {\bf The $\Do$-operator.} For causal diagrams, Pearl defined the $\Do$-operator as a graphical operation that gives semantics to {\em interventional queries} of the form ``What is the probability that we would observe $Y=y$ (at population-level) had $\mb X$ been $\mb x$?", denoted $\pr(\mb y \mid \Do(\mb x))$.  Further, he proved a set of necessary and sufficient conditions under which interventional queries can be answered using historical data.  A sufficient condition is the {\em backdoor-criterion},\footnote{Since it is not needed in our work, we do not discuss the graph-theoretic notion of backdoor-criterion.} which states that if there exists a set of variables $\mb C$ that satisfy a graphical condition relative to $\mb X$ and $Y$ in the causal diagram  $G$, the following holds (see~\cite{pearl2009causality}[Chapter~3] for details):
%
%
\begin{align} 
 \pr(\mb y \mid \Do(\mb x))
  &= \sum_{\mb c \in Dom(\mb C)} \pr(\mb y \mid \mb c, \mb x) \ \pr(\mb c)  \label{eq:backdoor}
\end{align}
%
%
In contrast to~\eqref{eq:abduction}, notice that the RHS of \eqref{eq:backdoor} is expressed in terms of observed probabilities and can be estimated from historical data using existing statistical and ML algorithms.  

\par {\bf Counterfactuals vs. interventional queries.} The $\Do$-operator is a population-level operator, meaning it can only express queries about the effect of an intervention at population level; in contrast, counterfactuals can express queries about the effect of an intervention on a sub-population or an individual. Therefore, every interventional query can be expressed in terms of counterfactuals, but not vice versa (see~\cite{pearl2016causal}[Chapter~4] for more details).  For instance,   $\pr(y \mid \Do(\mb x))= \pr( y_{\mb X \leftarrow \mb x})$; however, the counterfactual query $\pr( y_{\mb X \leftarrow \mb x}\mid \mb x',  y')$, which asks about the effect of the intervention $\mb X \leftarrow \mb x$ on a sub-population with attributes $\mb x'$ and $y'$, cannot be expressed in terms of the  $\Do$-operator (see Example~\ref{ex:exp2} below). Note that the probabilistic contrastive counterfactual statements in ~\eqref{eq:ppc}, used throughout this paper to explain a black-box decision-making system concerned with the effect of interventions at sub-population and individual levels, cannot be expressed using the $\Do$-operator and therefore cannot be assessed in general when the underlying probabilistic causal models are not fully observed. Nevertheless, in Section~\ref{sec:identif} we establish conditions under which these counterfactuals can be estimated or bounded using data. 

%\par{\bf Probabilistic Contrastive Counterfactuals}
%The probabilistic contrastive counterfactual statement in ~\eqref{eq:ppc} which is used through this paper for explaining black-box decision-making algorithms can be captured using the following counterfactual statements:

%\begin{align}  \small
%\pr(\text{Out.}_{\text{Att} \leftarrow %\text{<counter.-value>}}=\text{<foil-out.>}\mid \text{<actual-value>}, \text{<actual-out.>}) \label{eq:pfpc}
%\end{align}


%However, the counterfactual statement in~\eqref{eq:pfpc} can not be expressed in terms of the $\Do$-operator, hence can not be answered when the underling probabilistic causal models is not fully observed. Nevertheless, in Section~\ref{sec:identif} we establish conditions under which these counterfactual can be estimated or bounded using historical data. 

\begin{figure*}
    \centering
		\includegraphics[scale=0.55]{figs/dag.pdf}
	\vspace*{-.3cm}		\caption{A causal diagram for Example~\ref{ex:exp}.}
	\label{fig:german-dag}
\end{figure*}
%
\begin{example} \label{ex:exp2}
%\babak{We need to add the DAG for german}
% Note that every interventional query can be expressed in terms of counterfactuals but not the other way around. For example, $\pr(y \mid \Do(X=x))$ is equivalent to the counterfactual $\pr(Y_{X \leftarrow x})$ and $\pr(y \mid \Do(X=x), z)$ is equivalent to the counterfactual $\pr(Y_{X \leftarrow x}=y \mid Z_{X \leftarrow x}=z$. Notice that $\pr(Y_{X \leftarrow x}=y \mid Z_{X \leftarrow x} =z)$  reads as ``the probability of observing the response $Y=y$ given that $Z=z$ observed {\em after} the intervention $X \leftarrow x$", which should be contrasted with the query $\pr(Y_{X \leftarrow x}=y \mid Z=z$) that reads as ``the probability of observing the response $Y=y$ given that we observed $Z=z$ {\em before} the intervention $X \leftarrow x$".  However, the counterfactual query $\pr(Y_{X \leftarrow x}=y \mid y')$ that reads as ``the probability that the response is $Y=y$ after the intervention $X \leftarrow x$ on a group of individuals for which the observed response is actually $Y=y'$" cannot be expressed using the $\Do(.)$ operator. 
Continuing Example~\ref{ex:exp}, Figure~\ref{fig:german-dag} represents a simple causal diagram for the loan application domain, where $G$ corresponds to the attribute gender, $A$ to age, $D$ to the repayment duration in months, $O$ to the decision of a loan application, and $R$ compactly represents the rest of the attributes, e.g., status of checking account, employment, savings, etc. Note that the loan decision is binary: $O=1$ and $O=0$ indicate whether the loan has been approved or not, respectively. The interventional query $\pr(O=1 \mid \Do(D=24 \text{ months}))$ that is equivalent to the counterfactual $\pr(O_{D \leftarrow 24 \text{ months}} =1)$ reads as ``What is the probability of loan approval at population-level had all applicants selected repayment duration of 24 months?" This query can be answered using data and the causal diagram (since $\{G, A\}$ satisfies the backdoor-criterion in the causal diagram in Figure~\ref{fig:german-dag}).  However, the counterfactual query $\pr(O_{D \leftarrow 24\text{ months}}=1 \mid O=0)$, which reads as `What is the probability of loan approval for a group of applicants whose loan applications were denied had they selected a repayment duration of 24 months?", cannot be expressed using the $\Do$-operator.
\end{example}
%Pearl proved the following relationship between backdoor criterion and counterfactuals: If a set $\mb Z$ of variables satisfies the backdoor condition relative to $(\mb X, \mb Y)$, then the following independence known as {\em strong ignorability} holds~\cite[theo. 4.3.1]{pearl2016causal}: \begin{align}
%\mb Y_{\mb X \leftarrow \mb x} \indep \mb X \mid \mb Z \label{eq:ignore}
%\end{align}




==> prelim.tex <==

\begin{figure}[t]
    \centering
\begin{tikzpicture}[scale=0.7]
\begin{scope}[every node/.style={shape=rectangle, rounded corners,thick,draw, top color=white, bottom color=purple!25}]
    \node (A) at (-3,4) {Product};
    \node (B) at (2,4) {Review};
\end{scope}

\begin{scope}[>={Stealth[black]},
            %   every node/.style={fill=white,circle},
              every edge/.style={draw=black, thick}]
    \path [->] (A) edge node[above] {PID} (B);
\end{scope}
\end{tikzpicture}
    \caption{Schema graph}\label{fig:schema-graph}
\end{figure}



\section{Preliminaries}
\label{sec:prelim}

This section reviews basics of causal inference. 
% The notation we use in this paper is summarized in Table~\ref{tab:notations}. 
We denote variables by uppercase letters,
$X, Y, Z, $ $V$; their values with lowercase letters, $x,y,z, v$; and sets of variables or values using boldface ($\mb X$ or
$\mb x$).  The domain of a variable $X$ is $Dom(X)$, and the domain of
a set of variables is $Dom(\mb X) = \prod_{X\in \mb X} Dom(X)$. All domains are discrete and finite; continuous domains are assumed to be binned. We use the abbreviation $\pr(\mb x)$ to represent a joint probability distribution $\pr(\mb X=\mb x)$. 


\paratitle{Schemas, Databases, and Queries.}
We focus in this paper on star schemas \cite{snowflake} where there is a central fact table connected by Foreign Key (FK) joins to the other tables called `dimensional tables'. 
The schema is associated with a directed graph, called a {\em schema graph}, whose nodes are the table names and there is a directed labeled edge between two table names if they have an FK join between them \cite{KalashnikovLS18}. We further assume that the label of each edge makes clear the FK attribute to join on.  \babak{The restriction on star schema comes out the blue. Should we justify it?}


Let ${\mb A}=\{ID,\ldots,A_m\}$ denote the set of attributes and $\mathcal{R} (ID, A_2, \dots,$ $A_m)$
denote a relation schema over them. Then the
set ${\DDom}^m=\Dom(ID)\times \cdots\times \Dom(A_m)$ specifies the domain of all
possible tuples. A dataset $D\subseteq {\DDom}^m$ is a specific instance of the
schema $\mathcal{R}$. We use $t \in\DDom^m$ to denote a tuple in the schema $\mathcal{R}$. 
We assume that $ID$ is an attribute denoting the unique ID of each one of the tuples in $D$. 
We use $t.A_i \in \Dom(A_i)$ to denote the value of the attribute $A_i$ of the tuple $t$ and use $D.A_j$ to denote the column $\langle t_1.A_j, t_1.A_j, \dots, t_n.A_j\rangle$ where $|D| = n$ and $t_i$ denotes the tuples in $D$.

\babak{I am not sure why do we need the following paragraph in this section. It belongs to the body of the paper.}
Let ${\mb A}= {\mb A_{im}} \mathbin{\dot{\cup}} {\mb A_{mu}}$ where ${\mb A_{im}}$ denotes the immutable attributes and ${\mb A_{mu}}$ denotes the mutable attributes, ${\mb A_{im}} \cap {\mb A_{mu}} = \emptyset$. In particular, $ID \in {\mb A_{im}}$, i.e., the ID attribute of the tuples is considered immutable in the causal model that we define in the sequel.
% Let $\mb A_c\subset {\mb A}$ denote actionable attribute, $\mb A_m$ denote mutable and $\mb A_i$ denote immutable attributes.
\babak{same comment as above applied to what comes next}
An aggregate query has the form 
\textsc{SELECT Agg($A_i$), $A_j$ FROM $D$ WHERE Cond GROUPBY $A_j$}, where \textsc{Agg} is an aggregate function that is decomposable \amir{define}, e.g., $\ct$, $\sumsql$, $\avg$, $\minsql$ and \textsc{Cond} is a selection condition on the attributes of $D$. 

\begin{example}
The schema of the product table is depicted in Figure \ref{tbl:amazondatabase} is (PID, Category, Price, Sales Rank, Brand, Color). 
Each tuple in Table \ref{tbl:amazondatabase} has a unique id number (the first attribute) and each attribute has a domain. For example, $\Dom(Price) = [0,500K]$. 
The first tuple has $t_1.Category = Laptop$ and $t_1.Price = 999$ etc. 
The schema graph describing the link between that tables in Figure \ref{fig:database} is depicted in Figure~\ref{fig:schema-graph}. 
The mutable attributes are Price, Sales Rank, and Color. 

An example for an aggregate query on this database is:
\begin{align*}
&\select\ \avg(Price)& \\
&\where\  Category = 'Electronics \to Laptop ~\sqland\
Price > 500
\end{align*}
\end{example}



% \begin{table}
% %\begin{table}[b!] 
% 	\centering \small
% 	\begin{tabular}{|l|l|} \hline
% 		\textbf{    Symbol} & \textbf{Meaning} \\ \hline
% 		$X, Y, Z$ & attributes (variables)\\
% 		$\mb{X}, \mb{Y}, \mb{Z}$ & sets of attributes \\
% 		$Dom(X), Dom(\mb{X})$ & their domains \\
% 		$x \in Dom(X)$ & an attribute value \\ 
% 		$\mb{x} \in Dom(\mb{X})$& a tuple of attribute values \\
% 		$\mb{k} \in Dom(\mb{K})$& a tuple of context attribute values \\
% 		$\cg$ & causal diagram \\
% 		 $\pcm$ & probabilistic causal model\\
% 		 		 $O_{\mb X \leftarrow\mb x}$ & potential outcome\\
% 		 $\pr(\mb V= \mb v), \pr(\mb v)$ &  joint probability distribution\\
% 		 $\pr(o_{\mb X \leftarrow\mb x})$ & abbreviates $\pr(O_{\mb X \leftarrow\mb x}=o)$\\
% 	\hline
% 	\end{tabular}
% 	\caption{ {\bf Notation used in this paper.} \amir{Update}}
% 	\label{tab:notations}
% \end{table}

%\subsection{Probabilistic Causal Models}
%\label{sec:back}

%is an operation that sets the values of $\mb X$ to $\mb x$. Denote by $\cm_{\mb x}=\langle \mb U, \mb V, \mb F_{\mb x}\rangle$ a {\em modified causal model} induced by the intervention $\Do(\mb X=\mb x)$, where $\mb F_{\mb x}$ is obtained from $\mb F$ by replacing the structural equations associated with $\mb X$ by constants $\mb x$. The effect of an {\em intervention} $\Do(\mb X=\mb x)$ is given by the submodel $\cm_{\mb x}$.

\subsection{Background on probabilistic causal models}
\babak{This section is copied from old papers. It should be consilidated to at most three paragraphs.}

The basic semantic framework of our proposal rests on probabilistic causal models \cite{pearl2009causality}, which we review next. 

\paratitle{Probabilistic causal models.}  
A {\em probabilistic causal model} (PCM) is a tuple $\pcm$, where $\cm = \langle \mb U, \mb V, \mb F\rangle$ is a {\em causal model} consisting of a set of \emph{observable or endogenous} variables $\mb V$ and a set of
\emph{background or exogenous} variables $\mb U$ that are outside of the model, and $\mb F = (F_X)_{X \in \mb V}$
is a set of \emph{structural equations} of the form
$F_X : Dom(\Pa_{\mb V}(X)) \times Dom(\Pa_{\mb U}(X)) \rightarrow Dom(X)$, where
% $\Pa_{\mb U}(X) \subseteq \mb{U}$ and $\Pa_{\mb V}(X) \subseteq \mb V-\set{X}$
$\Pa_{\mb U}(X) \subseteq \mb{U}$ and $\Pa_{\mb V}(X) \subseteq \mb V-\set{X}$
are called \textit{exogenous parents} and \textit{endogenous parents} of $X$, 
respectively. The values of $\mb U$ are drawn from the distribution $\pr(\mb u)$. A PCM $\pcm$ can be represented as a directed graph
$\cg=\langle \mb V, \mb E \rangle$, called a {\em causal diagram}, where each node represents a variable, and there are directed edges from the
elements of $\Pa_{\mb U}(X) \cup \Pa_{\mb V}(X)$ to $X$. We say a variable $Z$ is a {\em descendant} of another variable $X$ if $Z$ is {\em caused} (either {\em directly} or {\em indirectly}) by $X$, i.e., if there is a directed edge or path from $X$ to $Z$ in $G$; otherwise, we say that $Z$ is a {\em non-descendant} of $X$. 

\paratitle{Causal DAG.}
A probabilistic causal 
model is
associated with a {\em causal DAG} (directed acyclic graph) 
$\cg$, whose nodes are the
endogenous variables $\mb V$, and whose edges are all pairs $(Z,X)$
such that $Z \in \Pa_{\mb V}(X)$. 
The causal DAG hides
exogenous variables (since we cannot observe them anyway) and instead
captures their effect by defining a probability distribution
$\pr_{\mb U}$ on the endogenous variables.
\footnote{ This is possible under the
{\em causal sufficiency} assumption: 
for any two variables $X, Y \in \mb{V}$, their exogenous parents are disjoint and independent $\Pa_{\mb U}(X) \indep \Pa_{\mb U}(Y)$.  When this assumption fails, one adds more endogenous variables to the model to expose their dependencies.}
We will only refer to endogenous variables in the rest of the paper and drop the subscript $\mb{V}$ from $\Pa_{\mb{V}}$. Similarly,  we will  drop the subscript $\mb U$ from the probability distribution $\pr_{\mb U}$ when it is clear from the context. Then the formula for $\pr(\mb V)$ is the same as that for a Bayesian network:
% {\footnotesize
\begin{align}
\pr(\mb V) = & \prod_{X \in \mb V} \pr(X | \Pa(X))  \label{eq:bayesian}
\end{align}
% }


In the context of relational databases, each node $\mb{V}$ represents an attribute name $A_i$ and the edges represent the relationships between the attributes. 
Given a database $D$, a {\em grounded causal DAG} is a DAG based a causal DAG $G$, where each node represents a cell of $D$ with attribute $A_i$ and the edges represent the inherited relationships between the attributes, as expressed in $G$. 
Formally, if $G = (V,E)$, the grounded DAG $G_g$ includes the vertices $\{t_k[A] \in D ~|~ A \in V\}$ and $(t_k[A_i], t_k[A_j])$ is in $G_g$ if $(A_i, A_j) \in E$. 
% Other cross-tuple edges may be included in $G_g$ based on causal rules that express background knowledge as proposed in \cite{SalimiPKGRS20}.
% \amir{say something about summarization functions}

\begin{figure*}[t]
    \centering
\begin{tikzpicture}[scale=0.7]
\begin{scope}[every node/.style={shape=rectangle, rounded corners,thick,draw, top color=white, bottom color=blue!25}]
    \node (Q) at (-9.7,6.5) {\small Quality[$p_1$]};
    \node (A) at (-13.8,4) {\small Category[$p_1$]};
    \node (B) at (-13,5.5) {\small Brand[$p_1$]};
    \node (K) at (-6.4,4) {\small Color[$p_1$]};
    \node (C) at (-7,5.5) {\small Price[$p_1$]};
    \node (F) at (-8,3) {\small Rating[$r_1$]};
    \node (G) at (-11.9,2) {\small Sentiment[$r_1$]};
\end{scope}

\begin{scope}[>={Stealth[black]},
              every edge/.style={draw=black, thick}]
    \path [->] (A) edge node {} (F);
    \path [->] (B) edge node {} (F);
    \path [->] (K) edge node {} (F);
    \path [->,bend right] (C) edge node {} (F);
    \path [->] (A) edge node {} (G);
    \path [->] (F) edge node {} (G);
    \path [->] (B) edge node {} (A);
    
    \path [->] (Q) edge node {} (C);
    \path [->] (Q) edge node {} (F);
    \path [->] (B) edge node {} (Q);
    \path [->] (Q) edge node {} (G);
    \path [->] (B) edge node {} (C);
    \path [->] (B) edge node {} (K);
\end{scope}
% \end{tikzpicture}
% \begin{tikzpicture}[scale=0.7]
\begin{scope}[every node/.style={shape=rectangle, rounded corners,thick,draw, top color=white, bottom color=red!25}]
    \node (Q) at (2.7,6.5) {\small Quality[$p_2$]};
    \node (A) at (-2.5,5) {\small Category[$p_2$]};
    \node (B) at (0,6) {\small Brand[$p_2$]};
    \node (K) at (6.4,4) {\small Color[$p_2$]};
    \node (P) at (5,5.5) {\small Price[$p_2$]};
    %\node (E) at (5.5,0) {Avg. Rating};
    \node (R) at (-1,2) {\small Rating[$r_2$]};
    \node (G) at (-4.7,2) {\small Sentiment[$r_2$]};
    \node (R3) at (6.3,2) {\small Rating[$r_3$]};
    \node (S3) at (2.6,2) {\small Sentiment[$r_3$]};
\end{scope}

\begin{scope}[>={Stealth[black]},
            every edge/.style={draw=black, thick}]
    \path [->] (A) edge node {} (R);
    \path [->] (B) edge node {} (R);
    \path [->] (K) edge node {} (R);
    \path [->] (P) edge node {} (R);
    \path [->] (A) edge node {} (G);
    % \path [->] (F) edge node {} (G);
    % \path [->] (F) edge node {} (H);
    % \path [->] (G) edge node {} (H);
    \path [->] (B) edge node {} (A);
    
    \path [->] (Q) edge node {} (P);
    \path [->] (Q) edge node {} (R);
    \path [->] (B) edge node {} (Q);
    \path [->] (Q) edge node {} (G);

    \path [->] (Q) edge node {} (R3);
    \path [->] (Q) edge node {} (S3);
    
    \path [->] (A) edge node {} (R3);
    \path [->] (B) edge node {} (R3);
    \path [->] (K) edge node {} (R3);
    \path [->,bend right] (P) edge node {} (R3);
    
    \path [->,dashed] (C) edge node {} (R);
    \path [->,dashed] (C) edge node {} (R3);
    \path [->,dashed] (P) edge node {} (F);
    
    \path [->] (R) edge node {} (G);
    \path [->] (R3) edge node {} (S3);
    
    \path [->] (B) edge node {} (P);
    \path [->] (B) edge node {} (K);
    
    % \path [->] (R2) edge node {} (C);
\end{scope}
\end{tikzpicture}
    \caption{Part of the grounded causal graph for the tuples in Figure \ref{fig:database}. 
    $A[p_i]$ ($A[r_j]$) represents the attribute $A$ of tuple $p_i$ ($r_j$). Blue nodes are related to $p_1$, red nodes are related to $p_2$, and dashed edges represent cross-tuple dependencies}
    % $A[p_i]$ represents the attribute $A$ of tuple $p_i$ and $Rating[r_j]$ ($Sentiment[r_j]$) represents the attribute Rating (Sentiment) in the tuple $r_j$}
    \label{fig:grounded-causal-graph}
\end{figure*}


\begin{example}\label{ex:grounded-graph}
Figure \ref{fig:grounded-causal-graph} shows a part of the grounded causal graph depicted in Figure \ref{fig:causal-graph}. Nodes of the form $A[t_i]$ represent the attribute $A$ of tuple $t_i$. The part of the graph shown in the figure focuses on $p_1, p_2, r_1, r_2, r_3$ in Figure \ref{fig:database} and shows the cross-attribute affect on the tuple, e.g., the Brand Vaio affects the average Rating of the laptop. There are also cross-tuple dependencies, e.g., the Price of the Vaio laptop ($p_1$) affects the Rating of the Asus laptop ($r_2$). 
\end{example}

% For example, in Table \ref{tbl:database}, changing the Education of $t_2$, may affect the Occupation of $t_5$. 


% Figure~\ref{fig:causal-dag} shows a simple
% example of a causal graph based  on Example~\ref{ex:univdomain:causalmodel}: the Score of a paper is affected by its
% Quality and by the Prestige of the author (assuming the reviews are
% single blind), whereas both Quality and Prestige are affected by the author's
% Qualification. Here $\mb V$ = \{\texttt{Qualification}, \texttt{Quality}, \texttt{Prestige}, \texttt{Score}\} are endogenous variables, $\mb U$ endogenous variables are unknown (e.g., mood of a reviewer while reviewing the paper, the expected number of papers to be accepted, scores of other papers the reviewer reviewed, etc.) leading to a probability distribution on $\mb V$. 
% The  dependencies can be represented by three structural  equations:
% %form can be represented as:
% % lg5 - is there a way to formate this more attractively?
% {\footnotesize
% \begin{align}\label{eq:se_background}
% \text{Quality} \sem   \text{Qualification}; & \ \  
% \text{Prestige} \sem  \text{Qualification};\nonumber\\
% \text{Score} \sem  \text{Quality}, \text{Prestige}.&
% \end{align}
% }

\paratitle{Interventions and potential outcomes.}
An {\em intervention} or an {\em action} on a set of variables
$\mb X \subseteq \mb V$, denoted 
$\mb X \leftarrow \mb x$, is an operation that {\em modifies} the underlying causal model by replacing the structural equations associated with $\mb X$ with a constant $\mb x \in Dom(\mb X)$. The {\em potential outcome} of a variable $Y$ after the intervention $\mb X \leftarrow \mb x$ in a context $\mb u \in Dom(\mb U)$, denoted $Y_{\mb X \leftarrow\mb x}(\mb u)$, is the {\em solution} to $Y$ in the modified set of structural equations.  Potential outcomes satisfy the following {\em consistency rule}. \sudeepa{check}
%
%
\begin{align}
\mb X(\mb u)= \mb x \implies Y_{\mb X \leftarrow\mb x}(\mb u)= y \label{eq:consistency}
\end{align}
%
%
%
This rule states that in contexts where $\mb X=\mb x$, the outcome is invariant to the intervention $\mb X \leftarrow\mb x$. For example, changing the income-level of applicants to high does not change the loan decisions for those who already had high-incomes before the intervention.

The distribution  $\pr(\mb u)$ induces a probability distribution over endogenous variables and potential outcomes. Using PCMs, one can express conditional {\em counterfactual queries} of the form $\pr(Y_{\mb X \leftarrow\mb x}=y \mid \mb k)$, or simply $\pr(y_{\mb X \leftarrow\mb x} \mid \mb k)$; this reads as \sudeepa{what is context} ``For contexts  with attributes $\mb k$, what is the probability that we would observe $Y=y$ had $\mb X$ been $\mb x$?" and is given by the following expression: 
%
%
\vspace{-0.1cm}
\begin{align}
  \pr(y_{\mb X \leftarrow \mb x} \mid \mb k)
  &= \sum_{\mb u } \ \pr(y_{\mb X \leftarrow \mb x}(\mb u)) \ \pr(\mb u \mid  \mb k) \label{eq:abduction}
\end{align}
%
%
%Equation (\ref{eq:abduction}) readily suggests Pearl's three-step procedure for answering counterfactual queries ~\cite{pearl2009causality}: (1) update $\pr(\mb u)$ to obtain $\pr(\mb u|  \mb e)$ ({\em abduction}). (2) obtain the modified causal model $M_{\mb x}$ to compute $Y_{X \leftarrow x}(\mb u)$ ({\em action}). (3) evaluate the RHS of (\ref{eq:abduction}) using the index function $\pr(Y_{X \leftarrow x}(\mb u)=y)$ {(\em prediction)}.
%

\noindent Equation~\eqref{eq:abduction} readily suggests Pearl's three-step procedure for answering counterfactual queries~ \cite{pearl2009causality}[Chapter~7]: (1) update $\pr(\mb u)$ to obtain $\pr(\mb u \mid  \mb k)$ ({\em abduction}), (2) modify the causal model to reflect the intervention ${\mb X \leftarrow \mb x}$ ({\em action}), and (3) evaluate the RHS of (\ref{eq:abduction}) using the index function $\pr(Y_{\mb X \leftarrow \mb x}(\mb u)=y)$ {(\em prediction)}. However, performing this procedure requires the underlying PCM to be fully observed, i.e, the distribution $\pr(\mb u)$ and the underlying structural equations must be known, which is an impractical requirement. In this paper, we assume that only background knowledge of the underlying causal diagram is available, but exogenous variables and structural equations are unknown. 

\begin{example}\label{ex:database}
Reconsider the database in Figure \ref{fig:database}. A causal intervention on the database that would change the Price of all Asus laptops to 100\% of their original value and is denoted $Price \gets 1.1 \times Price$. This change will cause other changes in the database based on the the dependency between the attributes and tuples, e.g., the causal graph shows a dependency between the Price and Ratings attributes expressed as a directed edge from the former to the latter. The context $\mb k$ in Equation~\eqref{eq:abduction} is the condition on the query output and $\mb u$ is a value in the domain of an attribute in the grounded graph (a part of it is shown in Figure \ref{fig:grounded-causal-graph}) \amir{say backdoor criteria without defining it}.
\end{example}

% \par {\bf The $\Do$-operator.} For causal diagrams, Pearl \cite{pearl2009causal} defined the $\Do$-operator as a graphical operation that gives semantics to {\em interventional queries} of the form ``What is the probability that we would observe $Y=y$ (at population-level) had $\mb X$ been $\mb x$?", denoted $\pr(\mb y \mid \Do(\mb x))$.  Further, he proved a set of necessary and sufficient conditions under which interventional queries can be answered using historical data.  A sufficient condition is the {\em backdoor-criterion},\footnote{Since it is not needed in our work, we do not discuss the graph-theoretic notion of backdoor-criterion.} which states that if there exists a set of variables $\mb C$ that satisfy a graphical condition relative to $\mb X$ and $Y$ in the causal diagram  $G$, the following holds (see~\cite{pearl2009causality}[Chapter~3] for details):
% %
% %
% \begin{align} 
%  \pr(\mb y \mid \Do(\mb x))
%   &= \sum_{\mb c \in Dom(\mb C)} \pr(\mb y \mid \mb c, \mb x) \ \pr(\mb c)  \label{eq:backdoor}
% \end{align}
% %
% %
% In contrast to~\eqref{eq:abduction}, notice that the RHS of \eqref{eq:backdoor} is expressed in terms of observed probabilities and can be estimated from historical data using existing statistical and ML algorithms.  

% \par {\bf Counterfactuals vs. interventional queries.} The $\Do$-operator is a population-level operator, meaning it can only express queries about the effect of an intervention at population level; in contrast, counterfactuals can express queries about the effect of an intervention on a sub-population or an individual. Therefore, every interventional query can be expressed in terms of counterfactuals, but not vice versa (see~\cite{pearl2016causal}[Chapter~4] for more details).  For instance,   $\pr(y \mid \Do(\mb x))= \pr( y_{\mb X \leftarrow \mb x})$; however, the counterfactual query $\pr( y_{\mb X \leftarrow \mb x}\mid \mb x',  y')$, which asks about the effect of the intervention $\mb X \leftarrow \mb x$ on a sub-population with attributes $\mb x'$ and $y'$, cannot be expressed in terms of the  $\Do$-operator (see Example~\ref{ex:exp2} below). Note that the probabilistic contrastive counterfactual statements in ~\eqref{eq:ppc}, used throughout this paper to explain a black-box decision-making system concerned with the effect of interventions at sub-population and individual levels, cannot be expressed using the $\Do$-operator and therefore cannot be assessed in general when the underlying probabilistic causal models are not fully observed. Nevertheless, in Section~\ref{sec:identif} we establish conditions under which these counterfactuals can be estimated or bounded using data. 

%\par{\bf Probabilistic Contrastive Counterfactuals}
%The probabilistic contrastive counterfactual statement in ~\eqref{eq:ppc} which is used through this paper for explaining black-box decision-making algorithms can be captured using the following counterfactual statements:

%\begin{align}  \small
%\pr(\text{Out.}_{\text{Att} \leftarrow %\text{<counter.-value>}}=\text{<foil-out.>}\mid \text{<actual-value>}, \text{<actual-out.>}) \label{eq:pfpc}
%\end{align}


%However, the counterfactual statement in~\eqref{eq:pfpc} can not be expressed in terms of the $\Do$-operator, hence can not be answered when the underling probabilistic causal models is not fully observed. Nevertheless, in Section~\ref{sec:identif} we establish conditions under which these counterfactual can be estimated or bounded using historical data. 


%

% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c|c| } 
%  \hline
%  Name & Age & Gender & Salary & Position & Team & School \\ 
%  \hline
%  Marie & 45 & F & 250 & Director&X & A \\ 
%  Dan & 23 & M & 200 & SE&X&B\\ 
%  Arthur& 33&M&175 & Scientist&X&B\\
%  Stacy& 35&F&225 &Manager&Y&A\\
%  John& 37&M&200&SE&Y&A\\
%  \hline
% \end{tabular}
% \end{center}


% \begin{example} \label{ex:exp2}
% Consider an database of all employees with the following attributes:
% Name, Age, Gender, Salary, Position, Team and education school. Figure~\ref{fig:} shows the causal graph corresponding to this dataset.

% Question: What will be the average salary of females if they are promoted from manager to Director
% \end{example}





% \begin{example} \label{ex:exp2}
% Consider an database of all employees with the following attributes:
% Name, Age, Gender, School, Attendance, Major, GPA
% Question: What will be the average GPA of students in Duke Univ. if all min. attendance is 80 percent.
% \end{example}


==> prelim2.tex <==

\begin{figure}[h]
    \centering
\begin{tikzpicture}[scale=0.7]
\begin{scope}[every node/.style={shape=rectangle, rounded corners,thick,draw, top color=white, bottom color=purple!25}]
    \node (A) at (-3,4) {Product};
    \node (B) at (2,4) {Review};
\end{scope}

\begin{scope}[>={Stealth[black]},
            %   every node/.style={fill=white,circle},
              every edge/.style={draw=black, thick}]
    \path [->] (A) edge node[above] {PID} (B);
\end{scope}
\end{tikzpicture}
    \caption{Schema graph}\label{fig:schema-graph}
\end{figure}


\section{Preliminaries}
\label{sec:prelim}

\paragraph{Schemas, databases, and aggregate queries.}
We focus in this paper on star schemas \cite{snowflake} where there is a central fact table connected by Foreign Key (FK) joins to the other tables called `dimensional tables'. 
The schema is associated with a directed graph, called a {\em schema graph}, whose nodes are the table names and there is a directed labeled edge between two table names if they have an FK join between them \cite{KalashnikovLS18}. We further assume that the label of each edge makes clear the FK attribute to join on. 
The restriction of star schemas will allow us to combine our model with causal inference on relational databases, while the schema graph allows our query syntax (which will be defined in Section \ref{sec:syntax}) to be simpler. 
% \babak{The restriction on star schema comes out the blue. Should we justify it?}


Let ${\mb A}=\{ID,A_1,\ldots,A_m\}$ denote the set of attributes and $\mathcal{R} (ID, A_2, \dots,$ $A_m)$
denote a relation schema over them. 
% \amir{do we still need ids if we have tuple identifiers?}. 
Then the set ${\DDom}^m=\Dom(ID)\times \Dom(A_1)\times \cdots\times \Dom(A_m)$ specifies the domain of all
possible tuples. A dataset $D\subseteq {\DDom}^m$ is a specific instance of the
schema $\mathcal{R}$. 
% We use $t \in\DDom^m$ to denote a tuple in the schema $\mathcal{R}$. 
We assume that $ID$ is an attribute denoting the unique ID of each one of the tuples in $D$. 
We use $A_i[t] \in \Dom(A_i)$ to denote the value of the attribute $A_i$ of the tuple $t$, and $A_j[D]$ to denote the entire column $\langle A_j[t_1], A_j[t_2], \dots, A_j[t_n]\rangle$, where $|D| = n$. We further associate each tuple with a unique identifier as demonstrated by the identifiers $p_i, r_j$ in Figure \ref{fig:database}.

We also allow aggregate queries on top of our hypothetical queries. We use a standard form of aggregate query \cite{?}, namely:
\textsc{SELECT Agg($A_i$), $A_j$ FROM $D$ WHERE Cond GROUPBY $A_j$}, where \textsc{Agg}$ \in \{\ct,\sumsql,\avg,\minsql\}$ and \textsc{Cond} is a selection condition on the attributes of $D$. 


\begin{example}
The schema of the product table is depicted in Figure \ref{tbl:amazondatabase} is (PID, Category, Price, Brand, Color, Quality). 
Each tuple in Figure \ref{tbl:amazondatabase} has a unique id number (the first attribute) and each attribute has a domain. For example, $\Dom(Price) = [0,500K]$. 
The first tuple has $Category[p_1] = Laptop$ and $Price[p_1] = 999$ etc. 
The schema graph describing the link between that tables in Figure \ref{fig:database} is depicted in Figure~\ref{fig:schema-graph}. 
The mutable attributes are Price, Quality, Category, Color, Rating, and Sentiment. 
An example for an aggregate query on this database is:
\begin{align*}
% &\select\ \avg(Price)& \\
% &\where\  Category = Laptop ~\sqland\
% Price > 500
&\select\ \avg(Rating)~ \from\ Product, Review\\
&\where\  Category = Laptop
\end{align*}
\end{example}

\paragraph{Causal model}
We assume that the database $D$ is associated with a Probabilistic Causal Model (PCM) $P$ \cite{?}. 
% that defines the probability distribution over $PWD(D)$ after a hypothetical update.
The PCM defines a probability distribution based on the database, the update, and the causal dependency DAG. 
We next give an intuitive description of a causal DAG. We refer the reader to the causal inference literature for the formal definitions of PCMs, causal DAGs, and the structural equations that define the probability distribution in a rigorous manner \cite{?}, as these are beyond the scope of this paper.

In a causal DAG $G = (\mb{V},\mb{E})$, each node $A_i \in \mb{V}$ represents an attribute name and each edge $(A_i, A_j) \in \mb{E}$ says that the attribute $A_i$ affects the attribute $A_j$. 
% \amir{verify:} Only attributes in ${\mb A_{mu}}$ can have incoming edges, as they are the only ones that can be changed. 
Given a database instance $D$, a {\em grounded causal DAG} is a DAG based a causal DAG $G$, where each node represents a cell of $D$ with attribute $A_i$ and the edges represent the dependency relationships between the attributes, as expressed in $G$. 
Formally, if $G = (\mb{V},\mb{E})$, the grounded DAG, $G_g$, includes the nodes $\{A[t_i] \in D ~|~ A \in \mb{V}\}$ and $(A_i[t_k], A_j[t_k])$ is in $G_g$ if $(A_i, A_j) \in \mb{E}$. Additionally, $(A_i[t_a], A_j[t_b])$ may be included in $G_g$ if there is a cross-tuple dependency between the attribute $A_i[t_a]$ and the attribute $A_j[t_b]$. 

Throughout the paper, we assume that we have {\em structural homogeneity}, introduced in \cite{SalimiPKGRS20}. 
% which is necessary for estimating the conditional probability distributions from a given database. 
\amir{verify:} Specifically, we assume that for every grounded attribute $A \in {\mb A_{mu}}$, its values in the database share the same conditional probability distribution, given their parents in the causal DAG. 
% For instance, in Figure~\ref{ex:grounded-graph}, we assume that all groundings of type $\mathit{Price}$ share the same conditional probability distribution.
For instance, in Figure~\ref{ex:grounded-graph}, we assume that $\pr_{D,P,u}(\mathit{Price}[p_1] \mid \mathit{Quality}[p_1])$ share the same probability distribution as $\pr_{D,P,u}(\mathit{Price}[p_2] \mid \mathit{Quality}[p_2])$.
This will allow us to compute what-if and how-to query results using causal inference in the following sections. 


\begin{table}[h]
\begin{small}
\centering
\caption{Notations}\label{tbl:notations}
\begin{tabular}{| c | c | c |}
\hline $D$ & Database instance\\
$PWD(D)$ & Possible worlds of $D$\\
$u$ & Hypothetical updates\\
$G$ & Causal DAG\\
$P$ & PCM based on $D$ and $G$\\
$\pr_{D,P,U}$ & Probability dist. over $PWD(D)$ defined by $D,P,U$\\
\hline
\end{tabular}
\end{small}
\end{table}


==> proofextension.tex <==
\onecolumn
\section{Extension: Computation of What-If Queries}


{Generalization: Let $f(Q,D,I) =g( f'(Q,D,B_1),\ldots,f'(Q,D,B_t))$.
Assumption: g is homogenous to degree 1 and f is composable.}

\begin{assumption}We make the following assumptions:\\
\begin{itemize}
    \item $f(Q,D,I) = g(\{f'(Q,D,B) \forall B\in \mathcal{B}_I\})$
    \item $\alpha g(\{x_1,\ldots,x_t\}) = g(\{\alpha x_1,\ldots,\alpha x_t\})$, $\alpha \geq 0$
    \item $ g(\{x_1,\ldots,x_t\}) + g(\{y_1,\ldots,y_t\}) = g(\{x_1+y_1,\ldots, x_t+y_t\})$
\end{itemize}\label{assume:homogenous}
\end{assumption}

\begin{lemma}
Consider a query 
\begin{align*}
&Q\equiv\when&\  g(A_l)\  Then\\
&\update&(A_c)= c\\
&~\and&\\
&\select&\ Agg(\post(B))\\
&\where&\  \pre(A_j)=a_j~\and\\
&&\post(A_i) = a_i %~\and\\
%&\groupby&\  \pre(A_k), \post(A_p)
\end{align*}
and $f(Q,D,I)=Agg(\{t'.B \mid t'\in I, t\in Pre(Q,I), t'.ID=t.ID, t' \in Post(Q,I)\})$.\\ If Agg satisfies the assumption~\ref{assume:homogenous}, then the expected output of the query $Q(D) = g\left(\left\{\expectation_{B' \in \overline{PWD}_{B''}}[f(Q, D, B')] \forall B''\in \mathcal{B}_D\right\}\right)$.
\label{lem:general}
\end{lemma}
\begin{proof}
%Let $S$ denote the subset of $D$ that satisfies $g(A_l)$.
%Expected output of the query for a group $\pre(A_k)=a_k$ and $\post(A_p)=a_p$ can be written as follows. Let $\mathcal{P}$ denote the subset of $PWD$ where $A_p=a_p$ and $A_i=a_i$ for all tuples in $S$.
The query $Q$ intervenes on all tuples $t\in D$ such that $g(t.A_l)=\texttt{True}$. As discussed in Section~\ref{sec:semantics}, we estimate the expected output by modelling the probability distribution over different instances in the possible world PWD and then evaluate query output over the instance $I$ (say $f(Q,D,I)$). To evaluate $f(Q,D,I)$, we first identify a subset $S\subseteq D$ that satisfies the pre-condition, i.e., all tuples $t$ where $t.A_j=a_j$. Therefore $S=\{t: t\in D, t.A_j = a_j\}$. Now, we consider the corresponding set of tuples in $I$ to evaluate the aggregate over $B$ only for the tuples that satisfy the $\post$ condition as 
 $f(Q,D,I) = Agg(\{t'.B \text{ such that }t'\in I, t\in S, t'.ID=t.ID, t'.A_i=a_i\})$. Under this notation, we calculate the query output as follows.

%\begin{align}
%  E[Q,D] &= \sum_{I\in PWD}Pr(I_{A_c \gets c}|g(D.A_l) = True) f(D,I)
%\end{align}


%$PWD = PWD_{n, Dom, schema}$
\begin{align}
  Q(D) &= E_{Pr(I_{D.A_c \gets c \ | \ g(D.A_l) = True})}[f(Q,D, I)] =  \sum_{I\in PWD}Pr(I_{D.A_c \gets c}|g(D.A_l) = True) f(Q,D, I)\\
\end{align}


Using the assumption that $f(Q,D,I) = \sum_{B\in \mathcal{B}_I} f'(Q,D,B)$, we get the following.
\begin{align}
\scriptsize
  Q(D) &= \sum_{I\in PWD_D}\left(\pr(I_{D.A_c \gets c|g(D.A_l) = True}) g(\{ f'(Q,D,B'), \forall B'\in \mathcal{B}_I\})\right)
 \end{align}
 Assuming block-level independence, we substitute $\pr(I_{D.A_c \gets c|g(D.A_l) = True})=\prod_{B\in \mathcal{B}_I} \pr(B_{D.A_c \gets c|g(D.A_l) = True})$
 
 \begin{align}
  &=\sum_{I\in PWD_D}\left(\left(\prod_{B\in \mathcal{B}_I} \pr(B_{D.A_c \gets c|g(D.A_l) = True})\right)  \left( g(\{ f'(Q,D,B'), \forall B'\in \mathcal{B}_I\})\right)\right)\\
 &=\sum_{I\in PWD_D} g\left(\left\{\left(\prod_{B\in \mathcal{B}_I} \pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) f'(Q,D,B') \forall B'\in \mathcal{B}_I\right\}\right)
 \end{align}
 
 Separating out $\pr(B'_{D.A_c \gets c|g(D.A_l) = True})$ from $\prod_{B\in \mathcal{B}_I} \pr(B_{D.A_c \gets c|g(D.A_l) = True})$, we get the following.
 \begin{align}
  &=\sum_{I\in PWD_D} g\left(\{\left(\prod_{B\in \mathcal{B}_I\setminus\{B'\}} \pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) \pr(B'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,B') \forall B'\in \mathcal{B}_I\}\right)\\
  &\text{Since $B'\in \mathcal{B}_I$ is the post interventional block corresponding $B''\in \mathcal{B}_D$ where $B'.ID=B''.ID$}\\
 &=\sum_{I\in PWD_D} g \left\{\sum_{\substack{B''\in \mathcal{B}_D,\\ \text{such that} \\ B'.ID=B''.ID }} \left(\left(\prod_{B\in \mathcal{B}_I\setminus\{B'\}}\pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) \pr(B'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,B')\right), \forall B'\in \mathcal{B}_I\right\}\\
 %&\text{Separating the second summation into two parts, $\sum_{\substack{B''\in \mathcal{B}_D,\\B'\in \mathcal{B}_I  \text{such that} \\ B'.ID=B''.ID }} \equiv \sum_{B''\in \mathcal{B}_D}\sum_{B'\in \mathcal{B}_I}\mathbbm{1}\{B'.ID=B''.ID\} $, where $\mathbbm{1}$ denotes indicator function}\\
  &=\sum_{I\in PWD_D}g\left\{ \left(\sum_{B'\in \mathcal{B}_I}\mathbbm{1}\{B'.ID=B''.ID\}\left(\left(\prod_{B\in \mathcal{B}_I\setminus\{B'\}}\pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) \pr(B'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,B')\right)\right), \forall B''\in\mathcal{B}_D\right\}\\
&=g\left\{\sum_{I\in PWD_D} \left(\sum_{B'\in \mathcal{B}_I}\mathbbm{1}\{B'.ID=B''.ID\}\left(\left(\prod_{B\in \mathcal{B}_I\setminus\{B'\}}\pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) \pr(B'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,B')\right)\right), \forall B''\in \mathcal{B}_D\right\}
\end{align}

Substituting $PWD_D$ as the Cartesian product of $\overline{PWD}_B$ over blocks, $PWD_D= \bigtimes_{B\in \mathcal{B}_D} \overline{PWD}_B$
\begin{align}
&=g\left\{\sum_{\substack{I\in \bigtimes_{B\in \mathcal{B}_D}  \overline{PWD}_B}} \left(\sum_{B'\in \mathcal{B}_I}\mathbbm{1}\{B'.ID=B''.ID\}\left(\left(\prod_{B\in \mathcal{B}_I\setminus\{B'\}}\pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) \pr(B'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,B')\right)\right),\forall B''\in \mathcal{B}_D\right\}
\end{align}


Substituting ${\bigtimes_{B\in \mathcal{B}_D}  \overline{PWD}_B} =  \overline{PWD}_{B''}\times \left(\bigtimes_{B\in \mathcal{B}_D\setminus \{B''\}}  \overline{PWD}_B\right)$

\begin{align}
&=g\left\{\sum_{\substack{I\in\overline{PWD}_{B''}\times \\\left(\bigtimes_{B\in \mathcal{B}_D\setminus \{B''\}}  \overline{PWD}_B\right) }} \left(\sum_{B'\in \mathcal{B}_I}\mathbbm{1}\{B'.ID=B''.ID\}\left(\left(\prod_{B\in \mathcal{B}_I\setminus\{B'\}}\pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) \pr(B'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,B')\right)\right), \forall {B''\in \mathcal{B}_D}\right\}
\end{align}
Let $I=I'\cup I''$ where $I'\in \overline{PWD}_{B''}$ and $I''\in \left(\bigtimes_{B\in \mathcal{B}_D\setminus \{B''\}}  \overline{PWD}_B\right)$.

\begin{align}
&=g\left\{\sum_{\substack{I'\in\overline{PWD}_{B''} }}\sum_{\substack{I''\in\left(\bigtimes_{B\in \mathcal{B}_D\setminus \{B''\}}  \overline{PWD}_B\right) }} \left(\sum_{B'\in \mathcal{B}_I}\mathbbm{1}\{B'.ID=B''.ID\}\left(\left(\prod_{B\in \mathcal{B}_I\setminus\{B'\}}\pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) \pr(B'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,B')\right)\right),{B''\in \mathcal{B}_D}\right\}
\end{align}

 $I'$ corresponds to the post-intervention block of tuples in $B''$, implying $\sum_{B'\in \mathcal{B}_I}\mathbbm{1}\{B'.ID=B''.ID\}$ in the equation ensures that the indicator variable is $1$ whenever $B'=I'$.  Therefore, we replace $B'$ with $I'$.
\begin{align}
&=g\left\{\sum_{\substack{I'\in\overline{PWD}_{B''} }}\sum_{\substack{I''\in\left(\bigtimes_{B\in \mathcal{B}_D\setminus \{B''\}}  \overline{PWD}_B\right) }} \left(\left(\prod_{B\in \mathcal{B}_I\setminus\{I'\}}\pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) \pr(I'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,I')\right), \forall {B''\in \mathcal{B}_D}\right\}
\end{align}

Separating out the terms that depend on $B''$ and $I'$ from the rest.
\begin{align}
&=g\left\{\sum_{\substack{I'\in\overline{PWD}_{B''} }}\left(\left(\pr(I'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,I')\right)\sum_{\substack{I''\in\left(\bigtimes_{B\in \mathcal{B}_D\setminus \{B''\}}  \overline{PWD}_B\right) }} \left(\prod_{B\in \mathcal{B}_I\setminus\{I'\}}\pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) \right),\forall {B''\in \mathcal{B}_D}\right\}
\end{align}

Blocks $B\in \mathcal{B}_I\setminus\{I'\}$ are independent. Therefore, $\left(\prod_{B\in \mathcal{B}_I\setminus\{I'\}}\pr(B_{D.A_c \gets c|g(D.A_l) = True})\right)=\pr(I''_{D.A_c \gets c|g(D.A_l) = True})$
\begin{align}
&=g\left\{\sum_{\substack{I'\in\overline{PWD}_{B''} }}\left(\left(\pr(I'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,I')\right)\sum_{\substack{I''\in\left(\bigtimes_{B\in \mathcal{B}_D\setminus \{B''\}}  \overline{PWD}_B\right) }} \left(\pr(I''_{D.A_c \gets c|g(D.A_l) = True})\right) \right), {B''\in \mathcal{B}_D}\right\}\\
&\text{Since $\sum_{\substack{I''\in\left(\bigtimes_{B\in \mathcal{B}_D\setminus \{B''\}}  \overline{PWD}_B\right) }} \left(\pr(I''_{D.A_c \gets c|g(D.A_l) = True})\right)$ is $1$}\\
&=g\{\sum_{\substack{I'\in\overline{PWD}_{B''} }}\left(\pr(I'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,I')\right),\forall B''\in \mathcal{B}_D \}
\end{align}
Notice that the term $\sum_{\substack{I'\in\overline{PWD}_{B''} }}\left(\pr(I'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,I')\right) $ denotes the expected value of $f'$ over the post-interventional distribution, denoted by $\expectation_{B' \in \overline{PWD}_{B''}}[f(Q, D, B')]$.
\end{proof}


==> proofs/DELETEME---singleblocksum.tex <==

Proposition~\ref{prop:singlerel-simple-backdoor-count} showed that a disjunction of different $\forw$ sub-clauses translates to a summation of different probability values. For simplicity, we now simplify $\valwhatif$ when $Agg=SUM$ for a single sub-clause which consists of a conjunction of $\pre$ and $\post$ clauses.

\begin{proposition}\label{prop:sum}
Given a single-relation database $D$ and a block $D_i\in \mathcal{B}_D$ and a what-if query $Q'$, $Agg=\sumsql$, and $\forw$ clause is denoted by $\pred_{\forw}$ where $\pred_{\forw}$ can be represented as $(\pred_{\forw,\pre}\wedge\pred_{\forw,\post})$, the following holds.
\begin{small}
\begin{equation} %\label{eq:whatif-block}
    \valwhatif(Q', D_i) =  \sum_{t\in D_i} \left(\sum_{y\in \Dom(Y)} \left(y  \pr_{D_i,U}( Y[t]=y,\mu_{\forw,\post}(t)=\true | \mu_{\forw,\pre}(t)=\true)\right)\right)
    \end{equation}
\end{small}
\end{proposition}
\begin{proof}
\begin{align}
\valwhatif(Q',D_i) &=\sum_{\substack{I_j\in\overline{PWD}(D_i) }}\left(\pr_{D_i,U}(I_j) \valwhatif(Q',D_i)\right) \\
%&\text{\amir{$f'$ is $\valwhatif(Q',D_i)$?}}\\
&= \sum_{\substack{I_j\in\overline{PWD}(D_i) }}\left(\pr_{D_i,U}(I_j) \sum_{t\in D_i,t'\in I_j ~:~ \key{}[t]=\key{}[t']}Y[t']\mathbbm{1}\{\pred_{\forw,\pre}(t)=\true \wedge \pred_{\forw,\post} (t')=\true\}\right) \\
&= \sum_{\substack{I_j\in\overline{PWD}(D_i) }}\left(\pr_{D_i,U}(I_j) \sum_{t\in D_i}Y[t']\mathbbm{1}\{\pred_{\forw,\pre}(t)=\true\}\mathbbm{1}\{ \pred_{\forw,\post}(t')=\true, \text{where } \key{}[t]=\key{}[t'], t'\in I'\}\right) \\
&=\sum_{t\in D_i}\left(\mathbbm{1}\{ \pred_{\forw,\pre}(t)=\true \} \sum_{\substack{I_j\in\overline{PWD}(D_i) }}\left(\pr_{D_i,U}(I_j) \sum_{t'\in I_j ~:~ \key{}[t]=\key{}[t']}Y[t']\mathbbm{1}\{ \pred_{\forw,\post}(t')=\true \}\right)\right)\\
%&=\sum_{t\in D_i}\mathbbm{1}\{\pred_{\forw,\pre}(t)=\true \}\sum_{t''\in D_i }\left( \sum_{\substack{I'\in\overline{PWD}_{D_i}\\ t'\in I', t''.ID=t'.ID=t.ID} }Y[t']\left(\pr_{D_i,U}(I') \mathbbm{1}\{  \pred_{\forw,\post}\}(t')=\true\right)\right) \\
%&\text{Innermost summation is non-zero only when $t''=t$}\\
&=\left(\sum_{t\in D_i}\mathbbm{1}\{ \pred_{\forw,\pre}(t)=\true\}\left( \sum_{\substack{I'\in\overline{PWD}_{D_i}\\ t'\in I',\key{}[t]=\key{}[t']} }Y[t']\left(\pr_{D_i,U}(I') \mathbbm{1}\{   \pred_{\forw,\post}(t')=\true\}\right)\right)\right) \\
&=\sum_{t\in D_i}\left( \sum_{y\in \Dom(Y)} \left(y \pr_{D_i,U}(Y[[t]=y, t\in \mu_{\forw,\post} | \mu_{\forw,\pre}(t)=\true)\right)\right)
\end{align}

\end{proof}
The post-update probability distribution $\pr_{D_i,U}$ can be estimated from the input database $D_i$ using the backdoor criterion, as shown above.
Proposition~\ref{prop:sum} extends to the case where $Agg=\avg$ as $\avg$ is equivalent to dividing the output of $\sumsql$ by the number of tuples, $|D_i|$. Similarly, Proposition~\ref{prop:sum} extends to any aggregate function that can be expressed as $c\times \sumsql$ for some constant $c$.


==> proofs/consistent-block-proofOLD.tex <==


\subsection{Extension to Multi-Relation Database\label{sec:muti-relation}}
Recall from Section~\ref{sec:what-if-syntax} that, when we have multiple relations in the what-if query $Q$, we have a relevant view $\cview$ containing the primary keys of the tuples from the relation $R$ (= $D$ for a single-relation database) containing the update attribute $B$, and having other relevant attributes as well as an aggregated form of the output attribute $Y$. Here we argue that our analysis so far extends to what-if queries with
%the previous propositions extend to the case where $D$ contains 
multiple relations because of following reasons.
\begin{itemize}
    \item $\cview$ has the same blocks as the %\cut{multi-relation Database $D$} 
    relation $R$ containing the update attribute $B$ (Proposition~\ref{prop:consistent-blocks} below). This shows that the query output by aggregating the output from individual blocks in %$D$ 
    $R$ is equivalent to aggregating the output from individual blocks in $\cview$.
    \item The probability distribution of  attributes aggregated from different relations into $\cview$ is the same as that of individual tuples in $R$. This property holds under the assumption that all tuples that are aggregated are homogenous, i.e. are distributed according to the same probability distribution (see Section~\ref{sec:model-PCM}). This assumption helps us estimate the probability distribution of the tuples (including aggregated attributes) in a single block of $\cview$ from the causal graph $G$, implying that the analysis in Section~\ref{sec:single-block} can be extended to $\cview$.
\end{itemize}


\subsubsection{Proof that $\cview$ Has the Same Blocks as the Multi-Relation Database}

We next prove that the block decomposition procedure that we describe in Section \ref{sec:whatif-algo} places two tuples in the same block in a multi-relation database $D$ if and only if it places their aggregated version in $\cview$ in the same block if it was performed on $\cview$. 

Recall that our procedure for dividing the database $D$ into independent blocks, which includes taking a tuple $t_1$, identifying all tuples with paths to and from $t_1$ in the causal graph and add them to the same block as $t_1$.This is repeated until all tuples are included in some block. 
% In particular, this procedure divides the tuples according to the connected components of the causal graph, i.e., if the attributes of $t_1$ and $t_2$ are in the same connected component, they are placed in the same block. 

\red{
\begin{enumerate}
    \item Construction of Causal graph for $\cview$ in terms of the causal graph. (Assumption: All tuples are homogeneous and follow the same causal structure)
    The aggregate node (Agg(A1,...,Ak)) is isomorphic to the constituent nodes (A1,....,Ak) and A1 to Ak are removed from the causal graph. Let this graph be G'.
    \item ~[Add as a proposition] To show: $Pr_{G',\cview}(X|,Pa(X)) = Pr_{G,D} (X| Pa(X))$. This is easy to see for any X which is not a child of A1,...,Ak. Now we need to show this only when X is a child of A1,..., Ak.
    \item any pair that is independent in D will be independent in cview (because cview is not adding new edges across tuples). therefore same blocks that were constructed for D will be fine for cview.
\end{enumerate}
This shows that $\cview$ captures the respective dependencies between attributes in $D$. 
}




\begin{proposition}\label{prop:consistent-blocks}
Given a (multi-relation) database $D$, its block-independent decomposition $\mathcal{B} = \{D_1, \ldots, D_\ell\}$, and a what-if query $Q$ creating update view $\cview$, then $t,t' \in D$ are placed in the same block by the above procedure of computing blocks in Section \ref{sec:whatif-algo} if and only if their corresponding tuples in $\cview$, i.e.,   $t_{v}, t'_v \in \cview$ would have been placed in the same block, if the block decomposition procedure was performed on $\cview$. 
% \red{if and only if their corresponding tuples in $\cview$, i.e.,   $t_{v}, t'_v \in \cview$ are placed in the same block, } \sr{--- there is no procedure on $\cview$ -- so this is still not clear}
%by our procedure in Section \ref{sec:whatif-algo}, 
where $t_v$ corresponds to $t$ if it contains a subset of its attributes or an aggregated form thereof (i.e., $\key[t] = \key[t_v]$). 
\end{proposition}


\begin{proof}
($\Leftarrow$) Assume $t, t' \in D$ are not placed in the same block $D_i$ by our procedure in Section \ref{sec:whatif-algo}.
Assume further that the block $D_i \subseteq D$ contains $t$ (and not $t'$). 
If $t,t'$ do not have primary key-foreign key relationship, then we know that $t_v \neq t_v'$ in $\cview$ (since they cannot be summarized to the same tuple) and the attributes of $t_v$ and $t_v'$ are still independent in $\cview$ or dropped from $\cview$. Therefore $t_v$ and $t_v'$ will be in different blocks if we apply our procedure on $\cview$. 
Assume $t,t'$ are independent but have a key relationship possibly through other tuples. 
According to our procedure, $D_i$ {\em contains all tuples that have a path to or from $t$ in the causal graph}. In particular, $D_i$ contains all tuples that have a primary key-foreign key relationship with $t$, as the causal graph contains edges between such tuples. \sr{what does `containing' key of $t$ mean? all keys can be different.} \amir{clearer now?}
Since $t' \not\in D_i$, in particular, it does not share a primary key-foreign key relationship with $t$. 
As mentioned in Section \ref{sec:what-if-syntax}, $\cview$ is created over the relation $R$ containing the update attribute $B$ in $Q$, and other attributes from different relations that are aggregated to $R$ with respect to the tuples in $R$. 
Suppose $t_v, t_v' \in \cview$ are the tuples generated from the (possibly aggregated) attributes of $t, t'$ and $t \in R$ w.l.o.g. 
% In particular, the key in $R$ is not aggregated, so if $t, t' \in R$, they are also independent in $\cview$. 
Here $t_v \in \cview$ can only contain summarized attributes of tuples that have a primary key-foreign key relationship with $t$, and thus cannot include attributes with the key of $t'$ and vice versa. 
Furthermore, if the attributes of $t$ and $t'$ were placed in different blocks in $D$, and they were summarized to $t_v \neq t_v' \in \cview$, then the attributes of $t_v$ and $t_v'$ are will also be placed in different blocks if the procedure is performed on $\cview$. 
% So in $\cview$, $t_v, t_v' \in \cview$ are independent.
So in $\cview$, $t_v, t_v' \in \cview$ will also be placed in different blocks.

($\Rightarrow$) Assume $t, t' \in D$ share the same block $D_i$, then there is a tuple $t'' \in R \cap D_i$ (it may be the case that $t=t''$ or $t'=t''$) and attributes $A, A', A''$ such that there is a path to/from $A[t]$ to/from $A''[t'']$ to/from $A'[t']$. 
If in $\cview$, $t$ and $t'$ are aggregated to the same tuple with the key of $t''$ (e.g., $r_2$, $r_3$ are summarized to the same tuple using $p_2$ in the view created by the what-if query in Figure \ref{fig:whatif-query} in our running example), 
then, denote this tuple by $t_v'' \in \cview$. $t_v''$ has the same key as $t''$ so, in particular, $t_v''$ will be in the same block with itself. 
Otherwise, both $t$ and $t'$ are in $R$, and clearly they will be placed in the same block if the procedure is performed on $\cview$ since they were placed in the same block when the procedure was performed on $D$.  
% Otherwise, they are translated to $t_v, t_v' \in \cview$, where $t_v$ are either (1) left as they are or are (2) aggregated or are (3) dropped. 
% None of these actions change the causal graph so the dependency between $t$ and $t'$ will be translated to a dependency between $t_v$ and $t_v'$. 
% Cases (1), (2) maintain the dependency between the tuples in the causal graph, so there is still a path between the (possibly aggregated) attributes $A[t_v]$ and $A'[t_v']$ in the causal graph. Hence, $t_v,t_v'$ will be in the same block in $\cview$. 
% Suppose there is a path from $A[t]$ to $A'[t']$ in the causal graph (w.l.o.g) and (3) is performed. Any attribute that has a path to $A[t]$ will still affect every attribute that has a path from $A'[t']$, as removing the attributes will not change the causal graph and 
\end{proof}

% \begin{corollary}
% Propositions \ref{prop:single-relation-decompose} and \ref{prop:consistent-blocks} imply Proposition \ref{prop:blocks}. 
% \end{corollary}

% \begin{proof}
% Given a query $Q$ on a block-independent database $D$, 
% the blocks do not change due to the $\use$ operator in $Q$ that creates $\cview$ (Proposition \ref{prop:consistent-blocks}), and the result of $Q$ on $\cview$ can be written as an aggregation of the result of what-if queries $Q'$ on each block in $\cview$. 
% Since these are the same blocks as in $D$, we get the conclusion from proposition \ref{prop:blocks}.
% \end{proof}


\begin{corollary}
Proposition \ref{prop:consistent-blocks} extends all propositions in Sections \ref{sec:to-blocks} and \ref{sec:single-block} to multi-relation databases and thus implies Propositions \ref{prop:blocks}, \ref{prop:causal-results}. 
\end{corollary}

\begin{proof}
%\amir{check:}
Given a query $Q$ on a block-independent database $D$, 
the blocks do not change due to the $\use$ operator in $Q$ that creates $\cview$ (Proposition \ref{prop:consistent-blocks}), and the result of $Q$ on $\cview$ can be written as an aggregation of the result of what-if queries $Q'$ on each block in $\cview$. 
Since these are the same blocks as in $D$, we get the conclusion from proposition \ref{prop:blocks}.
Furthermore, Propositions \ref{prop:single-relation-decompose} and \ref{prop:sum} show the formula for computation over single database blocks, and their aggregation according to Proposition \ref{prop:single-relation-decompose} gives the formulae detailed in Proposition \ref{prop:causal-results}.
\end{proof}

\subsubsection{Homogeneity Assumption}
Multi-relation database is processed by \use\ operator to generate $\cview$, which comprises of aggregated attributes obtained from different relations. The relevant view $\cview$ is used 

\sr{needs some work.. can we show formally how the structural homogenity is used in these proofs?}


% \begin{proposition}
% Given a (multi-relation) database $D$, its block-independent decomposition $\mathcal{B} = \{D_1, \ldots, D_\ell\}$, and a what-if query $Q$ creating $\cview$, then $t,t' \in D$ are independent if and only if their corresponding tuples in $\cview$ $t_{v}, t'_v \in \cview$ are independent, \sg{why is the part after where here?} \amir{since we have to define what we mean by $t_{v}, t'_v$}where $t_v$ corresponds to $t$ if it contains a subset of its attributes or an aggregated form thereof. 
% \end{proposition}


% \begin{proof}
% Assume $t, t' \in D$ are independent, i.e. there are no two attributes $A, A'$, such that there is a path from $A[t]$ to $A[t']$ or from $A[t']$ to $A[t]$. 
% % Now suppose $t, t'$ come from different relations. 
% In Section \ref{sec:whatif-algo} we specify that the block of $t$, denoted $D_i \subseteq D$, {\em is composed of all tuples that have a path to or from $t$ in the causal graph}. In particular, $D_i$ contains all tuples that contain the key of $t$. 
% $t' \not\in D_i$ so, in particular, it does not share a key with $t$. 
% As mentioned in Section \ref{sec:what-if-syntax}, $\cview$ is created over the relation $R$ containing the update attribute $B$ in $Q$, and other attributes from different relations that are aggregated to $R$ with respect to the tuples in $R$. 
% Suppose $t_v, t_v' \in \cview$ are the tuples generated from the (possibly aggregated) attributes of $t, t'$. 
% % In particular, the key in $R$ is not aggregated, so if $t, t' \in R$, they are also independent in $\cview$. 
% $t_v \in \cview$ can only summarize attributes of tuples with the same key as $t$, and thus cannot include attributes from $t'$ and vice versa. 

% Assume $t, t' \in D$ are dependent and share the same block, there exist two attributes $A,A'$ such that there is a path from $A[t]$ to $A'[t']$ w.l.o.g.
% % Thus, share the same block $t, t' \in D_i$. 
% In $\cview$, $t,t'$ can be aggregated to the same tuple (e.g., $r_2$, $r_3$ are summarized to the same tuple in the view created by the what-if query in Figure \ref{fig:whatif-query} in our running example). In particular, if $t,t'$ are the same tuple in $\cview$ they are in the same block. 
% Otherwise, they are translated to $t_v, t_v' \in \cview$, where the attributes $A$ and $A'$ are either (1) left as they are or are (2) aggregated or are (3) dropped. 
% None of these actions change the causal graph so the dependency between $t$ and $t'$ will be translated to a dependency between $t_v$ and $t_v'$. 
% % Cases (1), (2) maintain the dependency between the tuples in the causal graph, so there is still a path between the (possibly aggregated) attributes $A[t_v]$ and $A'[t_v']$ in the causal graph. Hence, $t_v,t_v'$ will be in the same block in $\cview$. 
% % Suppose there is a path from $A[t]$ to $A'[t']$ in the causal graph (w.l.o.g) and (3) is performed. Any attribute that has a path to $A[t]$ will still affect every attribute that has a path from $A'[t']$, as removing the attributes will not change the causal graph and 

% Thus, the block partition of $D$, $\mathcal{B} = \{D_1, \ldots, D_\ell\}$, can be translated into a block partition of $\cview$, $\mathcal{B}' = \{\cview_1, \ldots, \cview_\ell\}$, where $t, t' \in D$ are independent iff their corresponding tuples in $\cview$, $t_v, t_v' \in \cview$ are independent. 

% % $\cview.t is f(D.t_j \forall t_j\in D)$ where $t'.ID=t.ID$.
% \end{proof}

==> proofs/pre-post-split-extension.tex <==
show that any complex $\forw$ operator can be decomposed into a disjunction of conjunctions of disjoint $\forw$ sub-operators 
\sr{is not that obvious? DNF is a normal form for any Boolean formula}. 

\sr{not sure why this proposition is needed. this is obvious to me.}
\begin{proposition}
Given a what-if query $Q$ with $\forw$ operator $\mu_{For}$, the output of the query is equivalent to that of a what-if query $Q'$ where $Q'$ and $Q$ differ only in that $\pred_{\forw}$ operator of $Q'$ can be written as a disjunction of different $\forw$ operators $\lor_i (\pred_{\forw,\pre}^i\wedge \pred_{\forw,\post}^i)$ such that every tuple $t\in D$ and $t'\in I$, where $t$ and $t'$ have the same key satisfy one of the $\pred_{\forw,\pre}^i\wedge \pred_{\forw,\post}^i$ operators.
\end{proposition}
\begin{proof}
The $\forw$ operator defines a subset of $\cview$ and the instances $I\in PWD(\cview)$ to evaluate the query response. Let set $T_I$ denote the set of pairs of tuples in $\cview$ and corresponding tuples in an instance $I\in PWD(\cview)$ that satisfy the $\pred_{\forw}$ operator. More formally, $T_I=\{(t,t') ~:~\forall t\in \cview, \forall t'\in I,\text{ $t,t'$ share the same key and}~\pred_{\forw}(t,t')=\true \}$. We consider $T = \bigcup_{I\in PWD(\cview)} T_I$ and use these tuples to construct an alternate $\pred_{\forw}$ operator which is a disjunction of different sub-operators, where each sub-operator $\pred_{\forw}^i$   uniquely captures a tuple $(t,t')\in T$ i.e., $\pred_{\forw}^i (t,t')=\true$ and $\false$ for any other pair of tuples. This sub-operator is defined as a conjunction of attribute values of the tuples $t$ and $t'$, i.e. $\wedge_i \pre(A_i)=A_i[t] \wedge_j \post(A_j)=A_j[t]$. In this way, any complex $\forw$ operator can be represented as a disjunction of at most $|T|$ $\forw$ sub-operators, where each sub-operator consists of conjunction of $\pre$ and $\post$ conditions. 
Note that $|T|$ can be exponential in the size of the database, however, this expansion is used only for complex queries where the $\forw$ can not be decomposed directly into different sub-operators \amir{change back to say that this is just for the sake of the proof and the expansion is not used in the computation?}. %not used in the computation of the query, and is solely used to prove the existence of a decomposition of $\forw$ operator.
\end{proof}

==> queries.tex <==


\input{theory}

\subsection{$\ct$}
\begin{align*}
\query\  \select\ \ct(*)\  \where\  \post(A_i) = a_i\\ \and\ \update(A_c)= c
\end{align*}

The expected output of this query can be written as 

\begin{align*}
   &&\sum_{t\in D}  \pr[t.A_i=a_i | t.A_c\leftarrow c]\\
   &&\text{Assuming homogeneity}\\
   && =  \Pr[A_i=a_i| A_c\leftarrow c]
\end{align*}

\subsubsection{Alternate approach}

Let $D$ correspond to the input instance and PWD correspond to the possible set of $I$ after intervening on $A_c$.
$PWD=\prod PWD_t$ (assuming independence)


\begin{lemma}
Expected output of the following query is 
\begin{align*}
 \select\ \ct(*)\  \where\  \post(A_i) = a_i\\ \and\ \update(A_c)= c
\end{align*}
\end{lemma}

Expected output of the query can be written as
\begin{align}
   &= \sum_{I\in PWD} Pr(I|\update(A_c)=c, \pre(A_j)=a_j)Q(I)\\
   &\text{Substituting the formulae for $Q$}\\
   &= \sum_{I\in PWD} Pr(I) \sum_{t\in I}\mathbbm{1}\{{t.A_i=a_i}\}\\
   &\text{Assuming independence of tuples}\\
    &=\sum_{I\in PWD} \left(\left(\prod_{t\in I}Pr(I.t)\right) \sum_{t\in I}\mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   &=\sum_{I\in PWD}\sum_{ t\in I} \left(\left(\prod_{t'\in I}Pr(I.t')\right) \mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   &{t=\post(t_p)}\\
   &=\sum_{I\in PWD}\sum_{ \post(t_p)\in I} \left(\left(\prod_{t'\in I}Pr(I.t')\right) \mathbbm{1}\{{t.A_i=a_i}\}\right)\\
    &=\sum_{I\in PWD}\sum_{ t_p\in D} \left(\left(\prod_{t'\in I}Pr(I.t')\right) \mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   &=\sum_{t_p\in D}\sum_{I\in PWD} \left(\left(\prod_{t'\in I}Pr(I.t')\right) \mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   &=\sum_{t_p\in D}\sum_{I\in PWD}\left(\prod_{t'\in I,t'\neq t}Pr(I.t') \right) \left(Pr(I.t)\mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   %&=\sum_{t_p\in D}\pro{t'\neq t, T.t'\in PWD_t'}\sum_{I.t\in PWD_t} \left(Pr(I.t)\mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   &=\sum_{t_p\in D}\sum_{I\in PWD_t} \left(Pr(I)\mathbbm{1}\{{t.A_i=a_i}\}\right)\\
  &=\sum_{t_p\in D}Pr(t.A_i=a_i|\Do(A_c)=c)\\
  &=|D| Pr(A_i=a_i|\Do(A_c)=c)\\
\end{align}



\subsubsection{Relational model}

Expected output of the query can be written as
\begin{align}
   &= \sum_{I\in PWD} Pr(I)Q(I)\\
   &= \sum_{I\in PWD} Pr(I) \sum_{t\in I}\mathbbm{1}\{{t.A_i=a_i}\}\\
   &\text{Using independence of blocks}\\
    &=\sum_{I\in PWD} \left(\left(\prod_{B\in I}Pr(B)\right) \sum_{t\in I}\mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   &=\sum_{I\in PWD, B\in I} \left(\prod_{B\in I}Pr(B) \sum_{t\in B}\mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   %&=\sum_{B\in D}\sum_{I\in PWD} \left(\prod_{t'\in I}Pr(I.t') \mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   &=\sum_{B\in D}\sum_{I\in PWD}\prod_{B'\in I,B'\neq B}Pr(B')  \left(Pr(B)\sum_{t\in B} \mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   &=\sum_{B\in D}\sum_{I.B\in PWD_B} \left(Pr(B)\sum_{t\in B}\mathbbm{1}\{{t.A_i=a_i}\}\right)\\
  &=\sum_{t\in D}(Pr(t.A_i=a_i|\Do(A_c)=c)\\
  &=|D| Pr(A_i=a_i|\Do(A_c)=c)\\
\end{align}
\clearpage
\subsection{General }
\sg{Start here}
\begin{align*}
\query\  \select\ \ct(*)\  \where\  \post(A_i) = a_i\\ \and\ \pre(A_j)=a_j,\   \update(A_c)= c
\end{align*}


Option 1: We define $$PWD = \{(a_1,\cdots,a_t),  \forall a_i\in A_i\}^n$$
independent of query and intervention, depends only on schema and domain. 

Now we need to define 
$$Pr(I|\update(A_c)=c, \pre(A_j)=a_j)$$

This probability is $0$ for all instances where $t.A_j\neq a_j$ and $\olsi{t}.A_k\neq t.A_k \forall A_k$ \amir{where does this condition come from? what is $\olsi{t}$?}
and $\prod_{\olsi{t}\in I,t.A_j=a_j}Pr(t)$ otherwise.\\

Let $S\subseteq D$ denote the largest subset where $t.A_j=a_j, \forall t\in S$.

\begin{align}
   &= \sum_{I\in PWD} Pr(I|\update(A_c)=c, \pre(A_j)=a_j)Q(I)\\
   &= \sum_{I\in PWD} Pr(I|\update(A_c)=c, \pre(A_j)=a_j)\sum_{t\in D}\mathbbm{1}\{{\olsi{t}.A_i=a_i \amir{$\olsi{t}$?} \wedge t.A_j=a_j}\}\\
   &=\sum_{I\in PWD, \olsi{t}.a_j=t.a_j \forall t\in D\setminus S} \left(\prod_{\olsi{t}\in I,t.A_j=a_j}Pr(\olsi{t})\right)\sum_{t\in S}\mathbbm{1}\{{\olsi{t}.A_i=a_i }\}\\
    &=\sum_{I\in PWD, \olsi{t}.a_j=t.a_j \forall t\in D\setminus S} \left(\sum_{t\in S} \left(\prod_{\olsi{t}\in I,t.A_j=a_j}Pr(\olsi{t})\right)\mathbbm{1}\{{\olsi{t}.A_i=a_i }\}\right)\\
 &=\sum_{t\in S} \left(\sum_{I\in PWD, \olsi{t}.a_j=t.a_j \forall t\in D\setminus S} \left(\prod_{\olsi{t}\in I,t.A_j=a_j}Pr(\olsi{t})\right)\mathbbm{1}\{{\olsi{t}.A_i=a_i }\}\right)\\
 &=\sum_{t\in S} \left(\sum_{I\in PWD, \olsi{t}.a_j=t.a_j \forall t\in D\setminus S} \left(\prod_{\olsi{t'}\in I,t'.A_j=a_j,t\neq t'}Pr(\olsi{t'})\right) Pr(\olsi{t})\mathbbm{1}\{{\olsi{t}.A_i=a_i }\}\right)\\
  &=\sum_{t\in S} \left(\sum_{I\in PWD_t, \olsi{t}.a_j=t.a_j \forall t\in D\setminus S}  Pr(\olsi{t})\mathbbm{1}\{{\olsi{t}.A_i=a_i }\}\right)\\
  &=\sum_{t\in S}  Pr(\olsi{t}.A_i=a_i | do(t.A_c)=c)
\end{align}

\sg{Below is a different way to prove the same}
\begin{align*}
\query\  \select\ \ct(*)\  \where\  \post(A_i) = a_i\\ \and\ \pre(A_j)=a_j,\   \update(A_c)= c
\end{align*}
Option 2:
$$PWD^t \subseteq \{(a_1,\cdots,a_t),  \forall a_i\in A_i\}$$
and $PWD=\times_{t\in S} PWD^t$ where $S = \{t \in D : t.A_j = a_j\}$

\begin{align}
&=\sum_{I\in \times_{t \in S} PWD^t} Pr(I|\update(A_c)=c)Q(I)\\
&=\sum_{I\in \times_{t \in S} PWD^t} Pr(I|\update(A_c)=c)\sum_{\olsi{t}\in I} \mathbbm{1}\{\olsi{t}.A_i=a_i\}\\
&=\sum_{I\in \times_{t \in S} PWD^t} \left(\prod_{\olsi{t}\in I}Pr(\olsi{t})\right)\sum_{\olsi{t}\in I} \mathbbm{1}\{\olsi{t}.A_i=a_i\}\\
&=\sum_{I\in \times_{t \in S} PWD^t}\sum_{\olsi{t}\in I} \left(\prod_{\olsi{t}\in I}Pr(\olsi{t})\right) \mathbbm{1}\{\olsi{t}.A_i=a_i\}\\
&=\sum_{I\in \times_{t \in S} PWD^t} \sum_{\olsi{t}\in I} \left(\prod_{t'\neq t, \olsi{t'}\in I}Pr(\olsi{t'})\right)Pr(\olsi{t}) \mathbbm{1}\{\olsi{t}.A_i=a_i\}\\
&= \sum_{{t}\in S}\sum_{I\in \times_{t \in S} PWD^t} \left(\prod_{t'\neq t, \olsi{t'}\in I}Pr(\olsi{t'})\right)Pr(\olsi{t}) \mathbbm{1}\{\olsi{t}.A_i=a_i\}\\
&= \sum_{{t}\in S}\sum_{I\in  PWD^t} Pr(\olsi{t}) \mathbbm{1}\{\olsi{t}.A_i=a_i\}\\
&= \sum_{{t}\in S} Pr(\olsi{t}.A_i=a_i | do(A_c)=c)\\
\end{align}

\sg{Till here}

\clearpage
\subsection{Join Queries}
We define a general join query.
\begin{align*}
\query\  \select\ \ct(*)\ From\ T1, T2\  \where\  \post(T1.A_i) = T1.a_i \and\ \\ \update(T2.A_c)= c and\ T1.A1=T2.A1 \and\ \pre(T2.A_j)=a_j %\groupby\ T1.A_k
\end{align*}

$$PWD^t \subseteq \{(a_1,\cdots,a_t),  \forall a_i\in A_i\}$$
and $PWD=\times_{t\in S} PWD^t$ where $S = \{t \in D : t.A_j = a_j\}$

\begin{align}
&=\sum_{I\in \times_{t \in S} PWD^t} Pr(I|\update(A_c)=c)Q(I)\\
&=\sum_{I\in \times_{t \in S} PWD^t} Pr(I|\update(A_c)=c)\sum_{\olsi{t}\in I} \mathbbm{1}\{\olsi{t}.A_i=a_i\}\\
&=\sum_{I\in \times_{t \in S} PWD^t} \left(\prod_{\olsi{t}\in I}Pr(\olsi{t})\right)\sum_{\olsi{t}\in I} \mathbbm{1}\{\olsi{t}.A_i=a_i\}\\
&=\sum_{I\in \times_{t \in S} PWD^t}\sum_{\olsi{t}\in I} \left(\prod_{\olsi{t}\in I}Pr(\olsi{t})\right) \mathbbm{1}\{\olsi{t}.A_i=a_i\}\\
&=\sum_{I\in \times_{t \in S} PWD^t} \sum_{\olsi{t}\in I} \left(\prod_{t'\neq t, \olsi{t'}\in I}Pr(\olsi{t'})\right)Pr(\olsi{t}) \mathbbm{1}\{\olsi{t}.A_i=a_i\}\\
&= \sum_{{t}\in S}\sum_{I\in \times_{t \in S} PWD^t} \left(\prod_{t'\neq t, \olsi{t'}\in I}Pr(\olsi{t'})\right)Pr(\olsi{t}) \mathbbm{1}\{\olsi{t}.A_i=a_i\}\\
&= \sum_{{t}\in S}\sum_{I\in  PWD^t} Pr(\olsi{t}) \mathbbm{1}\{\olsi{t}.A_i=a_i\}\\
&= \sum_{{t}\in S} Pr(\olsi{t}.A_i=a_i | do(A_c)=c)\\
\end{align}


\clearpage
\clearpage
\subsection{$\select$}
\begin{align*}
\query\  \select\ \avg(\post(A_j))\  \where\  \post(A_i) = a_i\\ \and\ \update(A_c)= c
\end{align*}


The expected output of this query can be written as 

\begin{align*}
   &&\frac{1}{|D|} \sum_{t\in D,a_j\in \Dom(A_j)} a_j \times \pr[t.A_j=a_j, t.A_i=a_i | t.A_c\leftarrow c]\\
   &&\text{Assuming the dataset is a representative}\\
   &&\text{sample of the underlying causal graph}\\
   && = \sum_{a_j\in \Dom(A_j)} a_j \Pr[A_j=a_j, A_i=a_i| A_c\leftarrow c]
\end{align*}

\subsubsection{Proof}
\begin{align}
   &= \sum_{I\in PWD} Pr(I)Q(I)\\
   &\text{Substituting the formulae for $Q$}\\
   &= \sum_{I\in PWD} Pr(I) \sum_{t\in I}t.A_j\mathbbm{1}\{{t.A_i=a_i}\}\\
   &\text{Assuming independence of tuples}\\
    &=\sum_{I\in PWD} \left(\left(\prod_{t\in I}Pr(I.t)\right) \sum_{t\in I}t.A_j\mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   &=\sum_{I\in PWD}\sum_{ t\in I} \left(\left(\prod_{t'\in I}Pr(I.t')\right) t.A_j\mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   &{t=\post(t_p)}\\
   &=\sum_{I\in PWD}\sum_{ \post(t_p)\in I} \left(\left(\prod_{t'\in I}Pr(I.t')\right) t.A_j\mathbbm{1}\{{t.A_i=a_i}\}\right)\\
    &=\sum_{I\in PWD}\sum_{ t_p\in D} \left(\left(\prod_{t'\in I}Pr(I.t')\right) t.A_j\mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   &=\sum_{t_p\in D}\sum_{I\in PWD} \left(\left(\prod_{t'\in I}Pr(I.t')\right) t.A_j\mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   &=\sum_{t_p\in D}\sum_{I\in PWD}\left(\prod_{t'\in I,t'\neq t}Pr(I.t') \right) \left(Pr(I.t)t.A_j\mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   %&=\sum_{t_p\in D}\pro{t'\neq t, T.t'\in PWD_t'}\sum_{I.t\in PWD_t} \left(Pr(I.t)\mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   &=\sum_{t_p\in D}\sum_{I\in PWD_t} \left(Pr(I)t.A_j\mathbbm{1}\{{t.A_i=a_i}\}\right)\\
  &=\sum_{t_p\in D}E(t.A_j | t.A_i=a_i,\Do(A_c)=c)\\
  &=|D| E(t.A_j | t.A_i=a_i,\Do(A_c)=c)\\
\end{align}


\subsection{Join}
Suppose we know the causal graph over union of attributes.

\begin{align*}
\query\  \avg(\post(D_2.A_k))\ \where\  \pre(D_1.A_i) = \pre(D_2.A_j)\\\ \text{ and } \update(D_1.A_c)= c
\end{align*}

Suppose its a key-foreign key join (or a join similar to data augmentation) and we have a causal graph for the universal table.
\begin{align}
&\frac{1}{|D|}\sum_{t\in D_1,t'\in D_2, t.A_i=t'.A_j, \alpha\in \Dom(A_k)}\alpha \pr[ t'.A_k=\alpha | t.A_c\leftarrow c ]\\
&\sum_{\beta\in \Dom(A_i)\cap \Dom(A_j)} \alpha\pr[ t'.A_k=\alpha | A_i=\beta, A_j=\beta, t.A_c\leftarrow c ]
\end{align}

\subsection{$\select$}
\begin{align*}
\query\  \select\ \avg(\post(A_j))\  \where\  \post(A_i) = a_i\ \\
\and\ \pre(A_k=a_k) \and\ \update(A_c)= c
\end{align*}

Let $\gamma$ denote the sub-population with $A_k=a_k$.

\begin{align}
&\frac{1}{\gamma}\sum_{t\in D,a_j\in \Dom(A_j)} a_j \times \pr[t.A_j=a_j, t.A_i=a_i | t.A_c\leftarrow c, t.A_k=a_k]\\
&\sum_{a_j\in \Dom(A_j)} a_j \Pr[A_j=a_j, A_i=a_i|A_k=a_k, A_c\leftarrow c]
\end{align}




\subsection{Groupby}
A group-by query:

\begin{align*}
\query\ \select\ \post(A_2), \avg(\post(A_1))\ \where\ \\ \update(A_c)= c, \groupby\ \post(A_2)
\end{align*}


This is equivalent to saying:
For all $\alpha\in \Dom(A_2)$
\begin{align}
\query\ Select\  \avg(\post(A_1))\ \where\  \update(A_c)= c, \post(A_2)=\alpha
\end{align}

and this was handled by Section 3.1. 


\section{Old notes}

Below are some notes from discussion

\begin{align}
\query\  \select\ \avg(income)\  \where\  A_i' = google\\
\ \and\ A_k=female\   \and\ A_c\leftarrow phd
\end{align}

$A_i(A_c=c)$: the potential outcome of $A_i$ after intervention $A_c=c$. 

$$P(A_i(A_c=c))$$
$$P(A_i(A_c=c)| A_k=a_k)$$
$$P(A_i(A_c=c)| A_z(A_c=c)=a_z)$$
$$P(A_i(A_c=c)| A_z(A_c=c)=a_z, A_k=a_k)$$

$$P(A_i(A_c=c))= P(A_i| do(A_c=c))$$
$$P(A_i(A_c=c)| A_c=c')=? P(A_i| do(A_c=c), A_c=c')$$

Dynamic intervention: $$P(A_i(A_c=f(A_Z)))$$

$$P(A_i(A_c=c))= P(A_i| do(A_c=c)) = P(A_i | A_c=c)$$
$$P(A_i(A_c=c)| A_c=c')=? P(A_i| do(A_c=c), A_c=c')= P(A_i| A_c=c, A_c=c')$$

$f$ can be an indicator function or a real-valued function.

More general: stochastic intervention. 



==> running_example.tex <==
% \begin{table}[]
% \begin{center}
% \begin{tabular}{ |c|c|c|c|c|c|c|c| } 
%  \hline
%  CustID & GM & Tesla & Amazon & Walmart & WholeFoods & Yield \\ 
%  \hline
%  1 & 10 & 15 & 20 & 10 & 15 & 10\\ 
%  2 & 8 & 2 & 7 & 8 & 10 & 6 \\ 
%  3 & 35 & 0 & 51 & 5 & 0 & 12\\
%  4 & 0 & 21 & 0 & 15 & 0 & -20\\
%  5 & 2 & 40 & 25 & 0 & 5 & 74 \\
%  \hline
% \end{tabular}
% \end{center}
% \caption{Portfolio database \amir{work in progress}}\label{tbl:portfolio}
% \end{table}



\begin{table}[]
\begin{center}
\begin{tabular}{ |c|c|c|c|c|c|c|c| } 
 \hline
 ID & Age & Race & Marital Status & Education & Occupation & Income \\ 
 \hline
 1 & 25 & White & Single & BSc & Developer & 150\\ 
 2 & 25 & Asian & Married & MSc & Manager & 220\\ 
 3 & 35 & Black & Single & Phd & Scientist & 290\\
 4 & 55 & White & Divorced & BSc & Sales & 250\\
 5 & 50 & Black & Married & MSc & Director & 470 \\
 \hline
\end{tabular}
\end{center}
\caption{Income database}\label{tbl:database}
\end{table}


\begin{figure}[t]
    \centering
\begin{tikzpicture}[scale=0.7]
\begin{scope}[every node/.style={shape=rectangle, rounded corners,thick,draw}]
    \node (A) at (-.3,4) {Gender};
    %\node (B) at (0,4) {Nationality};
    \node (C) at (6.2,4) {Age};
    \node (E) at (3.5,3.7) {Marital Status};
    \node (F) at (7,2) {Education};
    \node (G) at (4,0) {Occupation};
    \node (H) at (0,1) {Income};
    % \node (M) at (-3.5,3) {9};
\end{scope}

\begin{scope}[>={Stealth[black]},
            %   every node/.style={fill=white,circle},
              every edge/.style={draw=black, thick}]
    \path [->] (C) edge node {} (E);
    \path [->] (A) edge node {} (E);
    %\path [->] (B) edge node {} (E);
    \path [->] (A) edge node {} (F);
    %\path [->] (B) edge node {} (F);
    \path [->] (C) edge node {} (F);
    \path [->] (E) edge node {} (F);
    \path [->] (A) edge node {} (G);
    %\path [->] (B) edge node {} (G);
    \path [->] (C) edge node {} (G);
    \path [->] (E) edge node {} (G);
    \path [->] (F) edge node {} (G);
    \path [->] (A) edge node {} (H);
    %\path [->] (B) edge node {} (H);
    \path [->] (C) edge node {} (H);
    \path [->] (E) edge node {} (H);
    \path [->] (F) edge node {} (H);
    \path [->] (G) edge node {} (H);
\end{scope}
\end{tikzpicture}
    \caption{Causal graph}\label{fig:causal-graph}
\end{figure}

% \begin{example}
% Consider a census database consisting of individual demographics along with education, occupation and income information.
% \end{example}


 \begin{figure}[t]
     \centering
 \begin{tikzpicture}[scale=0.7]
 \begin{scope}[every node/.style={shape=rectangle, rounded corners,thick,draw}]
     \node (A) at (2.5,2) {Yield};
     \node (B) at (0.5,3) {Amazon};
     \node (C) at (3,4) {WholeFoods};
     \node (J) at (6,4) {GM};
     \node (K) at (6,2.5) {Tesla};
     \node (L) at (-2,2) {Walmart};
     % \node (M) at (-3.5,3) {9};
 \end{scope}

 \begin{scope}[>={Stealth[black]},
                every node/.style={fill=white,circle},
               every edge/.style={draw=black, thick}]
     \path [<-] (A) edge node {} (B);
     \path [<-] (A) edge node {} (C);
     \path [->] (B) edge node {} (C);
     \path [->] (B) edge node {} (L);
     \path [->] (J) edge node {} (K);
     \path [<-] (A) edge node {} (L);
     \path [->] (J) edge node {} (A);
     \path [->] (K) edge node {} (A);
 \end{scope}
 \end{tikzpicture}
     \caption{Causal graph}\label{fig:causal-graph}
 \end{figure}

\begin{figure}
    \centering
    \begin{align*}
\when\ \intervene(Education)= MSc\\
\select\ \avg(Income)\\
\where\  \pre(Education) = BSc ~\sqland\\
\post(Age) < 50
\end{align*}
    \caption{Causal intervention query ``would studying for a Masters degree increase the income of individuals of age less than 50 with Bachelors degrees?''}
    \label{fig:query}
\end{figure}

==> semantics_old.tex <==
\subsection{Semantics of Counterfactual Queries}
We next define the semantics of the causal operators $\intervene$, $\pre$, $\post$ within the context of relational queries defined in Section \ref{sec:prelim}. 
In the following definitions, we assume that the database $D$ is associated with a PCM $P$ that defines the probability distribution after interventions. 
We use the notation of potential outcomes as described in the previous section. 

\paratitle{Database interventions.}
\amir{Trying to translate eq. 3 to databases:}
Define $Anc(t_i.A_k)$ as all the ancestors of the cell $t_i.A_k$ in the causal DAG $G_g$.

%\begin{align}
\begin{multline}
\pr(t_i.A_k = k_{A_c \gets c})\\
=\sum_{\vec{a}\in \Dom(Anc(t_i.A_k))}(\pr(t_i.A_k = k | Anc(t_i.A_k)=\vec{a}, t_j.A_c\gets c \forall t_j\in Anc(t_i.A_k))
\times\\
\pr(Anc(t_i.A_k)=\vec{a}|t_j.A_c\gets c \forall t_j\in Anc(t_i.A_k)))
\end{multline}
% \end{align}

\paratitle{Post-intervention distribution.}
Previous work \cite{SalimiPKGRS20} has also considered interventions on relational databases and defined the concept of relational peers in the presence of an intervention. Similarly, we can define the {\em peers of a cell} in the database as follows.

\begin{definition}
Given a database $D$, a grounded causal graph $G_g$, and an intervention $A_c \gets c$, the peers of the cell $t_i.A_k$ are the set of cells $t_j.A_c$ such that there is a path in $G_g$ from $t_j.A_c$ to $t_i.A_k$. Denote this set as $Influencers(t_i.A_k)$.
\end{definition}

In particular, $t_i.A_c$ can be an element in $\Pa(t_i.A_k)$.
\amir{Add example}

We can now use this definition to establish the probability of a cell $t_i.A_k$ getting a value $k \in \Dom(A_k)$ when the intervention is $A_c \gets c$: 
\begin{align}
\pr_{P, A_c \gets c}(t_i.A_k = k) \coloneqq \pr(t_i.{A_k} = k~|~ \forall t_j.A_c \in \Pa(t_i.A_k).~ t_j.A_c \gets c)
\end{align}

Now, that we have the probability distribution of a single cell in the database, we can define the probability of a tuple as the joint probability of all attributes: 
\begin{align}
\pr_{P, A_c \gets c}(t_i = (a_1, \ldots, a_m)) \coloneqq \pr_{P, A_c \gets c}(t_i.{A_1} = a_1, \ldots, t_i.{A_m} = a_m)
\end{align}

The probability space for tuples can be lifted to a probability space over all instances $I \subseteq {\DDom}^m$ where if $I = \{t_1, \ldots, t_n\}$, the probability of $I$ is given by the joint probability of all tuples in $I$:

\begin{align}
\pr_{P, A_c \gets c}(I) \coloneqq \pr_{P, A_c \gets c}(t_1, \ldots, t_n)
\end{align}

\amir{Add discussion on assumptions for simplification like block-independence}

% \paratitle{Intervene.}
% The $\intervene$ operator allows queries to define and perform causal interventions on the database. Let $A_c \in {\mb A_{mu}}$. 
% The semantics of the $\intervene(A_c) = c$ operator on $S$ is given by $\forall t_i \in D.~t_i.A_c \gets c$, i.e., changing the cells $t_i.A_c$ of all the tuples in $D$ to $c$. 

% Let $I$ be a database instance with the same schema as $D$ where for each $A_i \in {\mb A_{im}}$, the cell $t_i.A_j \in I$ has the same value as $t_i.A_j \in D$. 
% The probability of an instance $I$ is defined as $\Pr_P(I) = \Pr(I_{t_i.A_c \gets c})$. 
% \amir{remind that interventions can cause the change of other attributes}


% \amir{Add example for changes due to the PCM}

% \subsection{PRE Operator}
% \paratitle{Pre.}
% The $\pre$ operator is applied prior to performing the intervention and can thus contain any standard query operator that should be performed before to the intervention. 
% For example, assume that the query contains $\intervene(A_c) = c$ and $\pre(A_j) = a$ ($A_j$ can be a mutable or an immutable attribute). $\pre(A_j) = a$ is a selection condition whose result is $\{t_i \in D~|~t_i.A_j = a\}$ and the probability of an instance $I$ under the  is then defined as $\Pr(I_{t_i.A_c \gets c}~|~ t_i.A_j = a_j)$. 
% Note that all tuples with $t_i.A_j \neq a_j$ are not intervened on and remain unchanged, so if $t_i.A_j \neq a_j$ for all $t_i \in D$, the intervention is not performed on any tuple and $\Pr_P(I) = 0$ for all $I$. 
% Other operators can also be contained in $\pre$, such as $GroupBy$.

% \amir{Add example}



% \subsection{Possible worlds After Interventions}
% Applying a causal intervention on a database leads to a probability space containing multiple instances, each associated with a probability given by the PCM. 
% We therefore rely on notions from the field of probabilistic databases \cite{??} to account for the generated probability space. 

% \paratitle{Possible worlds.}
% Given a query $Q$ containing the $\intervene$ operator on the database $D$ associated with a PCM, the possible worlds of the pair $Q,D$ are all instances $I$ who have a positive probability. 

% \begin{definition}[Post-intervention PWD]
% Given a query $Q$ on a database $D$ associated with the PCM $P$ where $Q$ contains $\intervene(A_c) = c$ (where $A_c \in {\mb A_{mu}}$), $\pre(A_i) = a_i$ and $\post(A_j) = a_j$,
% the probability of an instance $I$ is $\Pr_P(I) = \Pr(I_{t.A_c = c}|t.A_i = a_i, t.{A_j}_{t.A_c \gets c} = a_j)$.  
% The post-interventional set of possible worlds, $PWD$, is the instances $I$ such that $\Pr_P(I) > 0$. 
% \end{definition}

% \amir{Add example}

% Since the PCM defines a probability space over all possible worlds, for a given query $Q$ on a database $D$, $\sum_{I\in PWD} \Pr(I) = 1$. 
 

% To simplify computations in the context of probabilistic databases, the literature proposes block-independent databases \cite{ReS07,DalviRS09}.
% \begin{definition}[Block-independent database]
% Given a database $D$ associated with a PCM $P$ with a grounded causal DAG $G_g$, a block of $D$ is a set of tuples $B \subseteq D$ such that for all $t \in B$ and for all $t' \in D\setminus B$, there are no edges in $G_g$ between the cells of $t$ and $t'$, i.e., $t$ and $t'$ are independent in the PCM. 
% \end{definition}

% \amir{Add example}

% In our model, given a database $D$ with independent blocks $B_1, \ldots, B_k$, we can decompose the probability of an instance $I$ by using the formula
% $\pr(I_{A_{c} \gets c}) = \prod_{i=1}^k \pr({B_i}_{A_c \gets c})$. 
% In particular, when the blocks are of size $1$, i.e., all tuples in $D$ are independent, we can say that $\pr(I_{A_c \gets c}) = \prod_{i=1}^n \pr({t_i}_{A_c \gets c})$. 



% $$\sum_{I\in PWD} \Pr(I) = 1$$

% $$\sum_{I\in PWD_t} \Pr(I) = 1$$

% $$PWD = \times PWD_t$$

% $$\Pr(I) = \prod_{I'\in PWD_t, \forall t\in D} \Pr(I')$$ due to independence between tuples/blocks

% \begin{example}
% \amir{Add example with a few possible worlds of Table 2 after an intervention and the probability of each one}
% \end{example}

% \subsection{POST Operator}
% \paratitle{Post.}
% The $\post$ operator is applied after performing the intervention and can contain any standard query operator, in a similar manner to $\pre$. 
% For example, assume that the query contains $\intervene(A_c) = c$ and $\post(A_j) = a$ ($A_j$ can be a mutable or an immutable attribute). The probability of an instance $I$ is then defined as $\Pr_P(I) = \Pr(I_{t_i.A_c \gets c}~|~ t_i.{A_j}_{t_i.A_c \gets c} = a_j)$. Other operators can also be contained in $\post$, such as $GroupBy$.

% \amir{Add example}

% \subsection{Output of Counterfactual Queries}

% {\color{red} First without GROUP BY -- a single distribution, then GROUP BY on PRE and POST -- a set of distributions}




==> student_causal_graph.tex <==
\begin{figure}[t]
    \centering
\begin{tikzpicture}[scale=0.7]
\begin{scope}[every node/.style={shape=rectangle, rounded corners,thick,draw,, top color=white, bottom color=blue!25}, 
other/.style={shape=rectangle, rounded corners,thick,draw,, top color=white, bottom color=red!25}]
    \node (A) at (2,5.5) {\small Age};
    \node (S) at (.3,5.5) {\small Gender};
    \node (C) at (4,5.5) {\small Country};
    \node (At) at (5.5,4) {\small Attendance};
    \node (H) at (0.2,3) {\small Hands Raised};
    \node (As) at (3,3) {\small Assignment};
    \node (An) at (3,2) {\small Announcement};
    \node (G) at (3,1) {\small Grade};
     \node (D) at (6,3) {\small Discussion};
    % \node (M) at (-3.5,3) {9};
\end{scope}

\begin{scope}[>={Stealth[black]},
            %   every node/.style={fill=white,circle},
              every edge/.style={draw=black, thick}]
    \path [->] (A) edge node {} (At);
    \path [->] (S) edge node {} (At);
    \path [->] (C) edge node {} (At);
       \path [->] (A) edge node {} (H);
    \path [->] (S) edge node {} (H);
    \path [->] (C) edge node {} (H);
       \path [->] (A) edge node {} (As);
    \path [->] (S) edge node {} (As);
    \path [->] (C) edge node {} (As);
       \path [->] (A) edge node {} (D);
    \path [->] (S) edge node {} (D);
    \path [->] (C) edge node {} (D);
       \path [->] (A) edge node {} (An);
    \path [->] (S) edge node {} (An);
    \path [->] (C) edge node {} (An);
    \path [->] (At) edge node {} (D);
    \path [->] (At) edge node {} (H);
    \path [->] (At) edge node {} (As);
    \path [->] (H) edge node {} (G);
    \path [->] (D) edge node {} (G);
    \path [->] (An) edge node {} (G);
\end{scope}
\end{tikzpicture}
    \caption{A graph showing the dependencies between the attributes in the database in Figure \ref{fig:database}. Blue nodes are attributes of the same tuple and the red node is an attribute of a different tuple. 
    }\label{fig:student-graph}
\end{figure}


==> theory.tex <==
\onecolumn
\section{Computation of What-If Queries}
\amir{what is the formal algorithm here assuming we run on the entire DB?}
\amir{what is the motivation for looking at blocks? why is the computation of what-if queries exponential in the DB size? prove}
In this section, we discuss the computation of hypothetical what-if queries. We assume that the database $D$ is associated with a PRCM $P$ that defines the probability distribution over $PWD(D)$ after a given hypothetical update $U = u_{R, B, f, S}$. 
We can also marginalize the distribution over $PWD(D)$, given an intervention, to get a distribution and a set of possible worlds for any subset of tuples $B\subseteq D$, $PWD_B$, where $PWD_B$ are all instances where all tuples $t' \notin B$ remain unchanged and all attributes of $t\in B$ can get all possible values from their respective domains \sr{B is update attribute, change $B$ to $D'$, change $B_1, B_2$ to $D_1, D_2$ etc. This is not marginalization, can use restricted to B ----- $PWD(B) \subseteq D$, and use $PWD(...)$ instead of subscript}.
The set $B$ is referred to as a \emph{block} \sr{which set? any subset of D?}. For this analysis, we consider a block decomposition of $D$, denoted by $\mathcal{B}_D=\{B_1,\cdots,B_k\}$ where $B_i\cap B_j = \phi, \forall i\neq j$ and $\cup B_i = D$, where tuples in different blocks are independent. 
We leverage the following properties to calculate the query output.


\begin{enumerate}
    \item $\sum_{I\in PWD} \Pr(I) = 1$ and $\sum_{I'\in PWD_B} \Pr(I') = 1$, i.e., the sum of probabilities for all possible worlds of a database or a tuple is 1 \sr{tuple is not mentioned.. database and subset mentioned}.
    \item Consider a partitioning of $D$ into non-overlapping blocks $\mathcal{B}_D=\{B_1,\cdots,B_k\}$. $PWD$ is the same as the Cartesian product of $\overline{PWD}_B, \forall B\in \mathcal{B}_D$, where $\overline{PWD}_B$ contains all instances from $PWD_B$ restricted to tuples in $B$. Mathematically, $\overline{PWD}_B = \{I\cap B,~\forall I\in PWD_B\}$  where $I\cap B = \{t: t\in I, t.ID=t'.ID \text{ for some }t'\in B\}$. \sr{why not define PWD(B) directly as possible worlds of B without mentioning other tuples?}
    \item If the tuples in different blocks of the database are independent, then $\Pr(I) = \prod\limits_{I'\in PWD_B, \forall B\in \mathcal{B}_D} \Pr(I') $ \sr{use $\Pr(I) = \prod\limits_{B\in \mathcal{B}_D}\prod\limits_{I'\in PWD_B} \Pr(I') $}
\end{enumerate} 

%\noindent \textbf{Block-level decomposition.}
%\sg{talk about blocks here and corresponding properties}
We now present a lemma that simplifies the output of the query by leveraging block-independence and the above-mentioned properties. In this proof, we assume that 
$f(Q,D,I) = \sum_{B\in \mathcal{B}_I} f'(Q,D,B)$ for some $f'$. All aggregates (Sum, Avg, Count) satisfy this assumption and it is crucial to decompose the query evaluation on $I$ according to the block-level decomposition. Note that $f(Q,D,B)=f'(Q,D,B)$ if $Agg$ denotes Count or Sum. Whenever $Agg=Avg$, $f'(Q,D,B)=c f(Q,D,B)$, where $c$ is a constant that can be estimated from the query $Q$. \sg{Add more discussion on f'} \sr{average is not correct... it cannot be expressed as sum of f'... we need g(f'(...))}



\begin{lemma}
Consider a query \sr{old version and restricted predicates -- remember B is update attribute, FOR clause can have arbitrary predicate with post and pre that may not be easily decomposable, and we have a USE clause augmenting with aggregates}
\begin{align*}
&Q\equiv\when&\  g(A_l)\  Then\\
&\update&(A_c)= c\\
&~\and&\\
&\select&\ Agg(\post(B))\\
&\where&\  \pre(A_j)=a_j~\and\\
&&\post(A_i) = a_i %~\and\\
%&\groupby&\  \pre(A_k), \post(A_p)
\end{align*}
and $f(Q,D,I)=Agg(\{t'.B \mid t'\in I, t\in Pre(Q,I), t'.ID=t.ID, t' \in Post(Q,I)\})$. \sr{what are pre(Q, I) and post(Q, I)?}\\ If $f(Q,D,I) = \sum_{B\in \mathcal{B}_I} f'(Q,D,B)$, then the expected output of the query $Q(D) = \sum_{B''\in \mathcal{B}_D}\expectation_{B' \in \overline{PWD}_{B''}}[f(Q, D, B')] $, where  $\expectation_{B' \in \overline{PWD}_{B''}}[f'(Q, D, B')]$ denotes the expected value of $f'$ over the post-interventional distribution of the block $B''$.
\label{lem:general}
\end{lemma}
\begin{proof}
%Let $S$ denote the subset of $D$ that satisfies $g(A_l)$.
%Expected output of the query for a group $\pre(A_k)=a_k$ and $\post(A_p)=a_p$ can be written as follows. Let $\mathcal{P}$ denote the subset of $PWD$ where $A_p=a_p$ and $A_i=a_i$ for all tuples in $S$.
The query $Q$ intervenes on all tuples $t\in D$ such that $g(t.A_l)=\texttt{True}$. As discussed in Section~\ref{sec:semantics}, we estimate the expected output by modelling the probability distribution over different instances in the possible world PWD and then evaluate query output over the instance $I$ (say $f(Q,D,I)$). To evaluate $f(Q,D,I)$, we first identify a subset $S\subseteq D$ that satisfies the pre-condition, i.e., all tuples $t$ where $t.A_j=a_j$. Therefore $S=\{t: t\in D, t.A_j = a_j\}$. Now, we consider the corresponding set of tuples in $I$ to evaluate the aggregate over $B$ only for the tuples that satisfy the $\post$ condition as 
 $f(Q,D,I) = Agg(\{t'.B \text{ such that }t'\in I, t\in S, t'.ID=t.ID, t'.A_i=a_i\})$. Under this notation, we calculate the query output as follows.

%\begin{align}
%  E[Q,D] &= \sum_{I\in PWD}Pr(I_{A_c \gets c}|g(D.A_l) = True) f(D,I)
%\end{align}


%$PWD = PWD_{n, Dom, schema}$
\begin{align}
  Q(D) &= E_{Pr(I_{D.A_c \gets c \ | \ g(D.A_l) = True})}[f(Q,D, I)] =  \sum_{I\in PWD}Pr(I_{D.A_c \gets c}|g(D.A_l) = True) f(Q,D, I)\\
\end{align}


Using the assumption that $f(Q,D,I) = \sum_{B\in \mathcal{B}_I} f'(Q,D,B)$, we get the following.
\begin{align}
\scriptsize
  Q(D) &= \sum_{I\in PWD(D)}\left(\pr(I_{D.A_c \gets c|g(D.A_l) = True}) \sum_{B'\in \mathcal{B}_I} f'(Q,D,B')\right)
 \end{align}
 
 Assuming block-level independence, we substitute $\pr(I_{D.A_c \gets c|g(D.A_l) = True})=\prod_{B\in \mathcal{B}_I} \pr(B_{D.A_c \gets c|g(D.A_l) = True})$
 
 \begin{align}
  &=\sum_{I\in PWD(D)}\left(\left(\prod_{B\in \mathcal{B}_I} \pr(B_{D.A_c \gets c|g(D.A_l) = True})\right)  \left( \sum_{B'\in \mathcal{B}_I} f'(Q,D,B')\right)\right)\\
 &=\sum_{I\in PWD(D)} \sum_{B'\in \mathcal{B}_I}\left(\left(\prod_{B\in \mathcal{B}_I} \pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) f'(Q,D,B')\right)
 \end{align}
 
 Separating out $\pr(B'_{D.A_c \gets c|g(D.A_l) = True})$ from $\prod_{B\in \mathcal{B}_I} \pr(B_{D.A_c \gets c|g(D.A_l) = True})$, we get the following.
 \begin{align}
  &=\sum_{I\in PWD(D)} \sum_{B'\in \mathcal{B}_I}\left(\left(\prod_{B\in \mathcal{B}_I\setminus\{B'\}} \pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) \pr(B'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,B')\right)\\
  &\text{Since $B'\in \mathcal{B}_I$ is the post interventional block corresponding $B''\in \mathcal{B}_D$ where $B'.ID=B''.ID$}\\
 &=\sum_{I\in PWD(D)} \sum_{\substack{B''\in \mathcal{B}_D,\\B'\in \mathcal{B}_I  \text{such that} \\ B'.ID=B''.ID }}\left(\left(\prod_{B\in \mathcal{B}_I\setminus\{B'\}}\pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) \pr(B'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,B')\right)\\
 &\text{Separating the second summation into two parts, $\sum_{\substack{B''\in \mathcal{B}_D,\\B'\in \mathcal{B}_I  \text{such that} \\ B'.ID=B''.ID }} \equiv \sum_{B''\in \mathcal{B}_D}\sum_{B'\in \mathcal{B}_I}\mathbbm{1}\{B'.ID=B''.ID\} $, where $\mathbbm{1}$ denotes indicator function}\\
  &=\sum_{I\in PWD(D)} \sum_{B''\in \mathcal{B}_D}\left(\sum_{B'\in \mathcal{B}_I}\mathbbm{1}\{B'.ID=B''.ID\}\left(\left(\prod_{B\in \mathcal{B}_I\setminus\{B'\}}\pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) \pr(B'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,B')\right)\right)\\
  &\text{Swapping the two summations as $\sum_{I\in PWD(D)} $ and $\sum_{B''\in \mathcal{B}_D}$ are independent of each other}\\
&=\sum_{B''\in \mathcal{B}_D}\sum_{I\in PWD(D)} \left(\sum_{B'\in \mathcal{B}_I}\mathbbm{1}\{B'.ID=B''.ID\}\left(\left(\prod_{B\in \mathcal{B}_I\setminus\{B'\}}\pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) \pr(B'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,B')\right)\right)
\end{align}

Substituting $PWD(D)$ as the Cartesian product of $\overline{PWD}_B$ over blocks, $PWD(D)= \bigtimes_{B\in \mathcal{B}_D} \overline{PWD}_B$
\begin{align}
&=\sum_{B''\in \mathcal{B}_D}\sum_{\substack{I\in \bigtimes_{B\in \mathcal{B}_D}  \overline{PWD}_B}} \left(\sum_{B'\in \mathcal{B}_I}\mathbbm{1}\{B'.ID=B''.ID\}\left(\left(\prod_{B\in \mathcal{B}_I\setminus\{B'\}}\pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) \pr(B'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,B')\right)\right)
\end{align}


Substituting ${\bigtimes_{B\in \mathcal{B}_D}  \overline{PWD}_B} =  \overline{PWD}_{B''}\times \left(\bigtimes_{B\in \mathcal{B}_D\setminus \{B''\}}  \overline{PWD}_B\right)$

\begin{align}
&=\sum_{B''\in \mathcal{B}_D}\sum_{\substack{I\in\overline{PWD}_{B''}\times \\\left(\bigtimes_{B\in \mathcal{B}_D\setminus \{B''\}}  \overline{PWD}_B\right) }} \left(\sum_{B'\in \mathcal{B}_I}\mathbbm{1}\{B'.ID=B''.ID\}\left(\left(\prod_{B\in \mathcal{B}_I\setminus\{B'\}}\pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) \pr(B'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,B')\right)\right)
\end{align}
Let $I=I'\cup I''$ where $I'\in \overline{PWD}_{B''}$ and $I''\in \left(\bigtimes_{B\in \mathcal{B}_D\setminus \{B''\}}  \overline{PWD}_B\right)$.

\begin{align}
&=\sum_{B''\in \mathcal{B}_D}\sum_{\substack{I'\in\overline{PWD}_{B''} }}\sum_{\substack{I''\in\left(\bigtimes_{B\in \mathcal{B}_D\setminus \{B''\}}  \overline{PWD}_B\right) }} \left(\sum_{B'\in \mathcal{B}_I}\mathbbm{1}\{B'.ID=B''.ID\}\left(\left(\prod_{B\in \mathcal{B}_I\setminus\{B'\}}\pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) \pr(B'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,B')\right)\right)
\end{align}

 $I'$ corresponds to the post-intervention block of tuples in $B''$, implying $\sum_{B'\in \mathcal{B}_I}\mathbbm{1}\{B'.ID=B''.ID\}$ in the equation ensures that the indicator variable is $1$ whenever $B'=I'$.  Therefore, we replace $B'$ with $I'$.
\begin{align}
&=\sum_{B''\in \mathcal{B}_D}\sum_{\substack{I'\in\overline{PWD}_{B''} }}\sum_{\substack{I''\in\left(\bigtimes_{B\in \mathcal{B}_D\setminus \{B''\}}  \overline{PWD}_B\right) }} \left(\left(\prod_{B\in \mathcal{B}_I\setminus\{I'\}}\pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) \pr(I'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,I')\right)
\end{align}

Separating out the terms that depend on $B''$ and $I'$ from the rest.
\begin{align}
&=\sum_{B''\in \mathcal{B}_D}\sum_{\substack{I'\in\overline{PWD}_{B''} }}\left(\left(\pr(I'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,I')\right)\sum_{\substack{I''\in\left(\bigtimes_{B\in \mathcal{B}_D\setminus \{B''\}}  \overline{PWD}_B\right) }} \left(\prod_{B\in \mathcal{B}_I\setminus\{I'\}}\pr(B_{D.A_c \gets c|g(D.A_l) = True})\right) \right)
\end{align}

Blocks $B\in \mathcal{B}_I\setminus\{I'\}$ are independent. Therefore, $\left(\prod_{B\in \mathcal{B}_I\setminus\{I'\}}\pr(B_{D.A_c \gets c|g(D.A_l) = True})\right)=\pr(I''_{D.A_c \gets c|g(D.A_l) = True})$
\begin{align}
&=\sum_{B''\in \mathcal{B}_D}\sum_{\substack{I'\in\overline{PWD}_{B''} }}\left(\left(\pr(I'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,I')\right)\sum_{\substack{I''\in\left(\bigtimes_{B\in \mathcal{B}_D\setminus \{B''\}}  \overline{PWD}_B\right) }} \left(\pr(I''_{D.A_c \gets c|g(D.A_l) = True})\right) \right)\\
&\text{Since $\sum_{\substack{I''\in\left(\bigtimes_{B\in \mathcal{B}_D\setminus \{B''\}}  \overline{PWD}_B\right) }} \left(\pr(I''_{D.A_c \gets c|g(D.A_l) = True})\right)$ is $1$}\\
&=\sum_{B''\in \mathcal{B}_D}\sum_{\substack{I'\in\overline{PWD}_{B''} }}\left(\pr(I'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,I')\right) 
\end{align}
Notice that the term $\sum_{\substack{I'\in\overline{PWD}_{B''} }}\left(\pr(I'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,I')\right) $ denotes the expected value of $f'$ over the post-interventional distribution, denoted by $\expectation_{B' \in \overline{PWD}_{B''}}[f'(Q, D, B')]$.
\end{proof}


Benefit of Lemma~\ref{lem:general}, suppose Agg  is count(*). Then $f(Q,D,I) = f'(Q,D,I) = \sum_{t'\in I,t\in D |t.ID=t'.ID} \mathbbm{1}\{t.A_j=a_j, t'.A_i=ai\}$.

Therefore, query output is $\Pr(A_i=a_i | A_j=a_j, \Do(A_c)=c)$ under independence assumptions, homogeneity and $A_c\cap (A_i\cup A_j) = \phi$.

\sg{We can show similar simplification for all aggregates.}

\begin{lemma}
Consider a query 
\begin{align*}
&Q\equiv\when&\  g(A_l)\  Then\\
&\update&(A_c)= c\\
&~\and&\\
&\select&\ Count(*)\\
&\where&\  \pre(A_j)=a_j~\and\\
&&\post(A_i) = a_i %~\and\\
%&\groupby&\  \pre(A_k), \post(A_p)
\end{align*}
then the expected output of the query $Q(D) =  |D| \pr(A_i=a_i|A_c\leftarrow c, A_j=a_j, g(A_j)) + \sum_{t\in D}\mathbbm{1}\{t.A_j=a_j, t\notin g(D.A_j), t.A_i=a_i\} $
\end{lemma}
\begin{proof}
For this query, Agg=Count and $B=*$.  Therefore,
\begin{align}
    f(Q,D,I) &= \sum_{t\in D,t'\in I} \mathbbm{1}\{t.A_j=a_j, t'.ID=t.ID, t'.A_i=a_i\}\\
    &=\sum_{t'\in I}\sum_{t\in D} \mathbbm{1}\{  t.A_j=a_j, t'.ID=t.ID, t'.A_i=a_i\}\\
     &=\sum_{B\in \mathcal{B}_I}\sum_{t'\in B}\sum_{t\in D} \mathbbm{1}\{ t.A_j=a_j, t'.ID=t.ID, t'.A_i=a_i\}\\
      &=\sum_{B\in \mathcal{B}_I}\sum_{t'\in B,t\in D} \mathbbm{1}\{  t.A_j=a_j, t'.ID=t.ID, t'.A_i=a_i\}\\
     &=\sum_{B\in \mathcal{B}_I} f(Q,D,B)
\end{align}
Using Lemma~\ref{}, $Q(D)$ is simplified as follows.\\
%\begin{align}
%Q(D)&=\sum_{B''\in \mathcal{B}_D}\sum_{\substack{I'\in\overline{PWD}_{B''} }}\left(\pr(I'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,I')\right) \\
%&=\sum_{B''\in \mathcal{B}_D} \sum_{\substack{I'\in\overline{PWD}_{B''} }}\left(\pr(I'_{D.A_c \gets c|g(D.A_l) = True}) \sum_{t\in B'',t'\in I' \mid t.ID=t'.ID}\mathbbm{1}\{t.A_j=a_j, t'.A_i=a_i\}\right) \\
%&=\sum_{t\in D} \sum_{\substack{t'\in\overline{PWD}_{t} }}\left(\pr(t'_{D.A_c \gets c|g(D.A_l) = True}) \mathbbm{1}\{t.A_j=a_j, t'.A_i=a_i\}\right) \\
%&=\sum_{t\in D}\mathbbm{1}\{t.A_j=a_j\} \sum_{\substack{t'\in\overline{PWD}_{t} }}\left(\pr(t'_{D.A_c \gets c|g(D.A_l) = True}) \mathbbm{1}\{ t'.A_i=a_i\}\right) \\
%&=\sum_{t\in D}\mathbbm{1}\{t.A_j=a_j, t\in g(D.A_j)\} \pr(t.A_i=a_i|D.A_c\leftarrow c)  + \sum_{t\in D}\mathbbm{1}\{t.A_j=a_j, t\notin g(D.A_j), t.A_i=a_i\}\\
%&=\sum_{t\in D}\mathbbm{1}\{t.A_j=a_j,t\in g(D.A_j)\} \pr(t.A_i=a_i|t.A_c\leftarrow c) + \sum_{t\in D}\mathbbm{1}\{t.A_j=a_j, t\notin g(D.A_j), t.A_i=a_i\} \\
%&= |D| \pr(A_i=a_i|A_c\leftarrow c, A_j=a_j, g(A_j)) + \sum_{t\in D}\mathbbm{1}\{t.A_j=a_j, t\notin g(D.A_j), t.A_i=a_i\} \\
%\end{align}
\begin{align}
Q(D)&=\sum_{B''\in \mathcal{B}_D}\sum_{\substack{I'\in\overline{PWD}_{B''} }}\left(\pr(I'_{D.A_c \gets c|g(D.A_l) = True}) f'(Q,D,I')\right) \\
&=\sum_{B''\in \mathcal{B}_D} \sum_{\substack{I'\in\overline{PWD}_{B''} }}\left(\pr(I'_{D.A_c \gets c|g(D.A_l) = True}) \sum_{t\in B'',t'\in I' \mid t.ID=t'.ID}\mathbbm{1}\{t.A_j=a_j, t'.A_i=a_i\}\right) \\
&=\sum_{B''\in \mathcal{B}_D} \sum_{\substack{I'\in\overline{PWD}_{B''} }}\left(\pr(I'_{D.A_c \gets c|g(D.A_l) = True}) \sum_{t\in B''}\left(\mathbbm{1}\{t.A_j=a_j\}\mathbbm{1}\{t'.A_i=a_i, \text{where } t'.ID=t.ID, t'\in I'\}\right)\right) \\
&=\sum_{B''\in \mathcal{B}_D}\left(\sum_{t\in B''}\left(\mathbbm{1}\{t.A_j=a_j\} \sum_{\substack{I'\in\overline{PWD}_{B''} }}\left(\pr(I'_{D.A_c \gets c|g(D.A_l) = True}) \sum_{t'\in I' \mid t.ID=t'.ID}\mathbbm{1}\{ t'.A_i=a_i\}\right)\right)\right) \sg{same as 34}\\
&=\sum_{B''\in \mathcal{B}_D}\left(\sum_{t\in B''}\mathbbm{1}\{t.A_j=a_j\}\sum_{t''\in B'' }\left( \sum_{\substack{I'\in\overline{PWD}_{B''}\\ t'\in I', t''.ID=t'.ID=t.ID} }\left(\pr(I'_{D.A_c \gets c|g(D.A_l) = True}) \mathbbm{1}\{ t'.A_i=a_i\}\right)\right)\right) \\
&\text{Innermost summation is non-zero only when $t''=t$}\\
&=\sum_{B''\in \mathcal{B}_D}\left(\sum_{t\in B''}\mathbbm{1}\{t.A_j=a_j\}\left( \sum_{\substack{I'\in\overline{PWD}_{B''}\\ t'\in I', t.ID=t'.ID} }\left(\pr(I'_{D.A_c \gets c|g(D.A_l) = True}) \mathbbm{1}\{ t'.A_i=a_i\}\right)\right)\right) \\
%&=\sum_{B''\in \mathcal{B}_D}\left(\sum_{t\in B''}\mathbbm{1}\{t.A_j=a_j\} \left(\sum_{t''\in B'',t''.ID=t.ID} \pr(t''.A_i=a_i| D.A_c{g(D.A_l)=True}\gets c)\right)\right) \\
&=\sum_{B''\in \mathcal{B}_D}\left(\sum_{t\in B''} \left( \pr(t.A_i=a_i| t.A_j=a_j, t''.A_c\leftarrow c, \  \forall t''\in B''\cap g(D.A_l))\right)\right) \end{align}
We now use backdoor criterion to estimate the probability values from the original database $D$.

\begin{align}
&\sg{can we have a better notation for the above equation}\\
&=\sum_{B''\in \mathcal{B}_D}\sum_{c\in \Dom (C_{B''})}\left(\sum_{t\in B''} \left( \pr(t.A_i=a_i| t.A_j=a_j, t''.A_c= c, \  \forall t''\in B''\cap g(D.A_l), C_{B''}=c)\right) \pr(c|t.A_j=a_j)\right) \\
\end{align}

\end{proof}

\clearpage
\input{proofextension}
\clearpage


Generalize to percentile
-------------------
\sg{Older proofs below}





\begin{lemma}
Count query under independence assumption
\end{lemma}
\begin{proof}
Expected output of the query can be written as
\begin{align}
   &= \sum_{I\in PWD} Pr(I|\update(A_c)=c, \pre(A_j)=a_j)Q(I)\\
   &\text{Assuming independence of tuples}\\
    &=\sum_{I\in PWD} \left(\left(\prod_{t\in I}Pr(I.t)\right) Q(I)\right)\\
   &=\sum_{I\in PWD}\sum_{ t\in I} \left(\left(\prod_{t'\in I}Pr(I.t')\right) \mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   &{t=\post(t_p)}\\
   &=\sum_{I\in PWD}\sum_{ \post(t_p)\in I} \left(\left(\prod_{t'\in I}Pr(I.t')\right) \mathbbm{1}\{{t.A_i=a_i}\}\right)\\
    &=\sum_{I\in PWD}\sum_{ t_p\in D} \left(\left(\prod_{t'\in I}Pr(I.t')\right) \mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   &=\sum_{t_p\in D}\sum_{I\in PWD} \left(\left(\prod_{t'\in I}Pr(I.t')\right) \mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   &=\sum_{t_p\in D}\sum_{I\in PWD}\left(\prod_{t'\in I,t'\neq t}Pr(I.t') \right) \left(Pr(I.t)\mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   %&=\sum_{t_p\in D}\pro{t'\neq t, T.t'\in PWD(t')}\sum_{I.t\in PWD(t)} \left(Pr(I.t)\mathbbm{1}\{{t.A_i=a_i}\}\right)\\
   &=\sum_{t_p\in D}\sum_{I\in PWD(t)} \left(Pr(I)\mathbbm{1}\{{t.A_i=a_i}\}\right)\\
  &=\sum_{t_p\in D}Pr(t.A_i=a_i|\Do(A_c)=c)\\
  &=|D| Pr(A_i=a_i|\Do(A_c)=c)\\
\end{align}


\end{proof}




==> whatif-algo--OLD.tex <==
\subsection{Computation of What-If Queries}\label{sec:whatif-algo}
% A naive computation of what-if queries would consider all possible paths in the grounded causal graph, and thus result in exponential complexity in the size of the database. 

In this section, we show how we efficiently compute the results of what-if queries. 
First, note that a naive computation of what-if queries would consider all instances in the possible world, and thus result in exponential complexity in the size of the database. 
We therefore provide two optimizations in this section: (1) instead of computing the query over the entire database, we compute the result of a slightly different query over subsets of tuples (as fewer tuples make the computation more efficient) and then combine the results to get the result of the original query over the entire database and (2) we show how standard causal inference techniques can be used to compute the query result when the post-update distribution is determined by a PRCM. 

\paragraph{Decomposing the computation}
We now review the definitions of block-independent databases and decomposable functions which are needed for the efficient computation of what-if query results and then we prove that the computation over blocks can be aggregated into the result over the entire database.
% that allow us to use causal inference techniques to compute the results. 
% Intuitively, instead of computing the query over the entire database, we want to compute the result of a slightly different query over small blocks of the database (as fewer tuples make the computation more efficient) and then be able to combine the results to get the result of the original query over the entire database. 
We use the standard assumption of block-independent database \cite{ReS07,DalviRS09} to simplify the calculation. This assumption has also been utilized in previous work on hypothetical reasoning \cite{JampaniXWPJH08}. 
First, we need the notion of Independence. We say that two tuples $t,t' \in D$ are {\bf independent} if there are no paths in the ground causal graph between any $A[t]$ and $A'[t']$, i.e., $t$ and $t'$.

% Therefore, we consider a partition of the database into blocks of tuples, where each block is independent from all other blocks. 

% However, if the database $D$ can be partitioned into blocks of tuples $B_1, \ldots, B_l$ such that $B_i \subseteq D$, $\cup_{i=1}^l B_i = D$, $B_i \cap B_j = \emptyset$, the computation can be made more effitient


% We use the following {\em structural homogeneity assumption} introduced in \cite{SalimiPKGRS20}, which is necessary for estimating the conditional probability distributions from a given observed dataset, and thereby conduct causal inference. \amir{More context?}
% % Recall that  $\fAtt^{\skl} \subseteq \FAtt^{\skl}$ denotes the set of all groundings of an attribute $\fAtt \in \FAtt$ in $\FAtt^{\skl}$: 

% \begin{itemize}
%     \item \textbf{Structural homogeneity:}  All grounded attributes ${\mb A_{mu}}$ of the same  attribute $A \in \mb A_{mu}$ share the same structural equation and, hence, the same conditional probability distribution in equation \ref{eq:bayesian}.
% \end{itemize}

% %that all the grounded atoms $\fAtt[\mb x] \in \fAtt^{\skl}$ of an attribute function $\fAtt \in \fAtt$ have the same generative process. 
% For instance, in Figure~\ref{ex:grounded-graph}, we assume that all groundings of type $\mathit{Price}$ share the same conditional probability distribution. 

% To simplify computation in the context of probabilistic databases, the literature proposes block-independent databases .

\begin{definition}[Block-independent database]
Given a database $D$, a hypothetical update $U$ and a post-update distribution stemming from a PRCM with a ground causal graph, $D$ is a {\bf block-independent database} if $D$ can be partitioned into blocks of tuples $B_1, \ldots, B_l$ such that $B_i \subseteq D$, $\cup_{i=1}^l B_i = D$, $B_i \cap B_j = \emptyset$, and for each $t \in B_i$ and $t' \in B_j$, $t$ and $t'$ are independent. 
\end{definition}

\begin{example}\label{ex:blocks}
Suppose that in the causal graph of the PRCM defined on the database presented in Figure \ref{fig:database}, tuples of different categories are independent. 
Then, $p_1, p_2, p_3$ in Figure \ref{tbl:amazondatabase} form a block that is independent from the rest of the tuples since they are the only ones with Category Laptop. 
\end{example}

This definition does not restrict our model in any way since, if there are no independent tuples in $D$, then $D$ is considered a single block. 

% Given a database $D$ with independent blocks $B_1, \ldots, B_l$, we can decompose the probability of a possible world $I \in PWD(D)$ by using the formula
% $\pr_{D,U}(I) = \prod_{i=1}^l \pr_{D,U}({B_i})$. 
% In particular, when the blocks are of size $1$, i.e., all tuples in $D$ are independent, we can say that $\pr_{D,U}(I) = \prod_{i=1}^n \pr_{D,U}({t_i})$. 





% We now present a proposition that allows us to compute the output of a what-if query over the entire database by computing a slightly different what-if query over each block and summing the results. 
We now present the second definition that will be used in our propositions of decomposable functions that allows us to compute the output of a what-if query over the entire database by computing a slightly different what-if query over each block and aggregating the results. 

\begin{definition}[Decomposable aggregate function]\label{def:decomposable}
Given a database $D$ that can be divided into blocks $\mathcal{B} = \{B_1, \ldots, B_l\}$, a what-if query $Q$, and a possible world $I \in PWD(D)$, an aggregate function $f: D \to \mathbb{R}$ is decomposable if there exist functions $f': \mathcal{B} \to \mathbb{R}$ and $g: \{x_1, \ldots, x_l\} \to \mathbb{R}$, $x_i \in \mathbb{R}$, such that: 

\begin{itemize}
    \item $\valwhatif(Q, D, I) = g(\{f'(Q,D,B) \mid \forall B\in \mathcal{B}_I\})$ where $\mathcal{B}_I$ is the block partition of $I$, and 
    \item $\alpha g(\{x_1,\ldots,x_l\}) = g(\{\alpha x_1,\ldots,\alpha x_l\})$, $\forall \alpha \geq 0$
    \item $ g(\{x_1,\ldots,x_l\}) + g(\{y_1,\ldots,y_l\}) = g(\{x_1+y_1,\ldots, x_l+y_l\})$
\end{itemize}\label{assume:homogenous}
% \begin{itemize}
%     \item $f(Q,D,I) = g(\{f'(Q,D,B) \mid \forall B\in \mathcal{B}_I\})$
%     \item $\alpha g(\{x_1,\ldots,x_l\}) = g(\{\alpha x_1,\ldots,\alpha x_l\})$, $\forall \alpha \geq 0$
%     \item $ g(\{x_1,\ldots,x_l\}) + g(\{y_1,\ldots,y_l\}) = g(\{x_1+y_1,\ldots, x_l+y_l\})$
% \end{itemize}\label{assume:homogenous}
\end{definition}

Every supported aggregate function in this paper  
($\sumsql$, $\avg$, $\ct$) is decomposable. We next demonstrate this for $\avg$. 
% e.g., $\sumsql$ can be broken down into the sum of each block as $f'$ and the sum of the sums of all blocks as $g$. 
\begin{example}\label{ex:decomposable}
Reconsider the what-if query in Figure \ref{fig:whatif-query}. Suppose the database can be partitioned into blocks by Category as demonstrated in Example \ref{ex:blocks}. 
In this case, $\valwhatif(Q, D, I) = \avg(\{Rating[t'] \mid t'\in \cviewpwd, Category[t] = Laptop, PID[t'] = PID[t]\})$. 
We use the formula for decomposing average $\avg(D) = \sum_{i=1}^l \frac{|B_i|}{|D|} \avg(B_i)$. 
For each block, 
$f'(Q,B'',B') = \frac{|B''|}{|D|} \avg(\{Rating[t'] \mid t'\in \cviewpwd, Category[t] = Laptop, PID[t']=PID[t]\})$ and $g = \sumsql$. Indeed, $\sumsql$ satisfies the properties in Definition \ref{def:decomposable}.
\end{example}

% represented as $f$ in the query in Figure \ref{fig:generic-query}, there exists a function that operates on blocks $f'$ such that $f(Q,D,I) = \sum_{B\in \mathcal{B}_I} f'(Q,D,B)$ for some $f'$. 
% All supported aggregates satisfy this assumption Note that $f(Q,D,B)=f'(Q,D,B)$ if $Agg$ denotes $\ct$ or $\sumsql$. Whenever $Agg=\avg$ or $Agg=\minsql$, $f'(Q,D,B)=c f(Q,D,B)$, where $c$ is a constant that can be estimated from the query $Q$. \sg{Add more discussion on f'}

% \begin{proposition}\label{prop:blocks}
% Consider the what-if query $Q$:
% \begin{align*}
% &Q\equiv\when\  g(A_l)\  Then\\
% &\update\ A_c= c\\
% &\select\ Agg(\post(B))\\
% &\where\  \pre(A_j)=a_j~\and\ \post(A_i) = a_i %~\and\\
% %&\groupby&\  \pre(A_k), \post(A_p)
% \end{align*}
% and $f(Q,D,I)$ as in Definition \ref{def:agg_func}. If $f(Q,D,I) = \sum_{B\in \mathcal{B}_I} f'(Q,D,B)$, then $Q(D) = \sum_{B''\in \mathcal{B}_D}\expectation_{B' \in \overline{PWD}(Q,B'')}[f'(Q, D, B')] $.
% \end{proposition}

\begin{proposition}[Decomposed computation]\label{prop:blocks}
Given a database $D$ that can be divided into blocks $\mathcal{B} = \{B_1, \ldots, B_l\}$, the what-if query $Q$:
\begin{align*}
&\use\\ 
& (\select\ T1.ID, T1.A_j, T1.A_i, Agg1(T2.B)\\
& \where\ T1.ID = T2.ID\\ 
& \groupby\ T1.ID) \as\ RelevantView\\
&\when\  g(A_l)\  Then\\
&\update(A_c)= c\\
&\outputw\ Agg2(\post(B))\\
&\forw\ \pre(A_j)=a_j~\and\
\post(A_i) = a_i 
%~\and\\
%&\groupby&\  \pre(A_k), \post(A_p)
\end{align*}
and $f(Q,D,I)=Agg(\{t'.B \mid t'\in I, t\in Pre(Q,I), t'.ID=t.ID, t' \in Post(Q,I)\})$. 
If $Agg$ is a decomposable function, i.e., there exist  functions $g$ and $f'$ according to Definition~\ref{def:decomposable}, 
% then the expected output of the query $Q(D) = g\left(\left\{\expectation_{B' \in \overline{PWD}_{B''}}[f'(Q, D, B')] \forall B''\in \mathcal{B}_D\right\}\right)$.
then $Q(D) = g(\{Q'(B'') \mid \forall B''\in \mathcal{B}\})$, 
where $Q'$ is the same query as $Q$ with $f'$ replacing $f$ and $Q'(B'') = \expectation_{B' \in \overline{PWD}_{B''}}[f'(Q, D, B')]$.
\label{lem:general}
\end{proposition}

\amir{Not sure if we need the following discussion. Leaving as is for now:}
In the proof of the above proposition, we leverage leverage the ability to marginalize the distribution $\pr_{D,U}$ over the possible worlds of the database $D$ given a what-if query $Q$ (Definition \ref{def:rel-poss-worlds}) to get a distribution and a set of possible worlds for any block $B_i\subseteq D$, which we denote as $PWD(B_i)$. $PWD(B_i)$ are all instances where all tuples $t' \notin B_i$ remain unchanged and all attributes of $t\in B_i$ can get all possible values from their respective domains. 
We further abuse notation and denote $\overline{PWD}(B_i)$ as the set of possible worlds of $B_i$ that only includes the subset of tuples that originated in $B_i$. 
% For this analysis, we consider a block decomposition of $D$, denoted by $\mathcal{B}_D=\{B_1,\cdots,B_k\}$ where $B_i\cap B_j = \phi, \forall i\neq j$ and $\cup B_i = D$ where tuples in different blocks are independent. 
We also notice that, given a database $D$ with a block partition $\mathcal{B}=\{B_1,\cdots,B_l\}$, and a what-if query, $Q$, with an update $U$:
\begin{enumerate}
    \item $\sum_{I\in PWD(D)} \Pr_{D,U}(I) = 1$ and $\sum_{I'\in PWD(B_i)} \Pr_{D,U}(I') = 1$, i.e., the sum of probabilities for all possible worlds of a database or a block is 1.
    \item $PWD(D) = \times_{i=1}^l \overline{PWD}(B_i)$, i.e., $PWD(Q,D)$ is equal to the Cartesian product of $\overline{PWD}(B_i), \forall B_i\in \mathcal{B}_D$, where $\overline{PWD}(B_i)$ contains all instances from $PWD(B_i)$ restricted to tuples in $B_i$.
    % \item Consider a partitioning of $D$ into blocks $\mathcal{B}_D=\{B_1,\cdots,B_l\}$. 
    % $PWD$ is equal to the Cartesian product of $\overline{PWD}_{B_i}, \forall B_i\in \mathcal{B}_D$, where $\overline{PWD}_{B_i}$ contains all instances from $PWD_{B_i}$ restricted to tuples in $B_i$. Mathematically, $\overline{PWD}_B = \{I\cap B,~\forall I\in PWD_B\}$  where $I\cap B = \{t: t\in I, t.ID=t'.ID \text{ for some }t'\in B\}$.
    \item If the tuples in different blocks of the database are independent, then $\Pr_{D,U}(I) = \prod\limits_{I'\in PWD(B_i), \forall B_i\in \mathcal{B}} \Pr_{D,U}(I') $
\end{enumerate} 


\begin{example}\label{ex:prop-blocks}
Continuing Example \ref{ex:decomposable}, for the what-if query $Q$ in Figure \ref{fig:whatif-query}. Suppose the database can be partitioned into blocks by Category as demonstrated in Example \ref{ex:blocks}. 
$Q(D)$ is then defined as the sum of the results of queries $Q'$ over each block $B$, where the aggregate function in $Q'$ for block $B$ is defined as $\frac{|B_i|}{|D|} \avg(\{Price[t'] \mid t'\in I, Category[t] = Laptop, PID[t']=ID[t]\})$. 
\end{example}


\paragraph{Computing results with causal inference}
% Proposition \ref{prop:blocks} proves that the computation can be performed on blocks. 
We provide the link between a what-if query result and causal inference. This link will allow us to compute the results for each block. 
The following proposition formulates the query result for each aggregate function we consider as an expression that can be inferred through causal approaches, although it applies for any what-if query without the need for a PRCM. 

% \begin{proposition}
% Given a what-if query $Q$ with a $\select$ clause on $\maxi/\mini Agg(\post(A_T))$, and a database $D$ partitioned into blocks $\mathcal{B} = \{B_1, \ldots, B_l\}$. 
% Assume that $Agg(\post(D.A_T))$ can be decomposed into $\sum_{B_i \in \mathcal{B}}Agg'(B_i)$, then $Q(D) = $ \amir{continue}.
% \end{proposition}

\begin{proposition}[Connection to causal inference]\label{prop:causal-results}
Given a database $D$, a what-if query $Q$ with an update $U$, and the post-update distribution $\pr_{D,U}$, where $Q$ is of the form:
\begin{align*}
% &\when\ g(A_l)\  Then\\
% &\update\ A_c\ BY\ f(A_c)\\
% &\select\ Agg(\post(B))\\
% &\where\  \pre(A_j)=a_j~ \and\
% \post(A_i) = a_i 
&\use\\ 
& (\select\ T1.ID, T1.A_j, T1.A_i, Agg1(T2.B)\\
& \where\ T1.ID = T2.ID\\ 
& \groupby\ T1.ID) \as\ RelevantView\\
&\when\  g(A_l)\  Then\\
&\update(A_c)= c\\
&\outputw\ Agg2(\post(B))\\
&\forw\ \pre(A_j)=a_j~\and\
\post(A_i) = a_i 
\end{align*}
the following holds:
\begin{itemize}
    \item If $Agg = \ct$, $B=*$, $Q(D) =  |g(A_l)| \pr_{D,U}(A_i=a_i| A_j=a_j, g(A_l)) + \sum_{t\in D}\mathbbm{1}\{t.A_j=a_j, t\notin g(D.A_l), t.A_i=a_i\}$
    \item If $Agg = \sumsql$, $Q(D)=|g(A_l)|\sum_{b\in \Dom(B)} a_j\pr_{D,U}(A_i=a_i,B=b| A_j=a_j, g(A_l)) + \sum_{t\in D} \mathbbm{1}\{t.A_j=a_j, t\notin g(D.A_l), t.A_i=a_i\}t.B$
    % $Q(D) =  \expectation(A_i=a_i|A_c = f(A_c), A_j=a_j, g(A_j)) + \expectation_{t\in D}\mathbbm{1}\{t.A_j=a_j, t\notin g(D.A_j), t.A_i=a_i\}$
    \item If $Agg = \avg $, $Q(D)=\frac{1}{|D|}(|g(A_l)|\sum_{b\in \Dom(B)} a_j\pr_{D,U}(A_i=a_i,B=b| A_j=a_j, g(A_l)) + \sum_{t\in D} \mathbbm{1}\{t.A_j=a_j, t\notin g(D.A_l), t.A_i=a_i\}t.B)$
    %\item If $Agg = \minsql$, \amir{continue}
\end{itemize}
\end{proposition}
\sg{Shall we add a discussion about computation of prob. in proposition here or a separate section with implementation and optimization?}

% For simplicity, Propositions \ref{prop:blocks} and \ref{prop:causal-results} do not consider a $\groupby$ clause and an intervention over multiple disconnected attributes, but it can easily be extended to include these. 


If the post-update distribution $\pr_{D,U}$ is determined by a PRCM, the equations in Proposition \ref{prop:causal-results} allow us to compute the query results by employing 
% After establishing the connection between what-if query results to causal inference, 
any available causal inference approach (e.g., regression \cite{angrist2008mostly} and matching \cite{ho2007matching, Rosenbaum93, iacus2009cem}) to get the probability estimations, and thus the query results. 

% We now describe the algorithm for computing the result of a what-if query. \amir{describe the algorithm and connect to causal inference.}

% \begin{algorithm}[]
% 	\SetKwFunction{Evaluate What-if Query}{Evaluate What-if Query}
% 	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
% 	\LinesNumbered
% 	\Input{What-if query $Q$, database $D$ with block partition $B_1, \ldots, B_l$}
%     \Output{$Q(D)$}
% 	\BlankLine
% 	Find $f'$ such that $f(Q,D,I) = g(f'(Q,D,B_1), \ldots, f'(Q,D,B_l))$\;
% 	$res \gets 0$\;
% 	\For{$B_i \in \mathcal{B}$}
% 	{
% 	   % $\expectation_{B' \in \overline{PWD}(Q,B_i)}[f(Q, D, B')] \gets$ \amir{connect to causal inference}\;
% 	   $sum_{u \in \dom(Backdoor(A_{c1}, A_{c2}))} \pr(B_{A_{c1}, A_{c2} \gets f_1(A_{c1}), f_2(A_{c2})}(u)) \pr(u \mid \post \amir{ conditions})$\;
% 	    $res \gets res + \expectation_{B' \in \overline{PWD}(Q,B_i)}[f(Q, D, B')]$\;
% 	}
% 	\Return $res$\;\label{l:return}
% 	\caption{Evaluate What-if Query} 
% 	\label{algo:what-if}
% \end{algorithm}


